Revisiting the Efficiency of Asynchronous Multi Party Computation Against General Adversaries

In this paper, we design secure multi-party computation (MPC) protocols in the asynchronous communication setting with optimal resilience. Our protocols are secure against a computationally-unbounded malicious adversary, characterized by an adversary structure $\mathcal{Z}$, which enumerates all possible subsets of potentially corrupt parties. Our protocols incur a communication of $\mathcal{O}(|\mathcal{Z}|^2)$ and $\mathcal{O}(|\mathcal{Z}|)$ bits per multiplication for perfect and statistical security respectively. These are the first protocols with this communication complexity, as such protocols were known only in the synchronous communication setting (Hirt and Tschudi, ASIACRYPT 2013).

==> AppPerfectAMPC.tex <==
\section{Perfectly-Secure AMPC}
\label{app:Perfect}
%----
\subsection{Asynchronous VSS Protocol}
%---
In this section, we recall the perfectly-secure VSS protocol $\PiPerVSS$ from \cite{CP20}. The protocol is designed with respect to an adversary structure
 $\AdvStructure$ and sharing specification $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$, such that 
  $\AdvStructure$
   satisfies the
   $\Q^{(4)}(\PartySet, \AdvStructure)$ condition (this automatically implies that $\ShareSpec$ satisfies the 
    $\Q^{(3)}(\ShareSpec, \AdvStructure)$
   condition). The input for the dealer $P_{\D}$ in the protocol is a vector of shares
    $(s_1, \ldots, s_h)$ and the goal is to ensure that the parties output a secret-sharing of $s \defined s_1 + \ldots + s_h$, such that 
    $[s]_q = s_q$, for each $S_q \in \ShareSpec$. 
    The protocol guarantees that even if $P_{\D}$ is {\it corrupt}, if some honest party completes the protocol, then every honest party eventually completes the protocol, such
    that there exists some value, which has been secret-shared by $P_{\D}$.
   
   The high level idea of the protocol is as follows: dealer gives the share
    $s_q$ to all the parties in the set $S_q \in \ShareSpec$. To verify whether dealer has distributed the {\it same} share to all the parties in $S_q$, the 
    parties in $S_q$ perform pairwise consistency test of the supposedly common share and {\it publicly} announce the result. 
    Next the parties check if there exists a subset of ``core" parties $\C_q$, where $S_q \setminus \C_q \in \AdvStructure$, who have positively confirmed the pairwise
    consistency of their supposedly common share. Such a subset $\C_q$ is guaranteed for an {\it honest} dealer, as the set of honest parties in $S_q$ always 
    constitute a candidate $\C_q$. To ensure that all honest parties have the same version of the core sets $\C_1, \ldots, \C_h$,
    dealer is assigned the task of identifying these sets based on the results of the pairwise consistency tests and making them public. 
    Once the core sets are identified and verified, it guarantees that 
        dealer has distributed some common share  to all {\it honest} parties within $\C_q$.
    The next goal is to ensure that even the honest parties in $S_q \setminus \C_q$ get this common share, which is required as per the semantics of our
    secret-sharing.
    For this, the (honest) parties in $S_q \setminus \C_q$ ``filter" out the supposedly common shares received during the pairwise consistency test
    and ensure that they obtain the common share held by the honest parties in $\C_q$. 
    Protocol $\PiPerVSS$ is formally presented in Fig \ref{fig:PerAVSS}.
    %----    
\begin{protocolsplitbox}{$\PiPerVSS$}{The perfectly-secure VSS protocol for realizing $\FVSS$ in the $\FAcast$-hybrid model. 
 The above steps are executed by every $P_i \in \PartySet$}{fig:PerAVSS}
\justify
%----

\begin{myitemize}
%----
\item {\bf Distribution of Shares by $P_{\D}$} : If $P_i$ is the dealer $P_{\D}$, then execute the following steps.
	\begin{myenumerate}
	%----
	\item On having the shares
	 $s_1, \ldots, s_h \in \F$, send $(\dist, \sid, P_{\D}, q, [s]_q)$ to all the parties $P_i \in S_q$, 
	 corresponding to each $S_q \in \ShareSpec$, where $s \defined s_1 + \ldots + s_h$ and $[s]_q = s_q$.
	%----
	\end{myenumerate} 
%----
\item {\bf Pairwise Consistency Tests and Public Announcement of Results} : For each $S_q \in \ShareSpec$, if $P_i \in S_q$, then execute the following steps.
	\begin{myenumerate}
	%----
	\item Upon receiving $(\dist, \sid, P_{\D}, q, s_{qi})$ from $\D$, send $(\test, \sid, P_{\D}, q, s_{qi})$ to every party $P_j \in S_q$.
	%----
	\item Upon receiving $(\test, \sid, P_{\D}, q, s_{qj})$ from $P_j \in S_q$,
	send $(\Sender, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i, j))$ to $\FAcast$ if 
	$s_{qi} = s_{qj}$, where $\sid^{(P_{\D}, q)}_{ij} = \sid || P_{\D} || q || i || j$.\footnote{The notation $\sid^{(P_{\D}, q)}_{ij}$ is used here to distinguish among the different calls to
	$\FAcast$ within the session $\sid$.}
	%----
	\end{myenumerate}
%----
\item {\bf Constructing Consistency Graph} : For each $S_q \in \ShareSpec$, execute the following steps.
	\begin{myenumerate}
	%----
	\item Initialize $\C_q$ to $\emptyset$. Construct an undirected consistency graph $G^{(i)}_q$ with $S_q$ as the vertex set.
	%----
         \item For every ordered pair of parties $(P_j, P_k)$ where $P_j, P_k \in S_q$, 
          keep requesting an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$, till an output is received.
   	%----
	\item Add the edge $(P_j, P_k)$ to $G^{(i)}_q$ if
	an output $(P_j, \Acast, \sid^{(P_{\D}, q)}_{jk}, \OK_q(j, k))$ and 
	$(P_k, \Acast, \sid^{(P_{\D}, q)}_{kj}, \allowbreak \OK_q(k, j))$ is received from $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$ and 
	$\FAcast$ with $\sid^{(P_{\D}, q)}_{kj}$ respectively.
	%----
	\end{myenumerate}
%----
\item {\bf Identification of Core Sets and Public Announcements} :  If $P_i$ is $P_{\D}$, then execute the following steps.
	%----
	\begin{myenumerate}
	%----
	\item For each $S_q \in \ShareSpec$, check if there exists a subset of parties $\W_q \subseteq S_q$, such that $S_q \setminus \W_q \in \AdvStructure$
	and the parties in $\W_q$ form a clique in the consistency graph $G^{\D}_q$. If such a $\W_q$ exists, then assign $\C_q \coloneqq \W_q$.
	%----
	\item Upon computing a set $\C_q$ satisfying the above conditions 
	for each $S_q \in \ShareSpec$, send $(\Sender, \Acast, \sid_{P_{\D}}, \allowbreak \{ \C_q \}_{S_q \in \ShareSpec})$, where $\sid_{P_{\D}} = \sid || P_{\D}$.
	%----
	\end{myenumerate}
%----
\item {\bf Share Computation} : Execute the following steps.
	%----
	\begin{myenumerate}
	%----
	\item[1.] For each $S_q \in \ShareSpec$ such that $P_i \in S_q$, initialize $[s]_q $ to $\bot$.
	%----
	\item[2.] Keep requesting an output from $\FAcast$ with $\sid_{\D}$ until an output is received.
	%----
	\item[3.] Upon receiving an output $(\Sender, \Acast, \sid_{P_{\D}}, \{ \C_q \}_{S_q \in \ShareSpec})$ from $\FAcast$ with $\sid_{P_{\D}}$, 
	wait until the parties in $\C_q$ form a clique in $G^{(i)}_q$, corresponding to each $S_q \in \ShareSpec$. Then verify if
	$S_q \setminus \C_q \in \AdvStructure$, for each $S_q \in \ShareSpec$. If the verification is successful, then proceed to compute the output
	as follows.
	%-----
	    \begin{myenumerate}
	    %---
	    \item[i.] Corresponding to each $\C_q$ such that $P_i \in \C_q$, set $[s]_q \coloneqq s_{qi} $.
	    %---
	    \item[ii.] Corresponding to each $\C_q$ such that $P_i \not \in \C_q$, set $[s]_q \coloneqq s_{q}$, where $(\test, \sid, P_{\D}, q, s_{q})$ 
	     is received from a set of parties $\C'_q$
	    such that $\C_q \setminus \C'_q \in \AdvStructure$. 
	    %---
	    \end{myenumerate}
	%----
	\item[4.] Once $[s]_q \neq \bot$ for each $S_q \in \ShareSpec$ such that $P_i \in S_q$, output $(\Share, \sid,P_{\D}, \{[s]_q\}_{P_i \in S_q})$.
	%----
	\end{myenumerate}
%----
\end{myitemize}
%----
\end{protocolsplitbox}
%----

The properties of $\PiPerVSS$ are stated in Theorem \ref{thm:PerVSS}.
%---
\begin{theorem}
\label{thm:PerVSS}
%---
 Consider a static malicious adversary $\Adv$ characterized by an adversary-structure $\AdvStructure$, satisfying the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition
  and let  $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$ be the sharing specification.\footnote{Hence $\ShareSpec$
   satisfies the $\Q^{(3)}(\ShareSpec, \AdvStructure)$ condition.} 
  Then protocol $\PiPerVSS$ UC-securely realizes the functionality $\FVSS$
   with perfect security in the $\FAcast$-hybrid model, in the 
   presence of $\Adv$.
   The protocol makes $\Order(|\AdvStructure| \cdot n^2)$ calls to $\FAcast$ with $\Order(\log{n})$ bit messages
    and additionally incur a communication of 
   $\Order(|\AdvStructure| \cdot n^2 \log{|\F|})$ bits.
   
   By replacing the calls to $\FAcast$ with protocol $\PiAcast$, the protocol incurs a total communication of $\Order(|\AdvStructure| \cdot (n^2 \log{|\F|} + n^4 \log{n}))$
   bits.
%---
\end{theorem}
%-----
\begin{proof}
%----
In the protocol, $|\ShareSpec| = |\AdvStructure|$. The dealer needs to send the share $s^{(q)}$ to all the parties in $S_q$ and every party in $S_q$ has to send
 the received share to every other party in $S_q$ during the pairwise consistency check. This incurs a communication of $\Order(|\AdvStructure| \cdot n^2 \log{|\F|} )$
  bits, since each $|S_q| = \Order(n)$ and each share $s^{(q)}$ can be represented by $\log{|\F|}$ bits. The number of calls to $\FAcast$ follows from the fact that every
  party in $S_q$ may Acast an $\OK$ message for every other party in $S_q$ and every such $\OK$ message represents the index of $2$ parties.

We next prove the security of the protocol. Let $\Adv$ be an arbitrary adversary, attacking the protocol $\PiPerVSS$ by corrupting a set of parties
  $Z^{\star} \in \AdvStructure$ and let $\Env$ be an arbitrary environment. We show the existence of a simulator $\SimPVSS$, such that for any
 $Z^{\star} \in \AdvStructure$,
  the outputs of the honest parties and the view of the adversary in the 
   protocol $\PiPerVSS$ is indistinguishable from the outputs of the honest parties and the view of the adversary in an execution in the ideal world involving 
  $\SimPVSS$ and $\FVSS$. The steps of the simulator will be different depending on whether the dealer is corrupt of honest.

If the dealer is {\it honest}, then the simulator interacts with $\FVSS$ and receives the shares of the corrupt parties, corresponding to the sets $S_q \in \ShareSpec$ 
 which they are part of. With these shares, the simulator then plays the role of the dealer as well as the honest parties, as per the steps of $\PiPerVSS$ and interact with
  $\Adv$. The simulator also plays the role of $\FAcast$. If $\Adv$ queries $\FAcast$ for the result of any pairwise consistency test involving an honest party, the simulator provides the appropriate result. In addition, the simulator records the result of any test involving corrupt parties which $\Adv$  sends to $\FAcast$. 
   Based on the results of these pairwise consistency tests, the simulator finds the core sets for each $S_q$ and sends these to $\Adv$ upon request.

If the dealer is {\it corrupt}, the simulator plays the role of honest parties and interacts with $\Adv$, as per the
 steps of  $\PiPerVSS$. This involves recording shares which $\Adv$ distributes to any
  honest party (on the behalf of the dealer),
   as well as performing pairwise consistency tests on their behalf. If $\Adv$ sends core sets for each $S_q \in \ShareSpec$ as input to $\FAcast$, then the simulator checks if these are {\it valid}, and accordingly, sends the shares held by {\it honest} parties in these core sets as the input shares to $\FVSS$ on the behalf
   of the dealer. The simulator is presented in Figure \ref{fig:SimPVSS}.

%----
\begin{simulatorsplitbox}{$\SimPVSS$}{Simulator for the protocol $\PiPerVSS$ where $\Adv$ corrupts the parties in set $Z^{\star}$, where $Z^{\star} \in \AdvStructure$}{fig:SimPVSS}
	\justify
%----
$\SimPVSS$ constructs virtual real-world honest parties and invokes the real-world adversary $\Adv$. The simulator simulates the view of
 $\Adv$, namely its communication with $\Env$, the messages sent by the honest parties and the interaction with $\FAcast$. 
  In order to simulate $\Env$, the simulator $\SimPVSS$ forwards every message it receives from 
   $\Env$ to $\Adv$ and vice-versa.  The simulator then simulates the various phases of the protocol as follows, depending upon whether the dealer is honest or corrupt. \\~\\
%---
 \centerline{\underline{\bf Simulation When $P_{\D}$ is Honest}} 
%----
\noindent {\bf Interaction with $\FVSS$}: the simulator interacts with the functionality $\FVSS$ and receives a request based delayed output
  $(\Share,\sid,P_{\D},\{[s]_q\}_{S_q \cap Z^{\star} \neq \emptyset})$, on the behalf of the parties in $Z^{\star}$. \\[.2cm]
%----
\noindent {\bf Distribution of Shares by $P_{\D}$}: On the behalf of the dealer, the simulator sends $(\dist, \sid, P_{\D}, q, [s]_q)$ to $\Adv$, corresponding to 
 every $P_i \in Z^{\star} \cap S_q$. \\[.2cm]
%----     
 \noindent {\bf Pairwise Consistency Tests}: For each $S_q \in \SharingSpec$ such that $S_q \cap Z^{\star} \neq \emptyset$,
  corresponding to each $P_i \in S_q \cap Z^{\star}$, the simulator does the following.
 	\begin{myitemize}
 	\item[--]  On the behalf of every party $P_j \in S_q \setminus Z^{\star}$, send $(\test, \sid, P_{\D}, q, s_{qj})$ to $\Adv$, where $s_{qj} = [s]_q$.
 	\item[--] If $\Adv$ sends $(\test, \sid, P_{\D}, q, s_{qi})$ on the behalf of $P_i$ to any $P_j \in S_q$, then record it.
 	\end{myitemize}
%-----
 \noindent {\bf Announcing Results of Consistency Tests}: 
\begin{myitemize}
\item[--] If for any $S_q \in \SharingSpec$, $\Adv$ requests an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$ corresponding to parties
 $P_i \in S_q \setminus Z^{\star}$ and $P_j \in S_q$, then the simulator provides output on the behalf of $\FAcast$ as follows.
 	\begin{myitemize}
 	\item If $P_j \in S_q \setminus Z^{\star}$, then send the output $(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$.
 	\item If $P_j \in (S_q \cap Z^{\star})$, then send the output $(P_i, \Acast ,\sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$, if 
	the message $(\test, \sid, P_{\D}, \allowbreak q, s_{qj})$ has been recorded 
	         on the behalf of $P_j$ for party $P_i$ and 
	       $s_{qj} = [s]_q$ holds.	         	       
	\end{myitemize} 
\item[--] If for any $S_q \in \SharingSpec$ and any $P_i \in S_q \cap Z^{\star}$, 
 $\Adv$ sends $(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ to $\FAcast$
 with $\sid^{(P_{\D}, q)}_{ij}$ on the behalf of 
  $P_i$ for any $P_j \in S_q$, then the simulator records it. 
  Moreover, if $\Adv$ requests an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$, then 
  the simulator sends the output $(P_i, \Acast ,\sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ on the behalf of $\FAcast$.
  %---
\end{myitemize}
%-----
\noindent {\bf Construction of Core Sets and Public Announcement}: 
\begin{myitemize}
\item[--] For each $S_q \in \ShareSpec$, the simulator plays the role of $P_{\D}$ and adds edge $(P_i,P_j)$ to the graph $G^{\D}_q$ over the vertex set $S_q$, if the following hold.
	\begin{myitemize}
	\item $P_i,P_j \in S_q$.
	\item One of the following is true.
		\begin{myitemize}
		\item $P_i,P_j \in S_q \setminus Z^{\star}$.
		\item If $P_i \in S_q \cap Z^{\star}$ and $P_j \in S_q \setminus Z^{\star}$, then the simulator has recorded 
		$(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ sent by $\Adv$ on the behalf of $P_i$ to $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$,
		 and recorded $(\test, \sid, P_{\D}, q, s_{qi})$ on the behalf of $P_i$ for $P_j$ such that $s_{qi} = [s]_q$.
		\item If $P_i, P_j \in S_q \cap Z^{\star}$, then the simulator has recorded $(P_i, \Acast, \sid^{(q)}_{ij}, \OK_q(i,j))$
		 and $(P_j, \Acast, \allowbreak \sid^{(q)}_{ji}, \OK_q(j,i))$ sent by $\Adv$ on behalf $P_i$ and $P_j$ respectively, to 
		 $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$ and $\FAcast$ with $\sid^{(P_{\D}, q)}_{ji}$.
		 %---		 
		\end{myitemize}
	\end{myitemize}
\item[--] For each $S_q \in \ShareSpec$, the simulator finds the set $\C_q$ which forms a clique in $G^{\D}_q$, such that $S_q \setminus \C_q \in \AdvStructure$.
  When $\Adv$ requests output from $\FAcast$ with $\sid_{P_{\D}}$, 
  the simulator sends the output $(\Sender, \Acast, \sid_{P_{\D}}, \{\C_q\}_{S_q \in \ShareSpec})$ on the behalf of $\FAcast$.\\~\\
\end{myitemize}
%---
% \noindent {\bf Verification of $\C_q$ for each $S_q \in \SharingSpec$}: \\[.2cm]
%--- 
% \noindent {\bf Share Computation}:  \\~\\
%---   
 \centerline{\underline{\bf Simulation When $P_{\D}$ is Corrupt}} 
 %---
  In this case, the simulator $\SimPVSS$ interacts with $\Adv$ during the various phases of $\PiPerVSS$ as follows. \\[.2cm]
%---
%----
\noindent {\bf Distribution of shares by $P_{\D}$}: If $\Adv$ sends $(\dist, \sid, P_{\D}, q, v)$ 
 on the behalf of $P_{\D}$ to any party $P_i \in S_q \setminus Z^{\star}$, then the simulator records it and sets $s_{qi}$ to be $v$. \\[.2cm]
%----     
 \noindent {\bf Pairwise Consistency Tests}: For each $S_q \in \SharingSpec$ such that 
  $S_q \cap Z^{\star} \neq \emptyset$, corresponding to each party $P_i \in S_q \cap Z^{\star}$ and each 
  $P_j \in S_q \setminus Z^{\star}$, the simulator does the following.
 	\begin{myitemize}
 	\item[--] If $s_{qj}$ has been set to some value, then send $(\test,\sid, P_{\D}, q, s_{qj})$ to $\Adv$ on the behalf of $P_j$.
 	\item[--] If $\Adv$ sends $(\test, \sid, q, P_{\D}, s_{qi})$ on the behalf of $P_i$ to $P_j$, then record it. 
 	\end{myitemize}
%-----
 \noindent {\bf Announcing Results of Consistency Tests}: 
\begin{myitemize}
\item[--] If for any $S_q \in \SharingSpec$, $\Adv$ requests an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$ corresponding to
 parties $P_i \in S_q \setminus Z^{\star}$ and $P_j \in S_q$, then the simulator provides the 
  output on the behalf of $\FAcast$ as follows, if $s_{qi}$ has been set to some value.
 	\begin{myitemize}
 	\item If $P_j \in S_q \setminus Z^{\star}$, then send the output $(P_i,\Acast,\sid^{(P_{\D}, q)}_{ij},\OK_q(i,j))$, if
	$s_{qj}$ has been set to some value and $s_{qi} = s_{qj}$ holds.
 	\item If $P_j \in S_q \cap Z^{\star}$, then send the output $(P_i,\Acast,\sid^{(P_{\D}, q)}_{ij},\OK_q(i,j))$, 
	 if $(\test, \sid, q, P_{\D}, s_{qj})$ sent by $\Adv$ on the behalf of $P_j$ to $P_i$ has been recorded and $s_{qj} = s_{qi}$ holds.
 	\end{myitemize} 
\item[--]  If for any $S_q \in \SharingSpec$ and any $P_i \in S_q \cap Z^{\star}$, 
 $\Adv$ sends $(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ to $\FAcast$
 with $\sid^{(P_{\D}, q)}_{ij}$ on the behalf of 
  $P_i$ for any $P_j \in S_q$, then the simulator records it. 
  Moreover, if $\Adv$ requests an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$, then 
  the simulator sends the output $(P_i, \Acast ,\sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ on the behalf of $\FAcast$.
  \end{myitemize}
%-----
\noindent {\bf Construction of Core Sets}: For each $S_q \in \ShareSpec$, the simulator plays the role of 
 the honest parties $P_i \in S_q \setminus Z^{\star}$ and adds the edge $(P_j,P_k)$ to the graph $G^{(i)}_q$ over vertex set $S_q$, if the following hold.
\begin{myitemize}
	\item[--] $P_j, P_k \in S_q$.
	\item[--] One of the following is true.
		\begin{myitemize}
		\item If $P_j, P_k \in S_q \setminus Z^{\star}$, then the simulator has set $s_{qj}$ and $s_{qk}$ to some values, such that $s_{qj} = s_{qk}$.
		\item If $P_j \in S_q \cap Z^{\star}$ and $P_k \in S_q \setminus Z^{\star}$, then the simulator has recorded 
		$(P_j, \Acast, \sid^{(P_{\D}, q)}_{jk}, \OK_q(j, k))$ sent by $\Adv$ on the behalf of $P_j$ to $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$,
		and recorded $(\test, \sid, q, P_{\D}, s_{qj})$ on the behalf of $P_j$ for $P_k$ and has set $s_{qk}$ to a value such that $s_{qj} = s_{qk}$.
		\item If $P_j, P_k \in S_q \cap Z^{\star}$, then the simulator has recorded 
		$(P_j, \Acast, \sid^{(P_{\D}, q)}_{jk}, \OK_q(j, k))$ and $(P_k, \Acast, \allowbreak \sid^{(P_{\D}, q)}_{kj}, \OK_q(k, j))$ sent by $\Adv$ on behalf of
		$P_j$ and $P_k$ respectively, to $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$ and $\FAcast$ with $\sid^{(P_{\D}, q)}_{kj}$. 		
		\end{myitemize}
\end{myitemize}
%---
\noindent {\bf Verification of Core Sets and Interaction with $\FVSS$}:
   %----
      \begin{myitemize}
      %----
        \item If  $\Adv$ sends $(\Sender, \Acast, \sid_{P_{\D}}, \{\C_q\}_{S_q \in \ShareSpec})$ to $\FAcast$ with $ \sid_{P_{\D}}$ on the behalf of
  $P_{\D}$, then the simulator records it. Moreover, if $\Adv$ requests an output from $\FAcast$ with $ \sid_{P_{\D}}$, then on the behalf
  of $\FAcast$, the simulator sends the output $(P_{\D}, \Acast , \sid_{P_{\D}}, \{\C_q\}_{S_q \in \ShareSpec})$.
       %---
       \item If simulator has recorded the sets  $ \{\C_q\}_{S_q \in \ShareSpec}$, then it plays 
     the role of the honest parties and verifies if $\C_q$ is valid for each $S_q \in \ShareSpec$, by checking
     if $S_q \setminus \C_q \in \AdvStructure$ and if $\C_q$ constitutes a clique in the graph $G^{(i)}_q$ of every party $P_i \in \PartySet \setminus Z^{\star}$.
    If each $\C_q$ is valid, then the simulator sends $(\Share, \sid, P_{\D}, \{s_q\}_{S_q \in \ShareSpec})$ to $\FVSS$, where $s_q$ is set to 
     $s_{qi}$ for any $P_i \in \C_q \setminus Z^{\star}$. 
     \end{myitemize}
     
%--- 
\end{simulatorsplitbox}   
%----

We now prove a series of claims, which helps us to prove the theorem. We start with an {\it honest}
 $P_{\D}$.
%-----
\begin{claim}
\label{claim:PVSSHonestDPrivacy}
%---
If $P_{\D}$ is honest, then the view of $\Adv$ in the simulated execution of $\PiPerVSS$ with $\SimPVSS$ is identically distributed to the view of $\Adv$ in the real execution of $\PiPerVSS$ involving honest parties.
%---
\end{claim}
%----
\begin{proof}
%----
Let $\ShareSpec^{\star} \defined
  \{S_q \in \ShareSpec \mid S_q \cap Z^{\star} \neq \emptyset \}$. Then the 
   view of $\Adv$ during the various executions consists of the following.
\begin{myenumerate}
\item[--] The shares $\{[s]_q\}_{S_q \in \ShareSpec^{\star}}$ distributed by $P_{\D}$: In the real execution, $\Adv$ receives $[s]_q$ from $P_{\D}$ for each $S_q \in \ShareSpec^{\star}$. In the simulated execution, the simulator provides this to $\Adv$ on behalf of $P_{\D}$. Clearly, the distribution of the shares is identical in both the
 executions.
%----
\item[--] Corresponding to every $S_q \in \ShareSpec^{\star}$, 
  messages $(\test, \sid, P_{\D}, q, s_{qj})$ received from party $P_j \in S_q \setminus Z^{\star}$,
    as part of pairwise consistency tests: While each $P_j$ sends this to $\Adv$ in the real execution, the simulator sends this on the behalf of $P_j$ in the simulated execution.
    Clearly, the distribution of the messages is identical in both the executions.    
%----
\item[--] For every $S_q \in \ShareSpec$ and every $P_i,P_j \in S_q$, the outputs $\OK_q(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$
 of the pairwise consistency tests, received as output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$: 
 To compare the distribution of these messages in the two executions,
  we consider the following cases, considering an arbitrary $S_q \in \ShareSpec$ and arbitrary $P_i, P_j \in S_q$.
	\begin{myitemize}
	%----
	\item[--] $P_i,P_j \in S_q \setminus Z^{\star}$: In both the executions, 
	 $\Adv$ receives $\OK_q(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ as the output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$.
	%----
	\item[--] $P_i \in S_q \setminus Z^{\star}, P_j \in (S_q \cap Z^{\star}) $:  In both the 
	 executions, $\Adv$ receives $\OK_q(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \allowbreak \OK_q(i,j))$ as the output from $\FAcast$ with 
	 $\sid^{(P_{\D}, q)}_{ij}$ if and only if $\Adv$ sent $(\test, \sid, P_{\D}, q, s_{qj})$ on the behalf of $P_j$ to $P_i$ such that $s_{qj} = [s]_q$ holds.
	%----
	\item[--] $P_i \in (S_q \cap Z^{\star}) $:  In both the executions, 
	$\Adv$ receives $\OK_q(P_i, \Acast, \sid^{(q)}_{ij}, \OK_q(i,j))$ if and only if 
	$\Adv$ on the behalf of $P_i$ has sent $(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ to $\FAcast$
	with $\sid^{(P_{\D}, q)}_{ij}$ for $P_j$.
	%----
	\end{myitemize}
%----
   Clearly, irrespective of the case, the distribution of the $\OK_q$ messages is identical in both the executions.
%---
\item[--] The core sets $\{\C_q\}_{S_q \in \ShareSpec}$: In both the 
 executions, the sets $\C_q$ are determined, based on the $\OK_q$ messages delivered to $P_{\D}$. So the distribution of these sets is also identical. 
\end{myenumerate}
%----
\end{proof}
%----

We next claim that if the dealer is {\it honest}, then conditioned on the view of the adversary $\Adv$ (which is identically distributed in both the executions, as per the previous claim),
  the outputs of the honest parties are identically distributed in both the executions.
%----
\begin{claim}
\label{claim:PVSSHonestDCorrectness}
%----
If $P_{\D}$ is honest, then conditioned on the view of $\Adv$, the output of the honest parties during the execution of $\PiPerVSS$ involving $\Adv$ has the
   same distribution as the output of the honest parties in the ideal-world involving $\SimPVSS$ and $\FVSS$.
%----
\end{claim}
%-----
%----
\begin{proof}
%----
Let $P_{\D}$ be honest and let $\View$ be an arbitrary view of $\Adv$. Moreover, let $\{s_q \}_{S_q \cap Z^{\star} \neq \emptyset}$ be the shares
 of the corrupt parties, as per $\View$. Furthermore, let $\{s_q \}_{S_q \cap Z^{\star} = \emptyset}$ be the shares, used by $P_{\D}$
  in the simulated execution, corresponding to the set $S_q \in \ShareSpec$, such that $S_q \cap Z^{\star} = \emptyset$.
   Let $s \defined \displaystyle \sum_{S_q \cap Z^{\star} \neq \emptyset} s_q + \sum_{S_q \cap Z^{\star} = \emptyset} s_q$.
   Then in the simulated execution, each {\it honest} party $P_i$ obtains the output $\{[s]_q\}_{P_i \in S_q}$ from $\FVSS$, where
   $[s]_q = s_q$. We now show that $P_i$ eventually obtains the
    output $\{[s]_q\}_{P_i \in S_q}$ in the real execution as well, if $P_{\D}$'s inputs in the protocol $\PiPerVSS$ are 
    $\{s_q \}_{S_q \in \ShareSpec}$.
    
    Since $P_{\D}$ is {\it honest}, it sends the share $s_q$ to {\it all} the parties in the set $S_q$, which is eventually delivered. Now consider {\it any} $S_q \in \ShareSpec$.
     During the pairwise consistency tests, each {\it honest} $P_k \in S_q$ will eventually send $s_{qk} = s_q$ to 
      {\it all} the parties in $S_q$. Consequently, every {\it honest} $P_j \in S_q$ will eventually send the message $\OK_q(j, k)$ for broadcast to
      $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$, corresponding to every {\it honest} $P_k \in S_q$. This is because $s_{qj} = s_{qk} = s_q$ will hold.
      So, every {\it honest} party (including $P_{\D}$) eventually receives the output
      $\OK_q(P_j, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(j, k))$ from $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$.
      This implies that the parties in $S_q \setminus Z^{\star}$ will eventually form a clique in the graph $G^{(i)}_q$
      of every {\it honest} $P_i$. This further implies that $P_{\D}$ will eventually find a set $\C_q$ where $S_q \setminus \C_q \in \AdvStructure$
      and where $\C_q$ constitutes a clique in the consistency graph of every honest party. 
      This is because the set $S_q \setminus Z^{\star}$ is guaranteed to eventually constitute a clique.
            Hence $P_{\D}$ eventually sends the sets $\{ \C_q\}_{S_q \in \ShareSpec}$ to $\FAcast$ with $\sid_{P_{\D}}$, which are eventually delivered to every honest
      party. Moreover, the verification of these sets will be eventually successful for every honest party.
      
      Next consider an arbitrary {\it honest} $P_i \in S_q$. If $P_i \in \C_q$, then it has already received the share $s_q$ from $P_{\D}$
      and $s_{qi} = s_q$ holds. Hence $P_i$ sets $[s]_q$ to $s_q$. So consider the case when $P_i \not \in \C_q$. In this case, 
      $P_i$ sets $[s]_q$, based on the supposedly common values $s_{qj}$ received from the parties
      $P_j \in S_q$ as part of pairwise consistency tests.
       Specifically, $P_i$ checks for a subset of parties $\C'_q \subseteq \C_q$ where $\C_q \setminus \C'_q \in \AdvStructure$, such that
      every party $P_j \in \C'_q$ has sent the {\it same} $s_{qj}$ value to $P_i$ as part of the pairwise consistency test.
      If $P_i$ finds such a set $\C'_q$, then it sets $[s]_q$ to the common $s_{qj}$.
      To complete the proof, we need to show that $P_i$ will eventually find such a set $\C'_q$
      and if such a set $\C'_q$ is found by $P_i$, then the common $s_{qj}$ is the same as $s_q$.
      
      Assuming that $P_i$ eventually finds such a $\C'_q$, the proof that the common $s_{qj}$ is the same as $s_q$
      follows from the fact that $\C'_q$ is guaranteed to contain at least one {\it honest} party from $\C_q$, who would have received the share
      $s_{qj} = s_q$ from $P_{\D}$ and sent to $P_i$ as part of the pairwise consistency test. This is because $\AdvStructure$
   satisfies the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition.
      Also, since the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition is satisfied, the set of {\it honest} parties in $\C_q$, namely the parties in 
      $\C_q \setminus Z^{\star}$, always constitute a candidate $\C'_q$ set. This is because every party $P_j \in \C_q \setminus Z^{\star}$
      would have sent $s_{qj} = s_q$ to every party in $S_q$ during the pairwise consistency test and these values are eventually delivered. 
      %----
   %----
\end{proof}
%----

We next prove certain claims with respect to a {\it corrupt} dealer. The first obvious claim is that the view of $\Adv$ in this
case is also identically distributed in both the real as well as simulated execution. This is simply
because in this case, the {\it honest} parties have {\it no} inputs
  and the simulator simply plays the role of the honest parties, {\it exactly}
 as per the steps of the protocol $\PiPerVSS$ in the simulated execution.

%------
\begin{claim}
\label{claim:PVSSCorruptDPrivacy}
%---
If $P_{\D}$ is corrupt, then 
the view of $\Adv$ in the simulated execution of $\PiPerVSS$ with $\SimPVSS$ is identically distributed to the view of $\Adv$ in the real execution of
$\PiPerVSS$ involving honest parties.
%---
\end{claim}
%-----
%----
\begin{proof}
%---
The proof follows from the fact that if $P_{\D}$ is {\it corrupt}, then $\SimPVSS$ participates in a full execution of the protocol
 $\PiPerVSS$, by playing the role of the honest parties as per the steps of $\PiPerVSS$.
 Hence, there is a one-to-one correspondence between simulated
  executions and real executions.
%---
\end{proof}
%----

We finally claim that if the dealer is {\it corrupt}, then conditioned on the view of the adversary (which is identical in both
the executions as per the last claim), the outputs of the honest parties are identically distributed in 
 both the executions.
 %----
\begin{claim}
\label{claim:PVSSCorruptDCorrectness}
%----
If $\D$ is corrupt, then conditioned on the view of $\Adv$, the output of the honest parties during the execution of $\PiPerVSS$ involving $\Adv$ has the  same distribution as the output of the honest parties in the ideal-world involving $\SimPVSS$ and $\FVSS$.
%----
\end{claim}
%-----
%----
\begin{proof}
%----
Let $P_{\D}$ be {\it corrupt} and let 
 $\View$ be an arbitrary view of $\Adv$. We note that it can be found out from $\View$ whether valid
   core sets $\{\C_q\}_{S_q \in \ShareSpec}$ have been generated during the corresponding execution of $\PiPerVSS$ or not. We now consider the following cases.
 %---
\begin{myitemize}
%----
\item[--] {\it No core sets $\{\C_q\}_{S_q \in \ShareSpec}$ are generated as per $\View$}: In this case, the honest parties do not obtain any output in either execution.
 This is because in the real execution of $\PiPerVSS$, the honest parties compute their output only when they get valid core sets $\{\C_q\}_{S_q \in \ShareSpec}$
 from $P_{\D}$'s broadcast. And if this is not the case, then in the simulated execution, 
  the simulator $\SimPVSS$ does not provide any input to $\FVSS$ on behalf of $P_\D$; hence, $\FVSS$ does not produce any output for the honest parties.
%----
\item[--] {\it Core sets $\{\C_q\}_{S_q \in \ShareSpec}$ generated as per $\View$ are invalid}:
 Again, in this case, the honest parties do not obtain any output in either execution.
  This is because in the real execution of $\PiPerVSS$, even if the sets 
   $\{\C_q\}_{S_q \in \ShareSpec}$ are received from $P_{\D}$'s broadcast,
    the honest parties compute their output only when each $\C_q$ set is found to be {\it valid}, with respect to the verifications
    performed by the honest parties in their own consistency graphs.
    And if these verifications fail (implying that the core sets are invalid), then in the simulated execution, 
    the simulator $\SimPVSS$ does not provide any input to $\FVSS$ on behalf of $P_\D$, implying that
     $\FVSS$ does not produce any output for the honest parties.
%----
\item[--] {\it Valid core sets $\{\C_q\}_{S_q \in \ShareSpec}$ are generated as per $\View$}:
  We first note that in this case, $P_{\D}$ has distributed some common share, say $s_q$, as determined by $\View$, 
  to all the parties in $\C_q \setminus Z^{\star}$, during the real execution of $\PiPerVSS$. 
  This is because all the parties in $\C_q \setminus Z^{\star}$ are {\it honest}, who form a clique
  in the consistency graph of the honest parties. Hence, 
  every $P_j, P_k \in \C_q \setminus Z^{\star}$ have broadcasted the messages $\OK_q(j, k)$ and $\OK_q(k, j)$
  after checking that $s_{qj} = s_{qk}$ holds, where $s_{qj}$ and $s_{qk}$ are the shares
  received from $P_{\D}$ by $P_j$ and $P_k$ respectively. 
  
  We next show that in the real execution of $\PiPerVSS$, every party in $S_q \setminus Z^{\star}$, eventually sets
  $[s]_q = s_q$. While this is obviously true for the parties in $\C_q \setminus Z^{\star}$, we consider an arbitrary party
  $P_i \in S_q \setminus (Z^{\star} \cup \C_q)$. From the protocol steps, 
   $P_i$ checks for a subset of parties $\C'_q \subseteq \C_q$ where $\C_q \setminus \C'_q \in \AdvStructure$, such that
      every party $P_j \in \C'_q$ has sent the {\it same} $s_{qj}$ value to $P_i$ as part of the pairwise consistency test.
      If $P_i$ finds such a set $\C'_q$, then it sets $[s]_q$ to the common $s_{qj}$.
      We next argue that $P_i$ will eventually find such a set $\C'_q$
      and if such a set $\C'_q$ is found by $P_i$, then the common $s_{qj}$ is the same as $s_q$.
      The proof for this is exactly the {\it same}, as Claim \ref{claim:PVSSHonestDCorrectness}. 
      
      Thus, in the real execution, every honest party $P_i$ eventually outputs $\{[s]_q = s_q \}_{P_i \in S_q}$.
      From the steps of $\SimPVSS$, the simulator sends the shares $\{s_q \}_{S_q \in \ShareSpec}$ to $\FVSS$ on the behalf of
      $P_{\D}$ in the simulated execution. Consequently, in the ideal world, $\FVSS$ will eventually deliver
      the shares $\{[s]_q = s_q \}_{P_i \in S_q}$ to every honest $P_i$.
      Hence, the outputs of the honest parties are identical in both the worlds.
     %----
\end{myitemize}
%----
\end{proof}
%----
The proof of the theorem now follows
  from Claims \ref{claim:PVSSHonestDPrivacy}-\ref{claim:PVSSCorruptDCorrectness}.
%---
\end{proof}

\subsection{Asynchronous Reconstruction Protocols}
%----
Let $s$ be a value which is secret-shared with respect to the sharing specification $\ShareSpec = (S_1, \ldots, S_h)$, such that $\ShareSpec$ satisfies the
 $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition. We first present the protocol 
  $\PiPerRecShare$, which allows {\it all} parties in $\PartySet$ to reconstruct a {\it single} share $[s]_q$, corresponding to a
  designated set $S_q \in \ShareSpec$. In the protocol, every party in $S_q$ sends the share $[s]_q$ to all the parties outside $S_q$, who then
  ``filter" out the potentially incorrect versions of $[s]_q$ and output $[s]_q$. 
     Protocol $\PiPerRecShare$ is formally presented in Figure \ref{fig:PerRecShare}.
%----
\begin{protocolsplitbox}{$\PiPerRecShare(q)$}{Perfectly-secure reconstruction protocol for session id $\sid$ to publicly
  reconstruct the share $[s]_q$ corresponding to $S_q \in \ShareSpec$. 
   The public inputs are $\PartySet$, $\AdvStructure$ and $\ShareSpec$. 
    The above steps are executed by every $P_i \in \PartySet$}{fig:PerRecShare}
%----
\justify
%----
\begin{myitemize}
%----
\item {\bf Sending share to all parties}: If $P_i \in S_q$, then execute the following steps.
	\begin{myenumerate}
	\item On having $[s]_q$, send $(\Share,\sid,q,[s]_q)$ to all the parties in $\PartySet \setminus S_q$.
	\end{myenumerate} 
%----
\item {\bf Computing output}: Based on the following conditions, execute the corresponding steps.
	\begin{myenumerate}
	\item {\bf $P_i \in S_q$}: Output $[s]_q$. %$(\recShare,\sid,q,[s]_q)$
	\item {\bf $P_i \notin S_q$}: Upon receiving $(\Share, \sid, q, v)$ from a set of parties $S'_q \subseteq S_q$ such that
	$S_q \setminus S'_q \in \AdvStructure$, output $[s]_q = v$.
	%---
	% in $S_q \setminus Z$ for some $Z \in \AdvStructure$, set $[s]_q = v$ and output $(\recShare,\sid,q,[s]_q)$
	\end{myenumerate} 
\end{myitemize}
%----
\end{protocolsplitbox}
%----

\begin{lemma}
%----
\label{lemma:PerRecShare}
%----
Let $\AdvStructure$ be an adversary structure and let $\ShareSpec = (S_1, \ldots, S_h)$ be a sharing specification, such that 
 $\ShareSpec$ satisfies the
 $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition. Moreover, let $s$ be a value, which is secret-shared as per $\ShareSpec$.
  Then for every $q \in \{1, \ldots, h \}$ and every adversary $\Adv$ corrupting a set of parties $Z^{\star} \in \AdvStructure$,
   all honest parties eventually output the share $[s]_q$ in the protocol $\PiPerRecShare$.
   The protocol incurs a communication of $\Order(n^2 \log{|\F|})$ bits.   
%----
\end{lemma}
%----
\begin{proof}
%----
Consider an arbitrary {\it honest} party $P_i \in \PartySet$. We consider two cases.
\begin{itemize}
%----
\item[--] $P_i \in S_q$: In this case, $P_i$ outputs $[s]_q$.
%----
\item[--] $P_i \notin S_q$: In this case, $P_i$ waits for a subset of parties $S'_q \subseteq S_q$ where $S_q \setminus S'_q \in \AdvStructure$, such that
      every party $P_j \in S'_q$ has sent the {\it same} share $v$ to $P_i$.
      If $P_i$ finds such a set $S'_q$, then it outputs $v$.
      To complete the proof, we need to show that $P_i$ will eventually find such a set $S'_q$
      and if such a set $S'_q$ is found by $P_i$, then the common $v$ is the same as $[s]_q$.
      
      Assuming that $P_i$ eventually finds such a common $S'_q$, the proof that the common $v$ is the same as $[s]_q$
      follows from the fact that $S'_q$ is guaranteed to contain at least one {\it honest} party from $S_q$, who would have sent the share
      $[s]_q$ to $P_i$. This is because the $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition is satisfied.
      Also, since the $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition is satisfied, the set of {\it honest} parties in $S_q$, namely the parties in 
      $S_q \setminus Z^{\star}$, always constitute a candidate $S'_q$ set. This is because every party $P_j \in S_q \setminus Z^{\star}$
      would have sent $[s]_q$ to $P_i$ and these values are eventually delivered to $P_i$. 
%----
\end{itemize}
%----
The communication complexity follows easily from the protocol steps.
%--
\end{proof}
%----

We now present the protocol $\PiPerRec$ (Fig \ref{fig:PerRec}), which allows {\it all} parties in $\PartySet$ to reconstruct a secret shared value $s$.
  The idea is simply to run an instance of $\PiPerRecShare$ for each $S_q \in \ShareSpec$, and to sum up the shares obtained as the
   output from each instantiation. 
%----
\begin{protocolsplitbox}{$\PiPerRec$}{Perfectly-secure reconstruction protocol for session id $\sid$ to reconstruct a shared value $s$. The public inputs of the protocol are $\PartySet, \ShareSpec$
  and $\AdvStructure$. The above steps are executed by every $P_i \in \PartySet$}{fig:PerRec}
%----
\justify
%----

\begin{myitemize}
%----
\item {\bf Reconstructing Shares}: For each $S_q \in \ShareSpec$, participate
 in an instance $\PiPerRecShare(q)$ with $\sid$ to obtain the output $[s]_q$.
%----
\item {\bf Output Computation}: Output $s = \displaystyle \sum_{S_q \in \ShareSpec} [s]_q$.
%----
\end{myitemize}
%----
\end{protocolsplitbox}
%----

The properties of the protocol $\PiPerRec$ are stated in Lemma \ref{lemma:PerRec}, which simply follows from the protocol steps and Lemma \ref{lemma:PerRecShare}.
%---
\begin{lemma}
%----
\label{lemma:PerRec}
%----
Let $\AdvStructure$ be an adversary structure and let $\ShareSpec = (S_1, \ldots, S_h)$ be a sharing specification, such that 
 $\ShareSpec$ satisfies the
 $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition.
  Moreover, let $s$ be a value, which is secret-shared as per $\ShareSpec$.
  Then for every adversary $\Adv$ corrupting a set of parties $Z^{\star} \in \AdvStructure$,
   all honest parties eventually output $s$ in the protocol $\PiPerRecShare$.
   The protocol incurs a communication of $\Order(|\ShareSpec| \cdot n^2 \log{|\F|})$ bits.   
%----
\end{lemma}
%----
\subsection{Properties of the Protocol $\OptMult$}
%---
In this section, we formally prove the properties of the protocol $\OptMult$ (see Fig \ref{fig:OptMult} for the formal description of the protocol). 
 While proving these properties, we will assume that  $\AdvStructure$ satisfies the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition.
  This further implies that the sharing specification $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$
  satisfies the $\Q^{(3)}(\ShareSpec, \AdvStructure)$ condition. 
  Moreover, while proving these properties, we also assume that for every $\iter$, 
  no honest party is ever included in the set $\Discarded$ and 
  all honest parties are eventually removed from the $ \Waitlist^{(i)}_{\iter'}, \LocalDiscarded^{(i)}_{\iter'}$ sets of every honest $P_i$ for every
  $\iter' < \iter$. Note that, these conditions regarding $\Discarded$ and 
  $ \Waitlist^{(i)}_{\iter'}, \LocalDiscarded^{(i)}_{\iter'}$ are ensured in the protocol $\MultLCE$ and $\MultGCE$ (where these sets are constructed and managed),
   where  $\OptMult$ is used as a subprotocol. 
  %----
  \begin{claim}
  \label{claim:OptMultAdvCondition}
  %----
 For every $Z \in \AdvStructure$ and every ordered pair $(p, q) \in \{1, \ldots, h \} \times \{1, \ldots, h \}$,
  the set $(S_p \cap S_q) \setminus Z$ contains at least one honest party.
  %----
  \end{claim}
  %-----
  \begin{proof}
  %----
  From the definition of the sharing specification $\ShareSpec$, we have
   $S_p = \PartySet \setminus Z_p$ and $S_q = \PartySet \setminus Z_q$, where $Z_p, Z_q \in \AdvStructure$. 
   Let $Z^{\star} \in \AdvStructure$ be the set of corrupt parties during the protocol $\OptMult$.
   If $(S_p \cap S_q) \setminus Z$ {\it does not} contain any honest party, then it implies that
   $((S_p \cap S_q) \setminus Z) \subseteq Z^{\star}$.
  This further implies that   $\PartySet \subseteq Z_p \cup Z_q \cup Z \cup Z^{\star}$, implying that 
   $\AdvStructure$ {\it does not} satisfy the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition, which is a contradiction.
  %---
  \end{proof}
%---
\begin{claim}
  \label{claim:OptMultACS}
  %----
 For every $Z \in \AdvStructure$, if all honest parties participate during the hop number $\hop$ in the protocol $\OptMult$, then
 all honest parties eventually obtain a common summand-sharing party, say $P_j$, for this hop, such that the honest parties
  will eventually hold $[c^{(j)}_{(Z, \iter)}]$. Moreover, party $P_j$ will be distinct from the summand-sharing party
   selected for any hop number $\hop' < \hop$.
  %----
  \end{claim}
  %-----
  \begin{proof}
  %---
  Since all honest parties participate in hop number $\hop$, it follows that 
  $\Products_{(Z, \iter)} \neq \emptyset$ at the beginning of hop number $\hop$. This implies that there exists at least one ordered pair $(p, q) \in \Products_{(Z, \iter)}$.
   From Claim \ref{claim:OptMultAdvCondition}, 
    there exists at least one {\it honest} party in $(S_p \cap S_q) \setminus Z$, say $P_k$, who will have both the shares 
  $[a]_p$ as well as $[b_q]$ (and hence the summand $[a]_p [b]_q$). We also note that $P_k$ {\it would not} have been selected as the common summand-sharing 
  party in any previous $\hop' < \hop$, as otherwise $P_k$ would have already included the summand $[a]_p[b]_q$ in the sum $c^{(k)}_{(Z, \iter)}$ shared
  by $P_k$ during hop $\hop'$, implying that $(p, q) \not \in \Products_{(Z, \iter)}$. Now during the hop number $\hop$, party $P_k$
  will randomly secret-share the sum $c^{(k)}_{(Z, \iter)}$ by making a
  call to $\FVSS$  and every honest $P_i$ will eventually receive an output
   $(\Share, \sid_{\hop, k, \iter, Z}, P_k, \{ [c^{(k)}_{(Z, \iter)}]_q \}_{P_i \in S_q})$  from $\FVSS$
    with $\sid_{\hop, k, \iter, Z}$. 
 Moreover, $P_k$ {\it will not} be present in the set $\Discarded$
  and if $P_k$ is present in the sets $ \Waitlist^{(i)}_{\iter'}, \LocalDiscarded^{(i)}_{\iter'}$ of any honest $P_i$ for any
  $\iter' < \iter$, then it is eventually removed from these sets.
  
  We next claim that during the hop number $\hop$, there will at least one instance of $\FABA$, corresponding to which {\it all} honest parties
  eventually receive the output $1$. For this, we consider two possible cases:
  %----
  \begin{myitemize}
  %---
  \item[--] {\it At least one honest party participates with input $0$ in the $\FABA$ instance corresponding to $P_k$}: Let 
  $P_i$ be an {\it honest} party, who sends $(\vote, \sid_{\hop, k, \iter, Z}, 0)$ to $\FABA$ with 
  $\sid_{\hop, k, \iter, Z}$. Then from the steps of $\OptMult$, it follows that there exists some $P_j \in \PartySet$, such that
  $P_i$ has received
    $(\decide, \sid_{\hop, j, \iter, Z}, 1)$ as the output from $\FABA$ with  $\sid_{\hop, j, \iter, Z}$. Hence, {\it every} honest party
    will eventually receive the output $(\decide, \sid_{\hop, j, \iter, Z}, 1)$ as the output from $\FABA$ with  $\sid_{\hop, j, \iter, Z}$.
  %----
  \item[--] {\it No honest party participates with input $0$ in the $\FABA$ instance corresponding to $P_k$}:
  In this case, {\it every} honest party will eventually send $(\vote, \sid_{\hop, k, \iter, Z}, 1)$ to $\FABA$ with 
  $\sid_{\hop, k, \iter, Z}$ and eventually receives the output $(\decide, \sid_{\hop, k, \iter, Z}, 1)$ from $\FABA$. 
  %---
  \end{myitemize}
  %----
  Now based on the above claim, we can further claim that 
   all honest parties will eventually participate with some input in all the
  $n$ instances of $\FABA$ invoked during the hop number $\hop$
  and hence all the $n$ instances of $\FABA$ during the hop number $\hop$ will eventually produce an output.
  Since the summand-sharing party for hop number $\hop$   
  corresponds to the least indexed $\FABA$ instance in which all the honest parties obtain $1$ as the output,
   it thus follows that eventually the honest parties will select a summand-sharing party. Moreover, this summand-sharing party will be common,
  as it is based on the outcome of $\FABA$ instances.
  
  Let $P_j$ be the summand-sharing party for the hop number $\hop$.
   We next show that the honest parties will eventually hold $[c^{(j)}_{(Z, \iter)}]$.
   For this, we note that since $P_j$ has been selected as the summand-sharing party, {\it at least} one {\it honest} party, say
   $P_i$, must have sent $(\vote, \sid_{\hop, j, \iter, Z}, 1)$ to $\FABA$ with 
  $\sid_{\hop, j, \iter, Z}$. If not, then $\FABA$ with $\sid_{\hop, j, \iter, Z}$ will never produce the output
  $(\decide, \sid_{\hop, j, \iter, Z}, 1)$ and hence $P_j$ will not be the summand-sharing party for the hop number $\hop$.
  Now since $P_i$ sent $(\vote, \sid_{\hop, j, \iter, Z}, 1)$ to $\FABA$, it follows that
  $P_i$ has received an output $(\Share, \sid_{\hop, j, \iter, Z}, P_j, \{ [c^{(j)}_{(Z, \iter)}]_q \}_{P_i \in S_q})$  from $\FVSS$
    with $\sid_{\hop, j, \iter, Z}$. This implies that $P_j$ must have sent the message 
    $(\Dealer, \sid_{\hop, j, \iter, Z}, (c^{(j)}_{{(\iter, Z)}_1}, \ldots, c^{(j)}_{{(\iter, Z)}_h}))$ to
    $\FVSS$ with $\sid_{\hop, j, \iter, Z}$. 
    Consequently, every honest party will eventually receive their respective outputs from 
     $\FVSS$ with $\sid_{\hop, j, \iter, Z}$ and hence the honest parties will eventually hold
     $[c^{(j)}_{(Z, \iter)}]$.
     
     Finally, to complete the proof of the claim, we need to show that party $P_j$ is different from the summand-sharing parties selected
     during the hops $1, \ldots, \hop - 1$. If $P_j$ has been selected as a summand-sharing party for any hop number $\hop' < \hop$, then
     no honest party ever sends $(\vote, \sid_{\hop, j, \iter, Z}, 1)$ to $\FABA$ with 
  $\sid_{\hop, j, \iter, Z}$. Consequently, $\FABA$ with $\sid_{\hop, j, \iter, Z}$ will never send the output 
  $(\decide, \sid_{\hop, j, \iter, Z}, 1)$ to any honest party and hence $P_j$ will not be selected as the summand-sharing party
  for hop number $\hop$, which is a contradiction.
  %--
  \end{proof}
%----
\begin{claim}
  \label{claim:OptMultComplexity}
  %----
  In protocol $\OptMult$, all honest parties eventually obtain an output.
   The protocol makes $\Order(n^2)$ calls to $\FVSS$ and $\FABA$.
  %----
  \end{claim}
  %-----
  \begin{proof}
  %---
  From Claim \ref{claim:OptMultAdvCondition} and \ref{claim:OptMultACS}, it follows that the number of hops in the protocol 
   is $\Order(n)$, as in each hop a new summand-sharing party is selected and if all honest parties are included
   in the set of summand-sharing parties $\Selected_{(Z, \iter)}$, then $\Products_{(Z, \iter)}$ becomes $\emptyset$.
   The proof now follows from the fact that in each hop, there are $\Order(n)$ calls to $\FVSS$ and $\FABA$. 
  %---
  \end{proof}
  %---
  \begin{claim}
  \label{claim:OptMultCorrectness}
  %---
  In protocol $\OptMult$, if no party in $\PartySet \setminus Z$ behaves maliciously, then for each $P_i \in \Selected_{(Z, \iter)}$, the condition
   $c^{(i)}_{(Z, \iter)} = \sum_{(p, q) \in \Products^{(i)}_{(Z, \iter)}} [a]_p[b]_q$ holds and
   $c_{(Z, \iter)} = ab$. 
  %--
  \end{claim}
%----
  \begin{proof}
  %---
  From the protocol steps, it follows that $\Selected_{(Z, \iter)} \cap Z = \emptyset$, as no honest part ever votes for any party from $Z$ as a candidate
  summand-sharing party during any hop in the protocol.  
  Now since $\Selected_{(Z, \iter)} \subseteq (\PartySet \setminus Z)$, 
  if no party in $\PartySet \setminus Z$ behaves maliciously, then it implies that every party 
  $P_i \in \Selected_{(Z, \iter)}$ has behaved honestly and secret-shares $c^{(i)}_{(Z, \iter)}$ by calling $\FVSS$, where
  $c^{(i)}_{(Z, \iter)} = \sum_{(p, q) \in \Products^{(i)}_{(Z, \iter)}} [a]_p[b]_q$.
  Moreover, from the protocol steps, it follows that for every $P_j, P_k \in \Selected_{(Z, \iter)}$:
  %---
  \[ \displaystyle \Products^{(j)}_{(Z, \iter)} \cap \Products^{(k)}_{(Z, \iter)} = \emptyset.  \]
  %---
  To prove this, suppose $P_j$ and $P_k$ are included in $\Selected_{(Z, \iter)}$ during hop number $\hop_j$ and $\hop_k$ respectively, where
  without loss of generality, $\hop_j < \hop_k$. 
  Then from the protocol steps, during $\hop_j$, the parties would set
  $\Products^{(k)}_{(Z, \iter)} = \Products^{(k)}_{(Z, \iter)} \setminus \Products^{(j)}_{(Z, \iter)}$. This ensures that
  during $\hop_k$, there exists no ordered pair $(p, q) \in \{1, \ldots, |\ShareSpec| \} \times \{1, \ldots, |\ShareSpec| \}$, such that
  $(p, q) \in \Products^{(j)}_{(Z, \iter)} \cap \Products^{(k)}_{(Z, \iter)}$.
  
  Since all the parties $P_i \in \Selected_{(Z, \iter)}$ have behaved honestly, 
   from the protocol steps, it also follows that :
  %---
  \[ \displaystyle \bigcup_{P_i \in \Selected_{(Z, \iter)}} \Products^{(i)}_{(Z, \iter)} = \{ (p, q) \}_{p, q = 1, \ldots, |\ShareSpec|}. \]
  %---
  Finally, from the protocol steps, it follows that 
   $\forall P_j \in \PartySet \setminus \Selected_{(Z, \iter)}$, the condition
  $c^{(j)}_{(Z, \iter)} = 0$ holds. Now since $c_{(Z, \iter)} =  c^{(1)}_{(Z, \iter)} + \ldots + c^{(n)}_{(Z, \iter)}$, it follows that
  if no party in $\PartySet \setminus Z$ behaves maliciously, then $c_{(Z, \iter)} = ab$. 
  %---
  \end{proof}
%-----
\noindent {\bf Lemma \ref{lemma:OptMult}.}
%----
{\it Let  $\AdvStructure$ satisfy the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition. Then
 for every $Z \in \AdvStructure$ and $\iter$, 
 the parties eventually compute  $[c_{(Z, \iter)}]$ and $([c^{(1)}_{(Z, \iter)}], \ldots, [c^{(n)}_{(Z, \iter)}])$ in $\OptMult$ 
 where $c_{(Z, \iter)} = c^{(1)}_{(Z, \iter)} + \ldots + c^{(n)}_{(Z, \iter)}$, 
  provided no honest party is ever included in the $\Discarded$ and $\LocalDiscarded^{(i)}_{\iter'}$ sets 
  and all honest parties are eventually removed from the $ \Waitlist^{(i)}_{\iter'}$ sets of every honest $P_i$ for every
  $\iter' < \iter$. If no party in $\PartySet \setminus Z$ behaves maliciously, then for all $P_i \in \Selected_{(Z, \iter)}$, the condition
   $c^{(i)}_{(Z, \iter)} = \sum_{(p, q) \in \Products^{(i)}_{(Z, \iter)}} [a]_p[b]_q$ holds and
   $c_{(Z, \iter)} = ab$. The protocol makes $\Order(n^2)$ calls to $\FVSS$ and $\FABA$}.
%----
\begin{proof}
%----
The proof follows from Claims \ref{claim:OptMultAdvCondition}-\ref{claim:OptMultCorrectness}.
%---
\end{proof}
%----
\subsection{Properties of the Protocol $\MultLCE$}
%---
In this section, we formally prove the properties of the protocol $\MultLCE$ (see Fig \ref{fig:MultLCE} for the formal description of the protocol). 
 While proving these properties, we will assume that  $\AdvStructure$ satisfies the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition.
  This further implies that the sharing specification $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$
  satisfies the $\Q^{(3)}(\ShareSpec, \AdvStructure)$ condition. Moreover, we will also assume that {\it no} honest party is ever included
  in the set $\Discarded$, which will be guaranteed in the protocol $\MultGCE$, where the set $\Discarded$ is constructed is managed and where
  $\MultLCE$ is used as a sub-protocol. 
  
  We next give the definition of a {\it successful} $\MultLCE$ instance, which will be used
  throughout this and next section.
  
   \begin{definition}
  \label{def:MultGCE}
  %---
  For an instance $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$, we define the following.
  %----
  \begin{myitemize}
  %----
  \item[--] The instance is called {\it successful} if and only if 
   for every $Z \in \AdvStruct$, the value $c_{(Z, \curr)} - c_{(Z', \curr)} = 0$, where $Z' \in \AdvStructure$ is the fixed
   set used in the protocol.  
  %---
   \item[--] If the instance is not successful, then the sets $Z, Z'$ are called the {\it conflicting-set} for the instance,
   if $Z$ is the smallest indexed set from $\AdvStructure$ such that $c_{(Z, \curr)} - c_{(Z', \curr)} \neq 0$.
   %---
  \end{myitemize}
  \end{definition} 
  %---
  
   We first show that any instance of $\MultLCE$ will be eventually found to be either successful or a failure by the honest parties. 
  %---
    \begin{claim}
   \label{claim:MultLCETermination}
   %----
For every $\iter$, any instance $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$
 will eventually be deemed to succeed or fail by the honest parties, 
  provided no honest party is ever included in the $\Discarded$ and $\LocalDiscarded^{(i)}_{\iter'}$ sets 
  and all honest parties are eventually removed from the $ \Waitlist^{(i)}_{\iter'}$ sets of every honest $P_i$ for every
  $\iter' < \iter$.
   Moreover, for a 
  successful
  instance, the parties output a sharing of $ab$, while if the instance is not successful, then 
   the parties identify the  {\it conflicting-sets} $Z, Z'$ for the instance.
  %----
  \end{claim}
  %----
  \begin{proof}
  %----
  Let $Z^{\star} \in \AdvStructure$ be the set of corrupt parties. If the lemma conditions hold, then
   it follows from 
    Lemma \ref {lemma:OptMult}, that corresponding to every $Z \in \AdvStructure$, the instance $\OptMult(\PartySet, \AdvStruct, \SharingSpec,[a], [b], Z, \iter)$ 
 eventually completes with honest parties obtaining the outputs $[c^{(1)}_{(Z, \iter)}] , \ldots, [c^{(n)}_{(Z, \iter)}], [c_{(Z, \iter)}]$, where
 $c_{(Z, \iter)} = c^{(1)}_{(Z, \iter)} + \ldots + c^{(n)}_{(Z, \iter)}$. Moreover, in the $\OptMult$ instance corresponding to $Z^{\star}$,
 the output $c_{(Z^{\star}, \iter)}$ will be the same as $ab$, since all the parties in $\PartySet \setminus Z^{\star}$ will be honest.
 
 Since $\ShareSpec$ satisfies the $\Q^{(3)}(\ShareSpec, \AdvStructure)$ condition, it follows that with respect to the fixed
  $Z' \in \AdvStruct$, the honest parties will eventually reconstruct the difference $c_{(Z, \curr)} - c_{(Z', \curr)}$, corresponding to {\it every}
  $Z \in \AdvStructure$. Now there are two possibilities. If all the differences $c_{(Z, \curr)} - c_{(Z', \curr)}$ turn out to be $0$, then 
  the $\MultLCE$ instance will be considered as successful by the honest parties and the honest parties will output
  $[c_{(Z', \iter)}]$, which is bound to be the same as $ab$. This is because $c_{(Z', \iter)} - c_{(Z^{\star}, \iter)} = 0$ and hence
  $c_{(Z', \iter)} = c_{(Z^{\star}, \iter)} = ab$ holds. The other possibility is that all the differences are {\it not} zero, in which case
  the instance $\MultLCE$ will not be considered as successful by the honest parties. Moreover, in this case, the parties will set
  $(Z, Z')$ as the conflicting set for the instance, where $Z$ is the smallest indexed set from $\AdvStructure$ such that $c_{(Z, \curr)} - c_{(Z', \curr)} \neq 0$.
  %---
  \end{proof}
%----    

    We next prove a series of claims regarding any $\MultLCE$ instance, which is {\it not} successful. 
    We begin by showing that 
    if any instance of $\MultLCE$ is {\it not} successful, then every honest party in eventually removed from the waiting-list
  of the honest parties for that instance. Moreover, no honest party will be ever included in the $\LocalDiscarded$ set of any honest party.
  %-----
   \begin{claim}
   \label{claim:MultLCEHonestPartyParticipation}
   %----
   For every $\iter$, if the instance $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$ is not successful, then 
   every honest party from the set $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ is eventually removed from the waiting list
      $\Waitlist^{(i)}_{\iter}$ of every honest party $P_i$. Moreover, no honest party is ever included
      in the $\LocalDiscarded^{(i)}_{\iter}$ set of any honest party $P_i$.
    %--- 
      \end{claim}
  %-----
  \begin{proof}
  %---
  Let the instance $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$ is not successful. This implies that the parties identify
  a pair of conflicting-sets $(Z, Z')$, such that $c_{(Z, \curr)} - c_{(Z', \curr)} \neq 0$. From the protocol steps, every honest party
  $P_i$ initializes $\Waitlist^{(i)}_{\iter}$ to  $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$. Let $P_j$ be an arbitrary 
  {\it honest} party belonging to $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$. From the protocol steps, 
  party $P_j$ secret-shares all the required values $d^{(jk)}_{(Z, \iter)}, e^{(jk)}_{(Z', \iter)}$ by calling appropriate instances of $\FVSS$
  and eventually these values are secret-shared, with every honest $P_i$ receiving the appropriate shares
  from corresponding $\FVSS$ instances. Consequently, $P_j$ will be eventually received from the set $\Waitlist^{(i)}_{\iter}$.
    Moreover, since $P_j$ is an {\it honest} party, the $d^{(jk)}_{(Z, \iter)}, e^{(jk)}_{(Z', \iter)}$ values shared
  by $P_j$ will be correct and consequently, the conditions for including $P_j$ to the $\LocalDiscarded^{(i)}_{\iter}$ 
  set of any honest party $P_i$ will fail. That is, if $P_j \in \Selected_{(Z, \iter)}$, then the parties will find that 
                  $\displaystyle c^{(j)}_{(Z, \iter)} - \sum_{P_k \in \Selected_{(Z', \iter)}} d^{(jk)}_{(Z, \iter)} = 0$.
   On the other hand, if $P_j \in \Selected_{(Z', \iter)}$, then the parties will find that
                $\displaystyle c^{(j)}_{(Z', \iter)} - \sum_{P_k \in \Selected_{(Z, \iter)}} e^{(jk)}_{(Z', \iter)} = 0$.
   Moreover, if there exists any $P_k \in \Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ such that
   either $d^{(jk)}_{(Z, \iter)} \neq e^{(kj)}_{(Z', \iter)}$ or $d^{(kj)}_{(Z, \iter)} \neq e^{(jk)}_{(Z', \iter)}$, 
   then after reconstructing the values shared by $P_j$ and the shares held by $P_j$, the parties
   will find that $P_j$ has behaved honestly and hence $P_j$ will not be included to the  
    $\LocalDiscarded^{(i)}_{\iter}$ set of any honest $P_i$. 
  %---
  \end{proof}

We next prove an important property by showing that if any instance of $\MultLCE$ is {\it not} successful, then 
 there exists at least one pair of {\it conflicting-parties} $P_j, P_k$, with one
  of them being corrupt, such that
  if both $P_j$ and $P_k$ are removed from the waiting-list of the honest parties, then all honest parties eventually identify the corrupt parties among
  $P_j$ and $P_k$.
  %----
  \begin{claim}
  \label{claim:MultLCECheaterIdentification}
  %---
  Let $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$ be an instance of $\MultLCE$ which  is not successful and let
   $Z, Z'$ be the corresponding conflicting-sets for the instance. Then there exists at least one pair of parties
   $P_j, P_k \in \Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$, with one of them being {\it maliciously-corrupt}, 
   such that if both
  $P_j$ and $P_k$ are removed from the set $\Waitlist^{(i)}_{\iter}$ of {\it any} honest party $P_i$, then eventually
  the corrupt party(ies) among $P_j, P_k$ will be eventually included
        in the set $\LocalDiscarded^{(i)}_{\iter}$ of {\it every} honest $P_i$.        
  %---
  \end{claim} 
  %----
  \begin{proof}
  %---
  Since the instance $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$ is not successful
  and  $Z, Z'$ are the corresponding conflicting-sets for the instance, 
    the outputs $c_{(Z, \iter)}$ and $c_{(Z', \iter)}$ in the corresponding $\OptMult$ instances are not the same; i.e.~$c_{(Z', \iter)} - c_{(Z^{\star}, \iter)} \neq 0$.
  Hence, there exists at least one {\it maliciously-corrupt} party in the set $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$. This is because if no
  summand-sharing party in $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ behaved maliciously, then from Lemma \ref{lemma:OptMult}, 
  $c_{(Z', \iter)} = c_{(Z^{\star}, \iter)} = ab$ and hence $c_{(Z', \iter)} - c_{(Z^{\star}, \iter)} = 0$, which is a contradiction. 
  Also from the protocol steps, the waiting-list  $\Waitlist^{(i)}_{\iter}$ of every {\it honest} party $P_i$ is initialized to 
  $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ and hence all {\it corrupt} parties in $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ will be included
   in $\Waitlist^{(i)}_{\iter}$. 
   
  Since $c_{(Z', \iter)} - c_{(Z^{\star}, \iter)} \neq 0$, it follows that the following holds:
  %---
  \[\displaystyle \sum_{P_j \in \Selected_{(Z, \iter)}} c^{(j)}_{(Z, \iter)} \neq \sum_{P_j \in \Selected_{(Z', \iter)}} c^{(j)}_{(Z', \iter)}.   \]
  %---
  Next, consider an {\it arbitrary} $P_j \in \Selected_{(Z, \iter)}$ and corresponding to $P_j$, let
   $\bard^{(jk)}_{(Z, \iter)}$ be the partition of the summand $c^{(j)}_{(Z, \iter)}$, which supposedly overlaps with summand 
   $c^{(k)}_{(Z', \iter)}$ corresponding to the party $P_k \in \Selected_{(Z', \iter)}$.
   That is, for every $P_j \in \Selected_{(Z, \iter)}$ and every $P_k \in \Selected_{(Z', \iter)}$
   %--
     \[ \displaystyle \bard^{(jk)}_{(Z, \iter)} \defined \sum_{(p, q) \in \Products^{(j)}_{(Z, \iter)} \cap \Products^{(k)}_{(Z', \iter)}} [a]_p [b]_q + \error^{(jk)}_{(Z, \iter)},  \]
   %----
    where $[a]_p [b]_q + \error^{(jk)}_{(Z, \iter)}$ are the summands used by $P_j$ for computing $c^{(j)}_{(Z, \iter)}$
       during the instance
      $\OptMult(\PartySet, \AdvStruct, \SharingSpec,[a], [b], Z, \iter)$ and where each $\error^{(jk)}_{Z, \iter} = 0$ for an 
      {\it honest} $P_j$. Hence for each $P_j \in \Selected_{(Z, \iter)}$,
      %----
      \[ \displaystyle c^{(j)}_{(Z, \iter)} = \sum_{P_k \in \Selected_{(Z', \iter)}} \bard^{(jk)}_{(Z, \iter)}, \]
     %----
     where $\displaystyle c^{(j)}_{(Z, \iter)} = \sum_{(p, q) \in \Products^{(j)}_{(Z, \iter)}} [a]_p [b]_q  $ holds for every
     {\it honest} $P_j \in \Selected_{(Z, \iter)}$.
  %---
  
  Similarly, for every $P_j \in \Selected_{(Z', \iter)}$ and every $P_k \in \Selected_{(Z, \iter)}$, let 
   $\bare^{(jk)}_{(Z', \iter)}$ be the partition of the summand $c^{(j)}_{(Z', \iter)}$, which supposedly overlaps with summand 
   $c^{(k)}_{(Z, \iter)}$ corresponding to the party $P_k \in \Selected_{(Z, \iter)}$. That is, 
    %--
     \[ \displaystyle \bare^{(jk)}_{(Z', \iter)} \defined \sum_{(p, q) \in \Products^{(j)}_{(Z', \iter)} \cap \Products^{(k)}_{(Z, \iter)}} [a]_p [b]_q + \error^{(jk)}_{Z', \iter},  \]
   %----
    where $[a]_p [b]_q + \error^{(jk)}_{Z', \iter}$ are the summands used by $P_j$ for computing $c^{(j)}_{(Z', \iter)}$
       during the instance
      $\OptMult(\PartySet, \AdvStruct, \SharingSpec,[a], [b], Z', \iter)$ and where each $\error^{(jk)}_{Z', \iter} = 0$ for an 
      {\it honest} $P_j$. Hence for each $P_j \in \Selected_{(Z', \iter)}$,
      %----
      \[ \displaystyle c^{(j)}_{(Z', \iter)} = \sum_{P_k \in \Selected_{(Z, \iter)}} \bare^{(jk)}_{(Z', \iter)}, \]
     %----
     where $\displaystyle c^{(j)}_{(Z', \iter)} = \sum_{(p, q) \in \Products^{(j)}_{(Z', \iter)}} [a]_p [b]_q  $ holds for every
     {\it honest} $P_j \in \Selected_{(Z', \iter)}$.
     %---
     
     Now since $\displaystyle \sum_{P_j \in \Selected_{(Z, \iter)}} c^{(j)}_{(Z, \iter)} \neq \sum_{P_j \in \Selected_{(Z', \iter)}} c^{(j)}_{(Z', \iter)}$, it
     follows that there exists at least one pair of {\it conflicting-parties} $P_j, P_k \in \Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$, such that
     one of the following holds:
     %----
     \begin{myitemize}
     %---
     \item[--] $P_j \in \Selected_{(Z, \iter)}$, $P_k \in \Selected_{(Z', \iter)}$ and $\bard^{(jk)}_{(Z, \iter)} \neq \bare^{(kj)}_{(Z', \iter)}$.
     %---
     \item[--] $P_j \in \Selected_{(Z', \iter)}$, $P_k \in \Selected_{(Z, \iter)}$ and $\bard^{(kj)}_{(Z, \iter)} \neq \bare^{(jk)}_{(Z', \iter)}$. 
     %----
     \end{myitemize}
     %----
     
     It is easy to see that at least one party among $P_j$ and $P_k$ is {\it maliciously-corrupt}. Next suppose
     that both $P_j$ and $P_k$ are removed from the set $\Waitlist^{(i)}_{\iter}$ of some {\it honest} party $P_i$.
     To complete the proof, we want to show that the corrupt party(ies) among $P_j, P_k$ will be eventually
     included in the $\LocalDiscarded^{(i)}_{\iter}$ of {\it every} honest $P_i$. 
     For simplicity and without loss of generality, let
     $P_j \in \Selected_{(Z, \iter)}$, $P_k \in \Selected_{(Z', \iter)}$ and $\bard^{(jk)}_{(Z, \iter)} \neq \bare^{(kj)}_{(Z', \iter)}$.
     
     Since $P_i$ has removed both $P_j$ as well as $P_k$ from $\Waitlist^{(i)}_{\iter}$
     
     
     
     
       
  %---

  
  
  \end{proof}
   
  
  Moreover, in the latter case, the corrupt summand-sharing parties corresponding to the conflicting $\OptMult$ instances
  will be wait-listed, till they participate in the cheater-identification phase by secret-sharing the required values.
  Furthermore, if they do so, then it will either lead to the identification of some corrupt parties or lead to at least one conflicting-pair of parties
   where the corrupt party in the pair is identified as a cheater, if the other party in the pair participates in the cheater-identification phase.
  %---  
  \begin{claim}
   \label{claim:MultLCETermination}
   %----
For every $\iter$, the following holds during the instance $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$, provided no honest
 party is every included in the set $\Discarded$.
%---
\begin{myitemize}
 %----
 \item[(a).] The instance  will eventually be deemed to succeed or fail by the honest parties, where for a successful
  instance, the parties output a sharing of $ab$.
 %---
 \item[(b).] If the instance is not successful, then the honest parties 
  will set some $(Z, Z')$ as the conflicting-sets, such that the set $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$
  will contain at least one corrupt party. 
  Moreover, if any maliciously-corrupt $P_j \in \Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ is included in
  the set $\Selected_{(Z'', \iter')}$ for any $Z'' \in \AdvStructure$
     and $\iter' > \iter$ during an instance $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter')$, then it implies that there exists at least
     one honest party $P_i$, such that $P_j$ has  been removed from $\Waitlist^{(i)}_{\iter}$. Furthermore, in this case, at least one of the following will hold:
     %----
        \begin{myenumerate}
        %----
        \item[i.] Either $\displaystyle c^{(j)}_{(Z, \iter)} - \sum_{P_k \in \Selected_{(Z', \iter)}} d^{(jk)}_{(Z, \iter)} \neq 0$ or 
        $\displaystyle c^{(j)}_{(Z', \iter)} - \sum_{P_k \in \Selected_{(Z, \iter)}} e^{(jk)}_{(Z', \iter)} \neq 0$ will hold
        and $P_j$ will be eventually included
        in the $\LocalDiscarded^{(i)}_{\iter}$ set of every honest $P_i$.
        %---
        \item[ii.] There will be at least one conflicting-pair of parties, say $(P_j, P_k)$, for the instance 
        $\MultLCE(\PartySet, \allowbreak \AdvStruct, \SharingSpec, [a], [b], \iter)$.\footnote{See Definition \ref{def:MultGCE} for the definition of conflicting-pair of parties.}
        Furthermore, if $P_k$ is removed from $\Waitlist^{(i)}_{\iter}$ of any honest $P_i$, then $P_j$ will be eventually included
        in the list $\LocalDiscarded^{(i)}_{\iter}$ of every honest $P_i$.        
        %---
        \end{myenumerate}
 %----
 \end{myitemize}
%---
\end{claim}
%----
\begin{proof}
%---
This proves the part (a) of the claim.
  
 Next, let us consider the case when the instance $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$ is not successful. 
  In this case, the parties will find a pair of {\it conflicting-sets} $(Z, Z')$, such that
  the outputs $c_{(Z, \iter)}$ and $c_{(Z', \iter)}$ in the corresponding $\OptMult$ instances are not the same; i.e.~$c_{(Z', \iter)} - c_{(Z^{\star}, \iter)} \neq 0$.
  Clearly, in this case there exists at least one corrupt party in the set $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$. This is because if no
  summand-sharing party in $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ behaved maliciously, then from Lemma \ref{lemma:OptMult}, 
  $c_{(Z', \iter)} = c_{(Z^{\star}, \iter)} = ab$ and hence $c_{(Z', \iter)} - c_{(Z^{\star}, \iter)} = 0$, which is a contradiction. 
  Also from the protocol steps, the waiting-list  $\Waitlist^{(i)}_{\iter}$ of every {\it honest} party $P_i$ is initialized to 
  $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ and hence all {\it corrupt} parties in $\Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$ will be included
   in $\Waitlist^{(i)}_{\iter}$. 
  
  Next, consider a {\it maliciously}-corrupt $P_j \in \Selected_{(Z, \iter)} \cup \Selected_{(Z', \iter)}$, such that
  $P_j$ is selected as a summand-sharing party and included in the set  $\Selected_{(Z'', \iter')}$ corresponding to some 
  $Z'' \in \AdvStructure$
    during an instance 
  $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter')$, where $\iter' > \iter$. 
  This implies that during the instance $\OptMult(\PartySet, \AdvStruct, \SharingSpec, [a], [b], Z'', \iter')$ in
   $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter')$,
  party $P_j$ is selected as a summand-sharing party during one of the hops, say $\hop$,  and included in 
  the set  $\Selected_{(Z'', \iter')}$. This implies that during the hop number $\hop$, at least one {\it honest}
  party, say $P_i$, sends the message $(\vote, \sid_{\hop, j ,\iter', Z''}, 1)$ to $\FABA$ with $\sid_{\hop, j, \iter', Z''}$ while 
  voting for candidate summand-sharing party. If not, then $\FABA$ with $\sid_{\hop, j, \iter', Z''}$ will never
  return the output $(\decide, \sid_{\hop, j, \iter', Z''}, 1)$ for any honest party and consequently, $P_j$ will not be included in 
  $\Selected_{(Z'', \iter')}$, which is a contradiction. Now from the protocol steps, since 
  $P_i$ sends the message $(\vote, \sid_{\hop, j ,\iter', Z''}, 1)$ to $\FABA$, it implies that
  $P_i$ has removed  $P_j$ from $\Waitlist^{(i)}_{\iter}$ and sets
  $\Waitlist^{(i)}_{\iter} = \Waitlist^{(i)}_{\iter} \setminus \{P_j \}$. Then from the steps of $\MultLCE$, 
  the following conditions also hold for $P_i$ before $P_j$ is removed by $P_i$ from $\Waitlist^{(i)}_{\iter}$.
  %---
    \begin{myenumerate}
		%----
		\item \textbf{If $P_j \in \Selected_{(Z, \iter)}$ and $P_j \notin \Selected_{(Z', \iter)}$}: In this case, 
		corresponding to every $P_k \in \Selected_{(Z', \iter)}$, party $P_i$ receives 
		an output $(\Share, \sid_{j, k, \iter, Z}, P_j, \{ [d^{(jk)}_{(Z, \iter)}]_q \}_{P_i \in S_q})$ from $\FVSS$ with session id
		$\sid_{j, k, \iter, Z}$. Consequently, every honest party eventually receives an output from this $\FVSS$ instance,
		 implying that the honest parties eventually hold $[d^{(jk)}_{(Z, \iter)}]$.		
		%----
		\item \textbf{If $P_j \notin \Selected_{(Z, \iter)}$ and $P_j \in \Selected_{(Z', \iter)}$}: In this case, corresponding to every $P_k \in \Selected_{(Z, \iter)}$,
		party $P_i$ receives an output $(\Share, \sid_{j, k,  \iter, Z'}, P_j, \{ [e^{(jk)}_{(Z', \iter)}]_q \}_{P_i \in S_q})$ 
		from $\FVSS$ with session id
		$\sid_{j, k, \iter, Z'}$. Consequently, every honest party eventually receives an output from this $\FVSS$ instance,
		 implying that the honest parties eventually hold $[e^{(jk)}_{(Z', \iter)}]$.			
		%----
		\item \textbf{If $P_j \in \Selected_{(Z, \iter)}$ and $P_j \in \Selected_{(Z', \iter)}$}: In this case,
		corresponding to every $P_k \in \Selected_{(Z, \iter)}$ and every
		$P_{\ell} \in \Selected_{(Z', \iter)}$,
		party $P_i$ receives an output $(\Share, \sid_{j, k, \iter, Z}, P_j, \allowbreak \{ [d^{(jk)}_{(Z, \iter)}]_q \}_{P_i \in S_q})$ 
		and $(\Share, \allowbreak \sid_{j, \ell, \iter, Z'}, P_j, \{ [e^{(j \ell)}_{(Z', \iter)}]_q \}_{P_i \in S_q})$
		from $\FVSS$ with session id
		$\sid_{j, k, \iter, Z}$ and $\sid_{j, \ell, \iter, Z'}$ respectively. Consequently, every honest party eventually receives an output from these
		$\FVSS$ instances, implying that the honest parties eventually hold 	$[d^{(jk)}_{(Z, \iter)}]$ and 	
		$[e^{(j \ell)}_{(Z', \iter)}]$.
		%----
		\end{myenumerate}
              %-------
   Thus, all the values which are supposed to be secret-shared by $P_j$ during the cheater-identification phase of the instance 
    $\MultLCE(\PartySet, \AdvStruct, \SharingSpec, [a], [b], \iter)$ will be eventually secret-shared and consequently, 
    $P_j$ will be removed from the waiting-list $\Waitlist^{(i)}_{\iter}$ of {\it all} honest parties $P_i$. Next, we claim that at least one of the following will
    hold, with respect to $P_j$.
    %----
      \begin{myenumerate}
      %---
      \item[i.] \textbf{If $P_j \in \Selected_{(Z, \iter)}$ and $P_j \notin \Selected_{(Z', \iter)}$}: Then 
       $\displaystyle c^{(j)}_{(Z, \iter)} - \sum_{P_k \in \Selected_{(Z', \iter)}} d^{(jk)}_{(Z, \iter)} \neq 0$.
       %---
       \item[ii.] \textbf{If $P_j \notin \Selected_{(Z, \iter)}$ and $P_j \in \Selected_{(Z', \iter)}$}: Then
               $\displaystyle c^{(j)}_{(Z', \iter)} - \sum_{P_k \in \Selected_{(Z, \iter)}} e^{(jk)}_{(Z', \iter)} \neq 0$.
       %---        
        \item[iii.] \textbf{If $P_j \in \Selected_{(Z, \iter)}$ and $P_j \in \Selected_{(Z', \iter)}$}: Then
        there will be at least one conflicting-pair of parties, say $(P_j, P_k)$.
      %---
      \end{myenumerate}     
    %----
    On contrary, if neither of the above $3$ conditions holds with respect to $P_j$, then it implies that $c_{(Z', \iter)} - c_{(Z^{\star}, \iter)} = 0$, which is a contradiction, since
     $(Z, Z')$ constitutes a pair of {\it conflicting-sets}.
  
  

%--
\end{proof}  




\subsection{The Perfectly-Secure AMPC Protocol}
%---
The perfectly-secure AMPC protocol in the $(\FTriples, \FVSS, \FABA)$-hybrid model is presented in Fig \ref{fig:PerAMPC}. The high level idea behind the protocol
 has been already discussed in Section \ref{sec:PerAMPC}. 
  The protocol has a {\it pre-processing} phase where secret-shared random multiplication triples are generated, an
  {\it input} phase, where each party verifiably generates a secret-sharing of its input for the function and a common subset of input-providers
  is selected and a {\it circuit-evaluation} phase where the circuit is securely evaluated and the function output is publicly reconstructed.
  
   In the protocol, all honest parties may not be reconstructing the function-output at the same ``time" and
   different parties may be at different phases of the protocol, as the protocol is executed asynchronously. Consequently, a party upon reconstructing the function-output
   {\it cannot} afford to terminate immediately, as its presence and participation might be needed for the completion of various phases of the protocol by other honest parties.
   A standard trick to get around this problem in the AMPC protocols \cite{HNP05,HNP08,Coh16}
    is to have an additional {\it termination phase}, whose code is executed concurrently throughout the protocol to check if a party can ``safely" terminate the protocol with 
   the function output.

%----
\begin{protocolsplitbox}{$\PiPerAMPC$}{The perfectly-secure AMPC protocol in the $(\FTriples, \FVSS, \FABA)$-hybrid model. The public inputs of
 the protocol are $\PartySet, \ckt$ and $\AdvStructure$. The above steps are executed by every 
 $P_i \in \PartySet$}{fig:PerAMPC}
	\justify
%----
Set the sharing specification as $\ShareSpec = (S_1, \ldots, S_h)
 \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$, where $\AdvStructure$ is the adversary structure.\footnote{Thus $\ShareSpec$ is
  {\it $\AdvStructure$-private}.}
%----
\begin{center}\underline{\bf Pre-Processing Phase}\end{center}
%----
Upon receiving the input $(\prep, \sid, P_i)$ from the environment, proceed as follows:
   %-----
     \begin{mydescription}
     %---
     \item [1.] Send $(\triples, \sid, P_i)$ to the functionality $\FTriples$.
     %---
     \item [2.] Request output from $\FTriples$ until an output
       $(\tripleshares, \sid, \{[a^{(\ell)}]_q, [b^{(\ell)}]_q, [c^{(\ell)}]_q) \}_{\ell \in \{1, \ldots, M\}, P_i \in S_q})$ is received from $\FTriples$. 
     %----
     \end{mydescription}  
%----
\begin{center}\underline{\bf Input Phase}\end{center}
 Once the output from $\FTriples$ is received then upon receiving the input $(\inp, \sid, x^{(i)})$ from the environment, proceed as follows:
%---
    \begin{myitemize}
    %----
    \item {\bf Secret-sharing of the Inputs and Collecting Shares of Other Inputs}:
    %---
      \begin{mydescription}
       %----
         \item Randomly select the shares $x^{(i)}_1, \ldots, x^{(i)}_h \in \F$, subject to the condition that
         $x^{(i)} = x^{(i)}_1 + \ldots + x^{(i)}_h$.
         Send $(\Dealer, \sid_i, P_i, (x^{(i)}_1, \ldots, x^{(i)}_h))$ to $\FVSS$, where 
         $\sid_i \defined \sid || i$.\footnote{The notation $\sid_i$ is used here to distinguish among the $n$ different calls to
         $\FVSS$.}
         %---
         \item For $j = 1, \ldots, n$, 
          request output from $\FVSS$ with $\sid_j$,  until receiving
          $(\Share, \sid_j, P_j, \{[x^{(j)}]_q \}_{P_i \in S_q})$,  where $P_j$ acts as the dealer.          
       %---
      \end{mydescription}
     %-------------- 
    \item {\bf Selecting Common Input-Providers}: 
    %Initialize a set of {\it local input-providers} $\LocalProv_i$ to $\emptyset$
    %and a set of {\it global input-providers} $\GlobalProv_i$ to $\emptyset$.
    %----
       \begin{mydescription}
         %------
             \item[1.]  If $(\Share, \sid_j, P_j, \{[x^{(j)}]_q \}_{P_i \in S_q})$ is received from $\FVSS$ with $\sid_j$, then  send              
              $(\vote, \sid_j, 1)$ to $\FABA$ with $\sid_j$, 
              where $\sid_j \defined \sid || j$.\footnote{The notation $\sid_j$ is used here to distinguish among the $n$ different calls to
         $\FABA$.}
             %----
             \item [2.] For $j = 1, \ldots, n$, request output from $\FABA$ with $\sid_j$ until receiving an output.
             %---
             \item [3.] If there exists a set of parties $\GlobalProv_i$, such that $\PartySet \setminus \GlobalProv_i \in \AdvStructure$
             and $(\decide, \sid_j, 1)$ is received from $\FABA$ with $\sid_j$ corresponding to each $P_j \in \GlobalProv_i$, 
             then send
              $(\vote, \sid_j, 0)$ to every $\FABA$ with $\sid_j$ for which no input has been provided yet.
          %----
             \item [4.] Once $(\decide, \sid_j, v_j)$ is received from $\FABA$ with $\sid_j$ for every $j \in \{1, \ldots, n \}$, set
                  $\CoreSet = \{P_j: v_j = 1\}$.
            %---
            \item [5.] Wait until receiving $(\Share, \sid_j, P_j, \{[x^{(j)}]_q \}_{P_i \in S_q})$ from $\FVSS$ for every $P_j \in \CoreSet$.              
               For every $P_j \not \in \CoreSet$, participate in an instance of the protocol $\PiPerDefaultShare$ with public input $0$, to generate a default secret-sharing of $0$.               
            %----
       \end{mydescription}
    \end{myitemize}
%----
\begin{center}\underline{\bf Circuit-Evaluation Phase}\end{center}
%Wait until the Input Phase is completed, resulting in a set $\CoreSet$ of input providers and the shares
 %for each input of the input-providers in $\CoreSet$ and the shares of the random multiplication triples are received. Then 
  Evaluate each gate $g$ in the circuit
 according to the topological ordering as follows, depending upon the type of $g$.
     %----
        \begin{myitemize}
         %-----
           \item {\bf Addition Gate}: If $g$ is an addition gate with inputs $x, y$ and output $z$, then corresponding to every $S_q$ such that
           $P_i \in S_q$, set $[z]_q = [x]_q + [y]_q$ as the share
           corresponding to $z$. Here $\{[x]_q\}_{P_i \in S_q}$ and $\{[y]_q\}_{P_i \in S_q}$ are $P_i$'s shares 
           corresponding to gate-inputs $x$ and $y$ respectively.
           %---
             \item {\bf Multiplication Gate}: If $g$ is the $\ell^{th}$ multiplication gate with inputs $x, y$ and output $z$, where $\ell \in \{1, \ldots, M \}$, then do the following:
        %----
               \begin{mydescription}
               %----
               \item [1.] Corresponding to every $S_q$ such that $P_i \in S_q$, set 
                  $[d^{(\ell)}]_q \defined [x]_q - [a^{(\ell)}]_q$ and $[e^{(\ell)}]_q \defined [y]_q - [b^{(\ell)}]_q$, where $\{[x]_q\}_{P_i \in S_q}$ and $\{[y]_q\}_{P_i \in S_q}$ are 
                  $P_i$'s shares corresponding to gate-inputs $x$ and $y$ respectively and $\{([a^{(\ell)}]_q, [b^{(\ell)}]_q, [c^{(\ell)}]_q)\}_{P_i \in S_q}$
                  are $P_i$'s shares corresponding to the $\ell^{th}$ multiplication-triple.
               %-----
               \item [2.] Participate in instances of $\PiPerRec$ with shares $\{[d^{(\ell)}]_q \}_{P_i \in S_q}$ and $\{[e^{(\ell)}]_q \}_{P_i \in S_q}$ to publicly reconstruct 
                 $d^{(\ell)}$ and $e^{(\ell)}$, where $d^{(\ell)} \defined x - a^{(\ell)}$ and $e^{(\ell)} \defined y - b^{(\ell)}$.
               %----  
               \item [4.] Upon reconstructing $d^{(\ell)}$ and $e^{(\ell)}$, corresponding to every $S_q$ such that $P_i \in S_q$, set
                 $[z]_q \defined d^{(\ell)} \cdot e^{(\ell)} + d^{(\ell)} \cdot [b^{(\ell)}]_q + e^{(\ell)} \cdot [a^{(\ell)}]_q + [c^{(\ell)}]_q$.
                 Set $\{[z]_q \}_{P_i \in S_q}$ as the shares corresponding to $z$.
               %---
               \end{mydescription}
        %----
          \item {\bf Output Gate}: If $g$ is the output gate with output $y$, then participate in an instance of $\PiPerRec$ with shares $\{[y]_q \}_{P_i \in S_q}$ to publicly
          reconstruct $y$.
        %----
       \end{myitemize}
%---
\begin{center}\underline{\bf Termination Phase}\end{center}
%---
Concurrently execute the following steps during the protocol:
   %----
   \begin{mydescription}
   %---
   \item[1.] If the circuit-output $y$ is computed, then send $(\Ready, \sid, P_i, y)$ to every party in $\PartySet$.
     %---
      \item[2.] If the message $(\Ready, \sid, P_j, y)$ is received from a set of parties ${\cal A}$ such that $\AdvStructure$ satisfies  $\Q^{(1)}({\cal A}, \AdvStructure)$ condition, then 
       send $(\Ready, \sid, P_i, y)$  to every party in $\PartySet$.
       %---
       \item[3.] If the message $(\Ready, \sid, P_j, y)$ is received from a set of parties $\W$ such that $(\PartySet \setminus \W) \in \AdvStructure$, 
       then output $y$ and terminate.
   %---
   \end{mydescription}
%---
\end{protocolsplitbox}
%----

Intuitively, protocol $\PiPerAMPC$ eventually terminates, as the set $\CoreSet$ is eventually decided. This is because even if the corrupt parties do not secret-share their inputs,
 the inputs of all honest parties are eventually secret-shared. Once $\CoreSet$ is decided, the evaluation of each gate will be eventually completed:
  while the addition gates are evaluated non-interactively, the evaluation of multiplication gates requires reconstructing the corresponding masked gate-inputs
  which is eventually completed due to the reconstruction protocols.
  The privacy of the inputs of the honest parties in $\CoreSet$ will be maintained as the sharing specification $\ShareSpec$ is $\AdvStructure$-private.
  Moreover, the inputs of the corrupt parties in $\CoreSet$ will be independent of the inputs of the honest parties in $\CoreSet$, as inputs are secret-shared
  via calls to $\FVSS$. Finally, correctness holds since each gate is evaluated correctly. 
   We next rigorously formalize this intuition by giving a formal security proof
   and show that the protocol $\PiPerAMPC$ is perfectly-secure, if the parties have access to ideal functionalities
   $\FTriples, \FVSS$ and $\FABA$.   \\~\\
%---
\noindent {\bf Theorem \ref{thm:PerAMPC}.}
%---
  {\it Protocol $\PiPerAMPC$ UC-securely realizes the functionality $\Functionality$ for securely computing  $f$ (see Fig \ref{fig:FAMPC} in Appendix \ref{app:UC}) 
   with perfect security in the $(\FTriples, \FVSS, \FABA)$-hybrid model, in the 
   presence of a static malicious adversary characterized by an adversary-structure $\AdvStructure$, satisfying the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition.
   The protocol makes one call to $\FTriples$ and $\Order(n)$ calls to $\FVSS$ and $\FABA$ and additionally incurs a communication of 
   $\Order(M \cdot |\AdvStructure| \cdot n^2 \log{|\F|})$ bits, where $M$ is the number of multiplication gates in the circuit $\ckt$ representing $f$.
   
   If $\AdvStructure$ satisfies the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition, then the calls to $\FTriples$ and $\FVSS$ in $\PiPerAMPC$
   can be replaced by protocol $\PiPerTriples$ and $\PiPerVSS$ respectively. The resultant protocol in the $\FABA$-hybrid model
    makes $\Order(|\AdvStructure| \cdot n^5)$ calls to $\FABA$ and incurs a communication of 
    $\Order(M \cdot |\AdvStructure|^2 \cdot (n^7 \log{|\F|} + n^9 \log n))$ bits.\footnote{We stress that in the $(\FTriples, \FVSS, \FABA)$-hybrid model, the protocol
  requires {\it only} the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition to be satisfied by $\AdvStructure$ 
   for reconstructing the intermediate values during the
  evaluation of multiplication gates via Beaver's method. To realize $\FTriples$, $\AdvStructure$ needs to satisfy
  the  $\Q^{(4)}(\PartySet, \AdvStructure)$ condition, due to which
  the overall protocol will require the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition to be satisfied by $\AdvStructure$.}
%---
}
%----
\begin{proof}
%----
The communication complexity in the $(\FTriples, \FVSS, \FABA)$-hybrid model follows from the fact that for evaluating each multiplication gate, the 
 parties need to run $2$ instances of the reconstruction protocol $\PiPerRec$. 
  The communication complexity in the $\FABA$-hybrid model follows from the communication complexity of the protocol $\PiPerTriples$
   and $\PiPerVSS$.
 
 For security, let $\Adv$ be an arbitrary real-world adversary, attacking protocol $\PiPerAMPC$ by corrupting the set of parties $Z^{\star} \in \AdvStructure$
  and let $\Env$ be an arbitrary environment. We  show  the  existence  of  a  simulator $\SimPerAMPC$, such  that 
   the output of honest parties and the view of the adversary in an execution of the real protocol with $\Adv$
    is identical to the output in an execution with $\SimPerAMPC$ involving $\Functionality$ in the ideal model. 
    This further implies that $\Env$ cannot distinguish between the two executions.
      The steps of the simulator are  given in 
   Fig \ref{fig:SimPerAMPC}. 
   
   The high level idea of the simulator is as follows. During the simulated execution, the simulator itself performs the role of the ideal functionality $\FTriples, \FVSS$
    and $\FABA$ whenever required. Performing the role of $\FTriples$ allows the simulator to learn the secret-sharing
     of all the multiplication-triples.
   During the input phase, whenever $\Adv$ secret-shares any value through $\FVSS$ 
    on the behalf of a corrupt party, the simulator 
    records this on the behalf of the corrupt party. This allows the simulator to learn the function-input of the corresponding
   corrupt party. On the other hand, for the {\it honest} parties, the simulator picks arbitrary values as their 
   function-inputs and simulates the secret-sharing of those input values using random shares, as per $\FVSS$. 
    To select the common input-providers during the simulated execution, the simulator
   itself performs the role of $\FABA$ and simulates the honest parties as per the steps of the protocol and $\FABA$. This allows the simulator
   to learn the 
   common subset of input-providers $\CoreSet$, which the simulator passes to the functionality $\Functionality$. Notice that 
   the function-inputs for each corrupt party in $\CoreSet$ will be available with the simulator. 
   This is because for every corrupt party $P_j$ which makes it to $\CoreSet$, at least one honest party $P_i$ should participate with input $1$ in the corresponding call to
   $\FABA$, implying that the honest party $P_i$ must have received its shares from $\FVSS$,  which $P_j$ sent to
   $\FVSS$. Since in the simulation, the role of $\FVSS$ is played by the simulator, it implies that the full vector of shares provided by 
   $P_j$ to $\FVSS$ will be known to the simulator.
      Hence along with $\CoreSet$, the simulator can send the corresponding function-inputs of the corrupt parties in $\CoreSet$ to $\Functionality$.
      Upon receiving the function-output, the simulator simulates the steps of the honest parties for the gate evaluations as per the
    protocol. Finally, for the output gate, the simulator arbitrarily computes a secret-sharing of the function-output $y$ received from $\Functionality$, which is consistent
    with the shares which corrupt parties hold for the output-gate sharing. Then on the behalf of the honest parties, the simulator sends the shares corresponding to
    the above sharing of $y$ during the public reconstruction of $y$. This ensures that in the simulated execution, $\Adv$ learns function-output $y$. For the termination phase, 
    the simulator sends $y$ on the behalf of honest parties.

\begin{simulatorsplitbox}{$\SimPerAMPC$}{Simulator for the protocol $\PiPerAMPC$ where $\Adv$ corrupts the parties in set
  $Z^{\star} \in \AdvStructure$}{fig:SimPerAMPC}
	\justify
%----
$\SimPerAMPC$ constructs virtual real-world honest parties and invokes the real-world adversary $\Adv$. The simulator simulates the view of
 $\Adv$, namely its communication with $\Env$, the messages sent by the honest parties and the interaction with various functionalities. 
  In order to simulate $\Env$, the simulator $\SimPerAMPC$ forwards every message it receives from 
   $\Env$ to $\Adv$ and vice-versa.  The simulator then simulates the various phases of the protocol as follows.
%---
\begin{center}\underline{\bf Pre-Processing Phase}\end{center}
%-----
{\bf Simulating the call to $\FTriples$}: The simulator simulates the steps of $\FTriples$, by itself playing the role of $\FTriples$.
 Namely, it receives from $\Adv$, the shares corresponding to the parties in $Z^{\star}$ for each multiplication-triple and then
 randomly generates a secret-sharing of $M$ random multiplication-triples $\{(\sima^{(\ell)}, \simb^{(\ell)}, \simc^{(\ell)})\}_{\ell = 1, \ldots, M}$,
  consistent with the shares corresponding to the parties in $Z^{\star}$, as provided by
  $\Adv$. 
  At the end of simulation of this phase, the simulator will know the entire vector of shares, corresponding to the secret-sharing of all
  multiplication-triples.
  %---
  \begin{center}\underline{\bf Input Phase}\end{center}
%-----
  \begin{myitemize}
  %--
   \item The simulator simulates the operations of the honest parties during the input phase, by randomly picking $\simx^{(j)}$ as the input, for
 every $P_j \not \in Z^{\star}$ and selecting random shares $\simx^{(j)}_1, \ldots, \simx^{(j)}_h$, such that
  $\simx^{(j)} = \simx^{(j)}_1 + \ldots + \simx^{(j)}_h$ and setting $[\simx^{(j)}]_q = \simx^{(j)}_q$, for $q = 1, \ldots, h$. 
  When $\Adv$ requests output from $\FVSS$ with $\sid_j$ on the behalf of any party $P_i \in Z^{\star}$,
  then the simulator  responds with an output 
  $(\Share, \sid_j, P_j, \{[\simx^{(j)}]_q \}_{P_i \in S_q})$ 
   on the behalf of $\FVSS$.
  %---
   \item Whenever $\Adv$ sends $(\Dealer, \sid_i, P_i, (x^{(i)}_1, \ldots, x^{(i)}_h))$ 
      to $\FVSS$ on the behalf of any $P_i \in Z^{\star}$, the simulator
      records the input $x^{(i)} \defined x^{(i)}_1 + \ldots + x^{(i)}_h$ on the behalf of $P_i$.
   %---
   \item When the simulation reaches the ``Selecting Common Input-Providers" stage, the simulator simulates the interface to $\FABA$ to $\Adv$, by itself
   performing the role of $\FABA$. 
   When the first honest party completes the simulated input phase, $\SimPerAMPC$ learns the set $\CoreSet$. 
   %---
    \end{myitemize}
 %----
 \noindent {\bf Interaction with $\Functionality$}:  Once the simulator learns $\CoreSet$, it sends to $\Functionality$ 
  the input values $x^{(i)}$ that it has recorded on the behalf of each
  $P_i \in (Z^{\star} \cap \CoreSet)$ and the set of input-providers $\CoreSet$. Upon receiving back the 
   output $y$ from $\Functionality$, the simulator starts the simulation of circuit-evaluation phase.
%---
\begin{center}\underline{\bf Circuit-Evaluation Phase}\end{center}
%----
The simulator simulates the evaluation of each gate $g$ in the circuit in topological order as follows:
%---
\begin{myitemize}
%----
\item {\bf Addition Gate}: Since this step involves local computation, the simulator does not have to simulate any messages on the behalf of the
honest parties. The simulator locally adds the secret-sharings corresponding to the gate-inputs and obtains the 
  secret-sharing corresponding to the gate-output.
%---
\item {\bf Multiplication Gate}: If $g$ is the $\ell^{th}$ multiplication gate in the circuit, then the simulator takes the complete secret-sharing of the 
 $\ell^{th}$ multiplication triple $(\sima^{(\ell)}, \simb^{(\ell)}, \simc^{(\ell)})$ and computes the messages of the honest parties as per the
  steps of the protocol (by considering the secret-sharing of the above multiplication-triple and the secret-sharing of the gate-inputs)
   and sends them to $\Adv$ on the behalf of the honest parties, as part of the instances of $\PiPerRec$ protocol.
     Once the simulation of the circuit-evaluation phase is done, the simulator will know the secret-sharing corresponding to the gate-output. 
%---
\item {\bf Output Gate}: Let $[\simy] = (\simy_1, \ldots, \simy_h)$ be the secret-sharing, corresponding to the output gate, available with $\SimPerAMPC$
 during the simulated circuit-evaluation. The simulator then randomly selects shares $\simby_1, \ldots, \simby_h$ such that
 $\simby_1+  \ldots +  \simby_h = y$ and $\simby_q = \simy_q$ corresponding to every $S_q \in \ShareSpec$ where
 $S_q \cap Z^{\star} \neq \emptyset$. Then as part of the instance of $\PiPerRec$ protocol to reconstruct the function output,
  the simulator sends the shares $\{\simby_q \}_{S_q \in \ShareSpec}$ to $\Adv$, on the behalf of the honest parties.
%----
\end{myitemize}
%-----
\begin{center}\underline{\bf Termination Phase}\end{center}
%---
 The simulator sends a $\Ready$ message for $y$ to $\Adv$ on the behalf of $P_i \not \in Z^{\star}$,
  if in the simulated execution, $P_i$ has computed $y$.   
 %-- 
\end{simulatorsplitbox}
    
 We next prove a sequence of claims, which helps us to show that the joint distribution of the honest parties
  and the view of $\Adv$ is identical in both the real, as well as the ideal-world.
    We first claim that in  any execution of $\PiPerAMPC$, a set $\CoreSet$ is eventually generated. This automatically implies that
    the honest parties eventually possess a secret-sharing of $M$ multiplication-triples generated by $\FTriples$, as well as 
    a secret-sharing of the inputs of the parties in $\CoreSet$.
  %-----
  \begin{claim}
  \label{claim:PerAMPCTermination}
  %---
  In any execution of $\PiPerAMPC$, a set $\CoreSet$ is eventually generated, such that for every $P_j \in \CoreSet$, there exists some $x^{(j)}$ held by $P_j$,
   which is eventually secret-shared.
  %---
  \end{claim}
  %--------
  \begin{proof}
  %---
  The proof of this claim is similar to the proof of Claim \ref{claim:PerTriplesTermination}
   and so we skip the formal proof.
  %---
  \end{proof}
  %----
   
We next show that the view generated by $\SimPerAMPC$ for $\Adv$ is identically distributed as $\Adv$'s view during the real execution of $\PiPerAMPC$.
%----
\begin{claim}
\label{claim:PerAMPCPrivacy}
%---
The view of $\Adv$ in the simulated execution with $\SimPerAMPC$ is identically distributed as the view of $\Adv$ in the real execution of
 $\PiPerAMPC$.
%---
\end{claim}
%-------
\begin{proof}
%----
It is easy to see that the view of $\Adv$ during the pre-processing phase is identically distributed in both the executions. This is because in both the executions,
 $\Adv$ receives no messages from the honest parties and the steps of $\FTriples$ are executed by the simulator itself in the simulated execution.
 Namely, in both the executions, $\Adv$'s view consists of the shares of $M$ random multiplication-triples, corresponding to the parties in $Z^{\star}$. 
 So let us fix these shares. Now conditioned on these shares,  
  for the input phase, $\Adv$ learns the shares $\{[x^{(j)}]_q \}_{P_j \not \in Z^{\star}, (S_q \cap Z^{\star}) \neq \emptyset}$ during the real execution,
  corresponding to the
 parties $P_j \not \in Z^{\star}$, while in the simulated execution it learns the shares 
  $\{[\simx^{(j)}]_q \}_{P_j \not \in Z^{\star}, (S_q \cap Z^{\star}) \neq \emptyset}$. Since the sharing specification $\ShareSpec$
   is $\AdvStructure$-private and the vector of shares $(x^{(j)}_1, \ldots, x^{(j)}_h)$ as well as 
   $(\simx^{(j)}_1, \ldots, \simx^{(j)}_h)$ are randomly chosen, it follows that the 
  the distribution of  the shares $\{[x^{(j)}]_q \}_{P_j \not \in Z^{\star}, (S_q \cap Z^{\star}) \neq \emptyset}$
  as well as $\{[\simx^{(j)}]_q \}_{P_j \not \in Z^{\star}, (S_q \cap Z^{\star}) \neq \emptyset}$ is identical and
  independent of both $x^{(j)}$ as well as $\simx^{(j0}$,
    so let us fix these shares. Since the role of $\FABA$ is played by the simulator itself, it follows easily that the view of $\Adv$ during the selection of the set $\CoreSet$
  is identically distributed in both the real as well as the simulated execution.
 
 During the evaluation of linear gates, no communication is involved. During the evaluation of multiplication gates, in the simulated execution,
 the simulator will know the secret-sharing associated with gate-inputs and also the secret-sharing of the associated
 multiplication-triple. Hence the simulator correctly sends the shares corresponding to the values $d^{(\ell)}$ and $e^{(\ell)}$ as per the protocol
 on the behalf of the honest parties. This ensures that the $\Adv$'s view during the evaluation of multiplications gates is identically distributed
 in both the executions.
  
 For the output gate, the shares received by $\Adv$ in the real execution from the honest correspond to a secret-sharing
 of the function-output $y$. From the steps of $\SimPerAMPC$, it is easy to see that the same holds even in the simulated execution,
 as $\SimPerAMPC$ sends to $\Adv$ shares corresponding to a secret-sharing of $y$, which are consistent with the shares
 held by $\Adv$. Hence the $\Adv$'s view is identically distributed in both the executions during the evaluation of output gate.
 Finally, it is easy to see that $\Adv$'s view is identically distributed in both the executions during the termination phase. This is because 
 in both the executions, every honest party who has obtained the function output $y$, sends a $\Ready$ message for $y$.
%---
\end{proof}
 %-----
 
  We next claim that conditioned on the view of $\Adv$ (which is identically distributed in both the executions from the last claim),
    the output of the honest parties is identically distributed in both the worlds.
 %---
 \begin{claim}
\label{claim:PerAMPCOutputDistribution}
%---
Conditioned on the view of $\Adv$, the output of the honest parties is
  identically distributed in the real execution of $\PiPerAMPC$ involving $\Adv$, as well as in the ideal execution
 involving $\SimPerAMPC$ and $\Functionality$.
%---
\end{claim}
%----
 \begin{proof}
 %----
 Let $\View$ be an arbitrary view of $\Adv$. And let $\CoreSet$ be the set of input-providers as determined by $\View$ 
  (from Claim \ref{claim:PerAMPCTermination}, such a set $\CoreSet$ is bound to exist).
  Moreover, according to $\View$,  for every $P_i \in \CoreSet$, there exists some input $x^{(i)}$, such that the parties hold a 
  secret-sharing of $x^{(i)}$. Furthermore, from Claim \ref{claim:PerAMPCPrivacy},  
   if $P_i \in Z^{\star}$ then the corresponding secret-sharing is included in $\View$ while for $P_i \not \in Z^{\star}$, 
   the corresponding $x^{(i)}$ is uniformly distributed, conditioned on the shares of $x^{(i)}$ available with $\Adv$ as determined by
   $\View$. Let us fix the $x^{(i)}$ values corresponding to the parties in $\CoreSet$
   and denote by $\vec{x}$ the vector of values $x^{(i)}$, where $x^{(i)} = 0$ if $P_i \not \in \CoreSet$.
   
   It is easy to see that in the ideal-world, the output of the honest parties is $y$, where $y \defined f(\vec{x})$.
   This is because $\SimPerAMPC$ provides the identity of $\CoreSet$ along with the inputs $x^{(i)}$ corresponding to $P_i \in (\CoreSet \cap Z^{\star})$ to
   $\Functionality$. We now show that the honest parties eventually output $y$ even in the real-world. For this, we argue
    that all the values during the circuit-evaluation phase of the protocol are correctly secret-shared. 
    Since the evaluation of linear gates need only local computation, it follows
 that the output of the linear gates will be correctly secret-shared. During the evaluation of a multiplication gate, the honest parties will hold a 
  secret-sharing of the corresponding $d^{(\ell)}$ and $e^{(\ell)}$ values, as during the pre-processing phase,
  all the multiplication-triples are generated in a secret-shared fashion, since they are computed
 and distributed by $\FTriples$. Since $\ShareSpec$ satisfies the $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition,
  the honest parties eventually get $d^{(\ell)}$ and $e^{(\ell)}$ through the instances of $\PiPerRec$.
     This automatically implies that the honest parties eventually hold a secret-sharing of $y$ and reconstruct it correctly, as
     $y$ is reconstructed through an instance of $\PiPerRec$. 
     Hence during the termination phase, every honest party will eventually send a $\Ready$ message for $y$, while the parties in $Z^{\star}$
     may send a $\Ready$ message for $y' \neq y$. Since $Z^{\star} \in \AdvStructure$, it follows that
     no honest party ever sends a $\Ready$ message for $y'$. Hence no honest party ever outputs $y'$, as it will never receive
     the required number of $\Ready$ messages for $y'$.
           Since the $\Ready$ messages of the {\it honest}
     parties for $y$ are eventually delivered to every honest party, it follows that eventually all honest parties 
     receive sufficiently many $\Ready$ messages to obtain some output, even if the corrupt parties does not send the required messages.
     
     Now let $P_i$ be the {\it first honest} party to terminate the protocol with some output. From the above arguments, the output has to be $y$.
     This implies that $P_i$ receives $\Ready$ messages for $y$ 
    from at least a set of parties $\PartySet \setminus Z$, for some $Z \in \AdvStructure$. 
       Let $\Hon$ be the set of {\it honest} parties whose $\Ready$ messages are received by $P_i$. It is easy to see that
   $\Hon \not \in \AdvStructure$, as otherwise $\AdvStructure$ does not satisfy the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition.
    The $\Ready$ messages of the parties in $\Hon$ are eventually delivered to every honest party
   and hence {\it each} honest party (including $P_i$) eventually executes the step $2$ of the termination phase and sends a
   $\Ready$ message for $y$.
   It follows that the $\Ready$ messages of {\it all} honest parties $\PartySet \setminus Z^{\star}$
    are eventually delivered
   to every honest party (irrespective of whether $\Adv$ sends all the required
   messages), consequently guaranteeing that all honest parties eventually obtain the output $y$.
    %---
 \end{proof}
 %-----  
The theorem now follows from Claim \ref{claim:PerAMPCTermination}-\ref{claim:PerAMPCOutputDistribution}.
%---
\end{proof}


%----------------OLD STUFF%%%%%%%%
\begin{comment}
Before we present protocol $\PiPerVSS$, we prove a helping lemma.

\begin{lemma}
\label{lemma:PerVSSHelping}
Consider an adversary structure $\AdvStructure$ which satisfies the $\Q^{(k)}(S, \AdvStructure)$ condition for some set $S$, where $k > 1$. Consider the set $S' \subseteq S$ such that $S' = S \setminus Z$ for some $Z \in \AdvStructure$. Then, $\AdvStructure$ satisfies the $\Q^{(k-1)}(S', \AdvStructure)$ condition.
\end{lemma}
\begin{proof}
Assume for contradiction that there is a set $S' = S \setminus Z$ for some $Z \in \AdvStructure$ such that $\AdvStructure$ does not satisfy the $\Q^{(k-1)}(S', \AdvStructure)$ condition. Then, $S' = Z_{i_1} \cup \ldots \cup Z_{i_{k-1}}$, for some $Z_{i_1}, \ldots , Z_{i_{k-1}} \in \AdvStructure$. Since $S' \cup Z = S$, this would mean that $Z_{i_1} \cup \ldots \cup Z_{i_{k-1}} \cup Z = S$. Thus, $\AdvStructure$ does not satisfy the $\Q^{k}(S,\AdvStructure)$ condition, which is a contradiction.
\end{proof}

The main purpose of $\FVSS$ is to enable a dealer $P_{\D} \in \PartySet$ to share values $s_1,\ldots,s_h$ such that each (honest) party in $S_q$ receives $s_q$, for each group of parties $S_q \in \ShareSpec$. Thus, $\D$ first distributes shares, by sending $s_q$ to each party in $S_q$, for all $S_q \in \ShareSpec$. While an honest dealer is sure to distribute the same value uniformly to all parties, a corrupt dealer may not. Therefore, the parties perform pairwise consistency tests, and upon receiving a value from the dealer, exchange this value with all the other parties in their respective groups. Each party $P_i$  announces the results of the test by sending $\OK_q(i,j)$ to $\FAcast$, if it receives a consistent value from party $P_j \in S_q$, for every group $S_q$ which $P_i$ is a part of. The parties then construct $h$ consistency graphs, one for each group in $\ShareSpec$, where edge $(P_i,P_j)$ is added to the consistency graph for $S_q$ if messages $\OK_q(i,j)$ and $\OK_q(j,i)$ are received as output from $\FAcast$ upon request. The dealer $P_{\D}$ waits for a core set $\C_q$ to form for each $S_q \in \ShareSpec$, such that $\C_q = S_q \setminus Z$ for some $Z \in \AdvStructure$, and that the set of parties in $\C_q$ forms a clique in the consistency graph for $S_q$. For an honest dealer, such a set will definitely form, since the honest parties in $S_q$ will be pairwise consistent with each other. The dealer then makes public the identity of the core sets using $\FAcast$. 

The parties compute their output as follows. From Lemma \ref{lemma:PerVSSHelping}, since $\AdvStructure$ satisfies the $\Q^{3}(\ShareSpec,\AdvStructure)$ condition, $\AdvStructure$ satisfies the $\Q^{2}(\C_q,\AdvStructure)$ condition. Because $\C_q$ forms a clique, the honest parties in $\C_q$ have all received the same value from $P_{\D}$.  We now wish for {\it all} honest parties in $S_q$ to obtain this value as their share. To do this, for every $S_q \in \ShareSpec$, each party in $S_q$ waits till it receives the same value as part of pairwise consistency checks from a set of parties $\C'_q = \C_q \setminus Z$ for some $Z \in \AdvStructure$. From Lemma \ref{lemma:PerVSSHelping}, since $\AdvStructure$ satisfies the $\Q^{2}(\C_q,\AdvStructure)$ condition, $\AdvStructure$ satisfies the $\Q^{1}(\C'_q,\AdvStructure)$ condition. thus, $\C'_q$ contains at least one honest party, and each party in $S_q$ will output the value received by this party from $P_{\D}$. Since the honest parties in $\C_q$ form such a valid set for $\C'_q$, each party in $S_q$ eventually outputs a share. We present $\PiPerVSS$ in Figure \ref{fig:PerAVSS}.


   
      
       Every other honest $P_k \in S_q$ will thus receive $(\test,\sid,q,s_{qj})$ from $P_j$ such that $s_{qj} = s^{(q)}_k$, and will send $(\Sender,\Acast,\sid^{(q)}_{kj},\OK_q(k,j))$ as input to $\FAcast$, which $\D$ will obtain as output upon request from $\FAcast$. Hence, for every $S_q \in \ShareSpec$, a core set $\C_q = S_q \setminus Z^{\star}$ which is a clique in $G^{\D}_q$ will eventually form, and $P_\D$ will send these core sets as input to $\FAcast$, which every (honest) party will receive as output from $\FAcast$, upon request.

We next show that for {\it any} core set $\C_q$ which is $S_q \setminus Z$ for some $Z \in \AdvStructure$, honest party $P_i$ will eventually set $[s]_q$ to $s^{(q)}$ based on values received as part of paiwise consistency tests from parties in $\C_q$. For this, we note that $P_i$ will eventually receive $s^{(q)}$ from a set of parties $\C'_q = \C_q \setminus Z^{\star}$ as part of pairwise consistency checks, from the {\it honest} parties in $\C_q$, and will set $[s]_q$ to some value. We next show that if $P_i$ receives $s'^{(q)}$ from a set of parties $\C'_q = \C_q \setminus Z$ for any $Z \in \AdvStructure$, then $s'^{(q)} = s^{(q)}$. For this, note that $\AdvStructure$ satisfies the $\Q^{(3)}(S_q,\AdvStructure)$ condition. From Lemma \ref{lemma:PerVSSHelping}, $\AdvStructure$ satisfies the $\Q^{(2)}(\C_q,\AdvStructure)$ condition, and thereby, the $\Q^{(1)}(\C'_q,\AdvStructure)$ condition. Thus, $\C'_q$ contains {\it at least} one honest party, which means that $s'^{(q)} = s^{(q)}$.

 Assuming that $P_i$ eventually finds such a common $\C'_q$, the proof that the common $s_{qj}$ is the same as $s_q$
      follows from the fact that $\C'_q$ is guaranteed to contain at least one {\it honest} party from $\C_q$, who would have received the share
      $s_{qj} = s_q$ from $P_{\D}$ and sent to $P_i$ as part of the pairwise consistency test. This is because the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition is satisfied.
      Also, since the $\Q^{(4)}(\PartySet, \AdvStructure)$ condition is satisfied, the set of {\it honest} parties in $\C_q$, namely the parties in 
      $\C_q \setminus Z^{\star}$, always constitute a candidate $\C'_q$ set. This is because every party $P_j \in \C_q \setminus Z^{\star}$
      would have sent $s_{qj} = s_q$ to every party in $S_q$ during the pairwise consistency test and these values are eventually delivered. 


  Consider an honest party $P_i$. Consider a set $S_q \in \ShareSpec$ such that $P_i \in S_q$. Let $\Hon_q$ be the set of honest parties in the core set $\C_q$ crresponding to $S_q$. Since each $\C_q$ is valid, it forms a clique in $G^i_q$. Thus, all parties in $\Hon_q$ received the same value corresponding to $S_q$ when $P_\D$ distributed shares. Suppose that this value is $s^{(q)}$, which is determined by $\View$. We show that in both worlds, $P_i$ outputs $s^{(q)}$ as its share corresponding to the set $S_q$. In $\PiPerVSS$, we first note that $P_i$ will eventually receive $s'^{(q)}$ from a set of parties $\C'_q = \C_q \setminus Z$ for some $Z \in \AdvStructure$ as part of pairwise consistency checks, and will thus set $[s]_q$ to some value. This is because it will eventually receive $s^{(q)}$ from $\Hon_q = \C_q \setminus Z^{\star}$. We next show that $s'^{(q)} = s^{(q)}$. For this, note that $\AdvStructure$ satisfies the $\Q^{(3)}(S_q,\AdvStructure)$ condition. From Lemma \ref{lemma:PerVSSHelping}, $\AdvStructure$ satisfies the $\Q^{(2)}(\C_q,\AdvStructure)$ condition, and thereby, the $\Q^{(1)}(\C'_q,\AdvStructure)$ condition. Thus, $\C'_q$ contains {\it at least} one honest party, which means that $s'^{(q)} = s^{(q)}$. In the ideal world, $\SimPVSS$ sets $[s]_q$ to $s^{(q)}$, since it sets it to a value held by an honest party in $\C_q$, and sends this as input to $\FVSS$. Hence, $P_i$ obtains $s^{(q)}$ as its share corresponding to $S_q$ in the ideal world. Since this is true for every $S_q \in \ShareSpec$, the output of each honest party is the same in both worlds.





$P_i$ waits till it receives $(\Share,\sid,q,v)$ from a set of parties in $S_q \setminus Z$ for some set $Z \in \AdvStructure$. Let $\Hon^{(q)}$ be the set of honest parties in $S_q$. Since $\Hon^{(q)} = S_q \setminus (Z^{\star} \cap S_q)$, where $(Z^{\star} \cap S_q) \in \ShareSpec$, and since each honest party in $S_q$ holds the same value $[s]_q$, $P_i$ will eventually $(\Share,\sid,q,v)$ from such a set of parties. Suppose that this set is $\C^{(q)}$. From \ref{lemma:PerVSSHelping}, since $\AdvStructure$ satisfies the $\Q^{(2)}(S_q,\AdvStructure)$ condition, $\AdvStructure$ satisfies the $\Q^{(1)}(\C^{(q)},\AdvStructure)$ condition. Therefore, $\C^{(q)}$ contains at least one honest party and therefore, $v = [s]_q$. Hence, $P_i$ outputs $[s]_q$.

\begin{proof}
%----
Consider a party $P_i \in \PartySet$. From \ref{lemma:PerRecShare}, $P_i$ receives $(\recShare,\sid_q,q,[s]_q)$ as the output of $\PiPerRecShare(\sid_q,q)$, where $\sid_q = \sid || q$. Hence, by the protocol steps, $P_i$ eventually outputs $s = \sum_{S_q \in \ShareSpec}[s]_q$.
%----
\end{proof}


\end{comment}




==> AppPerfectAMPCModified.tex <==
\section{Perfectly-Secure AMPC}
\label{app:Perfect}
%----
\subsection{Asynchronous VSS Protocol}
%---

Before we present protocol $\PiPerVSS$, we prove a helping lemma.

\begin{lemma}
\label{lemma:PerVSSHelping}
Consider an adversary structure $\AdvStructure$ which satisfies the $\Q^{(k)}(S, \AdvStructure)$ condition for some set $S$, where $k > 1$. Consider the set $S' \subseteq S$ such that $S' = S \setminus Z$ for some $Z \in \AdvStructure$. Then, $\AdvStructure$ satisfies the $\Q^{(k-1)}(S', \AdvStructure)$ condition.
\end{lemma}
\begin{proof}
Assume for contradiction that there is a set $S' = S \setminus Z$ for some $Z \in \AdvStructure$ such that $\AdvStructure$ does not satisfy the $\Q^{(k-1)}(S', \AdvStructure)$ condition. Then, $S' = Z_{i_1} \cup \ldots \cup Z_{i_{k-1}}$, for some $Z_{i_1}, \ldots , Z_{i_{k-1}} \in \AdvStructure$. Since $S' \cup Z = S$, this would mean that $Z_{i_1} \cup \ldots \cup Z_{i_{k-1}} \cup Z = S$. Thus, $\AdvStructure$ does not satisfy the $\Q^{k}(S,\AdvStructure)$ condition, which is a contradiction.
\end{proof}


%-----
\begin{claim}
\label{claim:PVSSHonestDPrivacy}
%---
If the dealer is honest, then the view of $\Adv$ in the simulated execution of $\PiPerVSS$ with $\SimPVSS$ is identically distributed to the view of $\Adv$ in the real execution of $\PiPerVSS$ involving honest parties.
%---
\end{claim}
%----
\begin{proof}
%----
Suppose that $\ShareSpec^{\star} = \{S_q \in \ShareSpec \mid S_q \cap Z^{\star} \neq \phi \}$. The view of $\Adv$ during the real execution of $\PiPerVSS$ consists of the following.
\begin{myenumerate}
\item[--] The shares $\{[s]_q\}_{S_q \in \ShareSpec^{\star}}$ distributed by $P_{\D}$ : In the real execution, $\Adv$ receives $[s]_q$ from $P_{\D}$ for each $S_q \in \ShareSpec^{\star}$. In the ideal world, the simulator provides this to $\Adv$ on behalf of $P_{\D}$.
%----
\item[--] Messages $(\test,\sid,q,s^{(q)}_j)$ received from every party $P_j \in S_q$, for every $S_q \in \ShareSpec^{\star}$, as part of pairwise consistency tests : While each honest $P_j$ sends this to $\Adv$ in the real execution, the simulator sends this on the behalf of $P_j$ in the ideal execution.
%----
\item[--] The results of pairwise consistency tests $\OK_q(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ messages for every request $\Adv$ makes to $\FAcast$ with $\sid^{(q)}_{ij} = \sid || q || i || j$, for every $S_q \in \ShareSpec$ and $P_i,P_j \in S_q$ : To compare the view of $\Adv$ between real and ideal executions, we consider the following cases considering some set $S_q \in \ShareSpec$.
	\begin{myitemize}
	%----
	\item[--] $P_i,P_j \in S_q \setminus Z^{\star}$ : In both the real and ideal executions, $\Adv$ receives $\OK_q(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ as the output from $\FAcast$.
	%----
	\item[--] $P_i \in S_q \setminus Z^{\star}, P_j \in (S_q \cap Z^{\star}) $:  In both the real and ideal executions, $\Adv$ receives $\OK_q(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ as the output from $\FAcast$ if $\Adv$ sent $(\test,\sid,q,s^{(j)}_q)$ such that $s^{(j)}_q = [s]_q$.
	%----
	\item[--] $P_i, P_j \in (S_q \cap Z^{\star}) $:  In both the real and ideal executions, $\OK_q(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ is based on the input $\Adv$ sends to $\FAcast$.
	%----
	\end{myitemize}
%----
\item[--] Broadcasted core sets $\{\C_q\}_{S_q \in \ShareSpec}$ for each set in $\ShareSpec$ : In both the real and ideal executions, each $\C_q$ broadcasted for $S_q \in \ShareSpec$ is based on the $\OK$ messages sent to / on behalf of $\FAcast$. 
\end{myenumerate}
%----
\end{proof}
%----

%----
\begin{claim}
\label{claim:PVSSHonestDCorrectness}
%----
If $\D$ is honest, then conditioned on the view of $\Adv$, the output of the honest parties during the execution of $\PiPerVSS$ involving $\Adv$ has the  same distribution as the output of the honest parties in the ideal-world involving $\SimPVSS$ and $\FVSS$.
%----
\end{claim}
%-----
%----
\begin{proof}
%----
In the ideal world, each honest party $P_i$ obtains output $\{[s]_q\}_{P_i \in S_q}$ from $\FVSS$. We show that $P_i$ eventually receives output $\{[s]_q\}_{P_i \in S_q}$ in the real world as well. For this, suppose that {\it all} honest parties have input $\participate$ in $\PiPerVSS$. Honest $P_\D$ distributes $s^{(q)}$ uniformly to all parties $P_j \in S_q$, for all $S_q \in \ShareSpec$. Consider some $S_q \in \ShareSpec$. During paiwise consistency tests, since all honest parties have input $\participate$, each honest $P_j \in S_q$ will send $(\test,\sid,q,s^{(q)}_j)$ to all other parties in $S_q$. Every other honest $P_k \in S_q$ will thus receive $(\test,\sid,q,s^{(q)}_j)$ from $P_j$ such that $s^{(q)}_j = s^{(q)}_k$, and will send $(\Sender,\Acast,\sid^{(q)}_{kj},\OK_q(k,j))$ as input to $\FAcast$, which $\D$ will obtain as output upon request from $\FAcast$. Hence, for every $S_q \in \ShareSpec$, a core set $\C_q = S_q \setminus Z^{\star}$ which is a clique in $G^{\D}_q$ will eventually form, and $P_\D$ will send these core sets as input to $\FAcast$, which every (honest) party will receive as output from $\FAcast$, upon request.

We next show that for {\it any} core set $\C_q$ which is $S_q \setminus Z$ for some $Z \in \AdvStructure$, honest party $P_i$ will eventually set $[s]_q$ to $s^{(q)}$ based on values received as part of paiwise consistency tests from parties in $\C_q$. For this, we note that $P_i$ will eventually receive $s^{(q)}$ from a set of parties $\C'_q = \C_q \setminus Z^{\star}$ as part of pairwise consistency checks, from the {\it honest} parties in $\C_q$, and will set $[s]_q$ to some value. We next show that if $P_i$ receives $s'^{(q)}$ from a set of parties $\C'_q = \C_q \setminus Z$ for any $Z \in \AdvStructure$, then $s'^{(q)} = s^{(q)}$. For this, note that $\AdvStructure$ satisfies the $\Q^{(3)}(S_q,\AdvStructure)$ condition. From Lemma \ref{lemma:PerVSSHelping}, $\AdvStructure$ satisfies the $\Q^{(2)}(\C_q,\AdvStructure)$ condition, and thereby, the $\Q^{(1)}(\C'_q,\AdvStructure)$ condition. Thus, $\C'_q$ contains {\it at least} one honest party, which means that $s'^{(q)} = s^{(q)}$.
%----
\end{proof}
%----

%------
\begin{claim}
\label{claim:PVSSCorruptDPrivacy}
%---
If the dealer is corrupt, then 
the the view of $\Adv$ in the simulated execution of $\PiPerVSS$ with $\SimPVSS$ is identically distributed to the view of $\Adv$ in the real execution of
$\PiPerVSS$ involving honest parties.
%---
\end{claim}
%-----
%----
\begin{proof}
\end{proof}
%----

%----
\begin{claim}
\label{claim:PVSSCorruptDCorrectness}
%----
If $\D$ is corrupt, then conditioned on the view of $\Adv$, the output of the honest parties during the execution of $\PiPerVSS$ involving $\Adv$ has the  same distribution as the output of the honest parties in the ideal-world involving $\SimPVSS$ and $\FVSS$.
%----
\end{claim}
%-----
%----
\begin{proof}
%----
Let $\D$ be corrupt and $\View$ be an arbitrary view of $\Adv$. We note that it can be found out from $\View$ whether the core sets $\{\C_q\}_{S_q \in \ShareSpec}$ generated during the corresponding execution of $\PiPerVSS$ are valid or not. We now consider the following cases.

\begin{myitemize}
%----
\item[--] {\it No core sets $\{\C_q\}_{S_q \in \ShareSpec}$ are generated as per $\View$ : } In both worlds, no output is obtained. In $\PiPerVSS$, the parties compute their output only when they receive some set $\{\C_q\}_{S_q \in \ShareSpec}$ upon request from $\FAcast$. In the ideal world, the simulator $\SimPVSS$ does not provide any input to $\FVSS$ on behalf of $P_\D$, and hence, $\FVSS$ does not produce any output for the honest parties.
%----
\item[--] {\it Invalid core sets $\{\C_q\}_{S_q \in \ShareSpec}$ are generated as per $\View$ : } In both worlds, no output is obtained. In $\PiPerVSS$, even if $\{\C_q\}_{S_q \in \ShareSpec}$ is received from $\FAcast$ upon request, the parties compute their output only when each $\C_q$ is {\it valid} corresponding to its consistecy graph for $S_q$. In the ideal world, the simulator $\SimPVSS$ does not provide any input to $\FVSS$ on behalf of $P_\D$ if valid core sets are not received, and hence, $\FVSS$ does not produce any output for the honest parties.
%----
\item[--] {\it Valid core sets $\{\C_q\}_{S_q \in \ShareSpec}$ are generated as per $\View$ : } Consider an honest party $P_i$. Consider a set $S_q \in \ShareSpec$ such that $P_i \in S_q$. Let $\Hon_q$ be the set of honest parties in the core set $\C_q$ crresponding to $S_q$. Since each $\C_q$ is valid, it forms a clique in $G^i_q$. Thus, all parties in $\Hon_q$ received the same value corresponding to $S_q$ when $P_\D$ distributed shares. Suppose that this value is $s^{(q)}$, which is determined by $\View$. We show that in both worlds, $P_i$ outputs $s^{(q)}$ as its share corresponding to the set $S_q$. In $\PiPerVSS$, we first note that $P_i$ will eventually receive $s'^{(q)}$ from a set of parties $\C'_q = \C_q \setminus Z$ for some $Z \in \AdvStructure$ as part of pairwise consistency checks, and will thus set $[s]_q$ to some value. This is because it will eventually receive $s^{(q)}$ from $\Hon_q = \C_q \setminus Z^{\star}$. We next show that $s'^{(q)} = s^{(q)}$. For this, note that $\AdvStructure$ satisfies the $\Q^{(3)}(S_q,\AdvStructure)$ condition. From Lemma \ref{lemma:PerVSSHelping}, $\AdvStructure$ satisfies the $\Q^{(2)}(\C_q,\AdvStructure)$ condition, and thereby, the $\Q^{(1)}(\C'_q,\AdvStructure)$ condition. Thus, $\C'_q$ contains {\it at least} one honest party, which means that $s'^{(q)} = s^{(q)}$. In the ideal world, $\SimPVSS$ sets $[s]_q$ to $s^{(q)}$, since it sets it to a value held by an honest party in $\C_q$, and sends this as input to $\FVSS$. Hence, $P_i$ obtains $s^{(q)}$ as its share corresponding to $S_q$ in the ideal world. Since this is true for every $S_q \in \ShareSpec$, the output of each honest party is the same in both worlds.
%----
\end{myitemize}

%----
\end{proof}
%----


\subsection{Asynchronous Reconstruction Protocols}

Suppose that $\AdvStructure$ satisfies the $\Q^{(2)}(\ShareSpec,\AdvStructure)$ condition. We first present protocol $\PiPerRecShare$, which allows all parties in $\PartySet$ to reconstruct a {\it single} share $[s]_q$, corresponding to the set $S_q \in \ShareSpec$, where $[s]_q$ is the share held by all {\it honest} parties in $S_q$. The idea behind the protocol is simiilar to how a party {\it outside} core set $\C_q$ obtained $[s]_q$ in $\PiPerVSS$, where $[s]_q$ is the value held by all {\it honest} parties in $\C_q$.  Protocol $\PiPerRecShare$ is presented in Figure \ref{fig:PerRecShare}.

%----
\begin{protocolsplitbox}{$\PiPerRecShare(\sid,q)$}{Perfectly-secure reconstruction protocol to reconstruct a single share $[s]_q$ for $S_q \in \ShareSpec$. The public inputs of the protocol are $\PartySet$, $\AdvStructure$ and $1 \leq q \leq |\ShareSpec|$. The above steps are executed by every $P_i \in \PartySet$}{fig:PerRecShare}
%----
\justify
%----
\begin{myitemize}
%----
\item {\bf Sending share to all parties : }If $P_i \in S_q$, then execute the following steps.
	\begin{myenumerate}
	\item On having $[s]_q$, send $(\Share,\sid,q,[s]_q)$ to all parties in $\PartySet \setminus S_q$.
	\end{myenumerate} 
%----
\item {\bf Computing output : } Based on the condition, execute the corresponding steps.
	\begin{myenumerate}
	\item {\bf $P_i \in S_q$ : } Output $(\recShare,\sid,q,[s]_q)$
	\item {\bf $P_i \notin S_q$ : } Upon receiving $(\Share,\sid,q,v)$ from a set of parties in $S_q \setminus Z$ for some $Z \in \AdvStructure$, set $[s]_q = v$ and output $(\recShare,\sid,q,[s]_q)$
	\end{myenumerate} 
\end{myitemize}
%----
\end{protocolsplitbox}
%----

\begin{lemma}
%----
\label{lemma:PerRecShare}
%----
Consider an adversary structure $\AdvStructure$ which satisfies the $\Q^{(2)}(\ShareSpec, \AdvStructure)$. Suppose that all the honest parties in set $S_q \in \ShareSpec$ hold the same value $[s]_q$. Protocol $\PiPerRecShare$ enables all parties in $\PartySet$ to eventually output $[s]_q$.
%----
\end{lemma}
%----
\begin{proof}
%----
Consider a party $P_i \in \PartySet$. We consider two cases.
\begin{itemize}
%----
\item[--] $P_i \in S_q$ : By the protocol definition, $P_i$ outputs $[s]_q$.
%----
\item[--] $P_i \notin S_q$ : $P_i$ waits till it receives $(\Share,\sid,q,v)$ from a set of parties in $S_q \setminus Z$ for some set $Z \in \AdvStructure$. Let $\Hon^{(q)}$ be the set of honest parties in $S_q$. Since $\Hon^{(q)} = S_q \setminus (Z^{\star} \cap S_q)$, where $(Z^{\star} \cap S_q) \in \ShareSpec$, and since each honest party in $S_q$ holds the same value $[s]_q$, $P_i$ will eventually $(\Share,\sid,q,v)$ from such a set of parties. Suppose that this set is $\C^{(q)}$. From \ref{lemma:PerVSSHelping}, since $\AdvStructure$ satisfies the $\Q^{(2)}(S_q,\AdvStructure)$ condition, $\AdvStructure$ satisfies the $\Q^{(1)}(\C^{(q)},\AdvStructure)$ condition. Therefore, $\C^{(q)}$ contains at least one honest party and therefore, $v = [s]_q$. Hence, $P_i$ outputs $[s]_q$.
%----
\end{itemize}
%----
\end{proof}
%----

We now present protocol $\PiPerRec$, which allows {\it all} parties in $\PartySet$ to reconstruct an additively secret shared value $s$, assuming that each (honest) party in $S_q$ holds the same share $[s]_q$, for all $S_q \in \ShareSpec$. The idea is simply to run protocol $\PiPerRecShare$ for each $S_q \in \ShareSpec$, and to sum up the shares obtained as output from each instantiation. We present protocol $\PiPerRec$ in Figure \ref{fig:PerRec}. 

%----
\begin{protocolsplitbox}{$\PiPerRec$}{Perfectly-secure reconstruction protocol to reconstruct a shared value $s$. The public inputs of the protocol are $\PartySet$ and $\AdvStructure$. The above steps are executed by every $P_i \in \PartySet$}{fig:PerRec}
%----
\justify
%----

\begin{myitemize}
%----
\item {\bf Reconstructing shares :} For each $S_q \in \ShareSpec$, execute an instance $\PiPerRecShare(\sid_q,q)$ to obtain output $(\recShare,\sid_q,q,[s]_q)$, where $\sid_q = \sid || q$.
%----
\item {\bf Output Computation :} Once output has been obtained for each $S_q \in \ShareSpec$, set $s = \sum_{S_q \in \ShareSpec}[s]_q$ and output $(\rec,\sid,s)$.
%----
\end{myitemize}
%----
\end{protocolsplitbox}
%----

\begin{lemma}
%----
\label{lemma:PerRec}
%----
Consider an adversary structure $\AdvStructure$ which satisfies the $\Q^{(2)}(\ShareSpec, \AdvStructure)$. Suppose that for every $S_q \in \ShareSpec$, all the honest parties in set $S_q \in \ShareSpec$ hold the same value $[s]_q$. Protocol $\PiPerRec$ enables all parties in $\PartySet$ to eventually output $s = \sum_{S_q \in \ShareSpec}[s]_q$.
%----
\end{lemma}
%----
\begin{proof}
%----
Consider a party $P_i \in \PartySet$. From \ref{lemma:PerRecShare}, $P_i$ receives $(\recShare,\sid_q,q,[s]_q)$ as the output of $\PiPerRecShare(\sid_q,q)$, where $\sid_q = \sid || q$. Hence, by the protocol steps, $P_i$ eventually outputs $s = \sum_{S_q \in \ShareSpec}[s]_q$.
%----
\end{proof}


%%%%%%%%%%OLD STUFF%%%%%%
\begin{comment}
%----
The main purpose of $\FVSS$ is to enable a dealer $P_{\D} \in \PartySet$ to share values $s_1,\ldots,s_h$ such that each (honest) party in $S_q$ receives $s_q$, for each group of parties $S_q \in \ShareSpec$. Thus, $\D$ first distributes shares, by sending $s_q$ to each party in $S_q$, for all $S_q \in \ShareSpec$. While an honest dealer is sure to distribute the same value uniformly to all parties, a corrupt dealer may not. Therefore, the parties perform pairwise consistency tests, and upon receiving a value from the dealer, exchange this value with all the other parties in their respective groups. Each party $P_i$  announces the results of the test by sending $\OK_q(i,j)$ to $\FAcast$, if it receives a consistent value from party $P_j \in S_q$, for every group $S_q$ which $P_i$ is a part of. The parties then construct $h$ consistency graphs, one for each group in $\ShareSpec$, where edge $(P_i,P_j)$ is added to the consistency graph for $S_q$ if messages $\OK_q(i,j)$ and $\OK_q(j,i)$ are received as output from $\FAcast$ upon request. The dealer $P_{\D}$ waits for a core set $\C_q$ to form for each $S_q \in \ShareSpec$, such that $\C_q = S_q \setminus Z$ for some $Z \in \AdvStructure$, and that the set of parties in $\C_q$ forms a clique in the consistency graph for $S_q$. For an honest dealer, such a set will definitely form, since the honest parties in $S_q$ will be pairwise consistent with each other. The dealer then makes public the identity of the core sets using $\FAcast$. 

The parties compute their output as follows. From Lemma \ref{lemma:PerVSSHelping}, since $\AdvStructure$ satisfies the $\Q^{3}(\ShareSpec,\AdvStructure)$ condition, $\AdvStructure$ satisfies the $\Q^{2}(\C_q,\AdvStructure)$ condition. Because $\C_q$ forms a clique, the honest parties in $\C_q$ have all received the same value from $P_{\D}$.  We now wish for {\it all} honest parties in $S_q$ to obtain this value as their share. To do this, for every $S_q \in \ShareSpec$, each party in $S_q$ waits till it receives the same value as part of pairwise consistency checks from a set of parties $\C'_q = \C_q \setminus Z$ for some $Z \in \AdvStructure$. From Lemma \ref{lemma:PerVSSHelping}, since $\AdvStructure$ satisfies the $\Q^{2}(\C_q,\AdvStructure)$ condition, $\AdvStructure$ satisfies the $\Q^{1}(\C'_q,\AdvStructure)$ condition. thus, $\C'_q$ contains at least one honest party, and each party in $S_q$ will output the value received by this party from $P_{\D}$. Since the honest parties in $\C_q$ form such a valid set for $\C'_q$, each party in $S_q$ eventually outputs a share. We present $\PiPerVSS$ in Figure \ref{fig:PerAVSS}.

%----
\begin{protocolsplitbox}{$\PiPerVSS$}{The perfectly-secure VSS protocol in the $(\FAcast)$-hybrid model. The public inputs of the protocol are $\PartySet$, $\AdvStructure$ and $P_{\D}$. The above steps are executed by every $P_i \in \PartySet$}{fig:PerAVSS}
\justify
%----

\begin{myitemize}
%----
\item {\bf Distribution of shares by $P_{\D}$} : If $P_i$ is $P_{\D}$, then execute the following steps.
	\begin{myenumerate}
	%----
	\item On having input $s^{(1)}, \ldots, s^{(h)} \in \F$, for each $S_q \in \ShareSpec$, send $(\dist,\sid,q,s^{(q)})$ to all parties $P_i \in S_q$.
	%----
	\end{myenumerate} 
%----
\item {\bf Pairwise consistency tests} : For each $S_q \in \ShareSpec$, if $P_i \in S_q$, then execute the following steps on having input $\participate$.
	\begin{myenumerate}
	%----
	\item Upon receiving $(\dist,\sid,q,s^{(q)}_i)$ from $\D$, send $(\test,\sid,q,s^{(q)}_i)$ to every party $P_j \in S_q$.
	%----
	\item Upon receiving $(\test,\sid,q,s^{(q)}_j)$ from $P_j \in S_q$, if $s^{(q)}_i = s^{(q)}_j$, send $(\Sender,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ to $\FAcast$, where $\sid^{(q)}_{ij} = \sid || q || i || j$.
	%----
	\end{myenumerate}
%----
\item {\bf Constructing consistency graph} : For each $S_q \in \ShareSpec$, execute the following steps.
	\begin{myenumerate}
	%----
	\item For every $P_j \in S_q$, request output for every $P_k \in S_q \setminus \{P_j\}$ with $\sid^{(q)}_{jk}$ from $\FAcast$ until $(P_j,\Acast,\sid^{(q)}_{jk},\OK_q(j,k))$ is received.
	%----
	\item Initialize a set $\C_q$ to $\phi$. Construct a consistency graph $G^i_q$ with $S_q$ as the vertex set.
	%----
	\item Add the edge $(P_j,P_k)$ to $G^i_q$ if $(P_j,\Acast,\sid^{(q)}_{jk},\OK_q(j,k))$ and $(P_k,\Acast,\sid^{(q)}_{kj},\OK_q(k,j))$  is received from $\FAcast$. 
	%----
	\end{myenumerate}
%----
\item {\bf Identification of core sets} :  If $P_i$ is $P_{\D}$, then execute the following steps.
	%----
	\begin{myenumerate}
	%----
	\item For each $S_q \in \ShareSpec$, once a set $\W_q$ of parties which form a clique in $G^{\D}_q$ is identified, such that $\W_q = \ S_q \setminus Z$ for some $Z \in \AdvStructure$, then assign $\C_q \coloneqq \W_q$.
	%----
	\item Upon computing non empty $\C_q$ for each $S_q \in \ShareSpec$, send $(\Sender,\Acast,\sid_{\D},\{ \C_q \}_{S_q \in \ShareSpec})$, where $\sid_{\D} = \sid || \D$.
	%----
	\end{myenumerate}
%----
\item {\bf Share computation} : Execute the following steps.
	%----
	\begin{myenumerate}
	%----
	\item For each $S_q \in \ShareSpec$ such that $P_i \in S_q$, set $[s]_q$ to $\bot$.
	%----
	\item Request output with $\sid_{\D}$ from $\FAcast$ until $(\Sender,\Acast,\sid_{\D},\{ \C_q \}_{S_q \in \ShareSpec})$ is received.
	%----
	\item Wait until the parties in $\C_q$ form a clique in $G^i_q$, such that $\C_q = S_q \setminus Z$ for some $Z \in \AdvStructure$, for all $S_q \in \ShareSpec$. Upon receiving $(\dist,\sid,q,s^{(q)})$ from a set of parties $\C'_q = \C_q \setminus Z$ for some $Z \in \AdvStructure$, set $[s]_q = s^{(q)}$.
	%----
	\item Upon setting $[s]_q$ to some non $\bot$ value for each $S_q \in \ShareSpec$ such that $P_i \in S_q$, output $(\Share,\sid,P_{\D},\{[s]_q\}_{P_i \in S_q})$.
	%----
	\end{myenumerate}
%----
\end{myitemize}
%----
\end{protocolsplitbox}
%----

We next prove the security of the protocol by showing the existence of a simulator $\SimPVSS$, such that for any set of corrupted parties $Z^{\star} \in \AdvStructure$ and for all possible inputs, the outputs of parties and the view of the adversary in the real world protocol $\PiPerVSS$ is indistinguishable from the outputs of parties and the view of the adversary in an execution of with $\SimPVSS$ invoving $\FVSS$ in the ideal model. The steps of the simulator will be different depending on whether the dealer is corrupt of honest.

If the dealer is {\it honest}, then the simulator interacts with $\FVSS$ and receives the outputs of the corrupt parties, corresponding to the sets $S_q \in \ShareSpec$ which they are a part of. The simulator then distributed these shares on the behalf of the dealer, as well as performs pairwise consistency tests on the behalf of the honest parties. If $\Adv$ queries $\FAcast$ for the result of any test involving an honest party, the simulator provides the appropriate result. In addition, the simulator records the result of any test involving corrupt parties which $\Adv$  sends to $\FAcast$. Based on these, the simulator finds core sets for each $S_q$ and sends these as output to $\Adv$ upon request.

If the dealer is {\it corrupt}, the simulator plays the role of honest parties corresponding to $\PiPerVSS$. This involves recording shares which $\Adv$ distributes to any honest party, as well as performing pairwise consistency tests on their behalf. If the $\Adv$ sends core sets for each $S_q \in \ShareSpec$ as input to $\FAcast$, then the simulator checks if these are {\it valid}, and accordingly, sends the shares held by {\it honest} parties in these core sets as the input shares to $\FVSS$. The simulator is presented in Figure \ref{fig:SimPVSS}.

%----
\begin{simulatorsplitbox}{$\SimPVSS$}{Simulator for the protocol $\PiPerVSS$ where $\Adv$ corrupts the parties in set $Z^{\star}$, where $Z^{\star} \in \AdvStructure$}{fig:SimPVSS}
	\justify
%----
$\SimPVSS$ constructs virtual real-world honest parties and invokes the real-world adversary $\Adv$. The simulator simulates the view of
 $\Adv$, namely its communication with $\Env$, the messages sent by the honest parties and the interaction with $\FAcast$. 
  In order to simulate $\Env$, the simulator $\SimPVSS$ forwards every message it receives from 
   $\Env$ to $\Adv$ and vice-versa.  The simulator then simulates the various phases of the protocol as follows, depending upon whether the dealer is honest or corrupt. \\~\\
%---
 \centerline{\underline{\bf Simulation when $\D$ is Honest}} 
%----
\noindent {\bf Interaction with $\FVSS$}: the simulator interacts with the functionality $\FVSS$ and receives a request based delayed output $(\Share,\sid,P_{\D},\{[s]_q\}_{S_q \cap Z^{\star} \neq \phi})$\\[.2cm]
%----
\noindent {\bf Distribution of shares by the dealer}: On the behalf of the dealer, the simulator sends $(\dist,\sid,[s]_q,q)$ to all parties $P_i \in Z^{\star} \cap S_q$\\[.2cm]
%----     
 \noindent {\bf Pair-wise Consistency Tests}: For each $S_q \in \SharingSpec$ such that $S_q \cap Z^{\star} \neq \phi$, for each party $P_i \in S_q \cap Z^{\star}$, the simulator does the following on the behalf of every honest party $P_j \in S_q \setminus Z^{\star}$.
 	\begin{myitemize}
 	\item[--] Send $(\test,\sid,q,s^{(q)}_j)$ to $\Adv$, where $s^{(q)}_j = [s]_q$.
 	\item[--] If $\Adv$ sends $(\test,\sid,q,s^{(q)}_i)$ on the behalf of $P_i$ to $P_j$, then record it.
 	\end{myitemize}
%-----
 \noindent {\bf Results of Consistency Tests and Public Announcement}: 
\begin{myitemize}
\item[--] If, for some $S_q \in \SharingSpec$, $\Adv$ queries $\FAcast$ with $\sid^{(q)}_{ij} = \sid || q || i || j$ for parties $P_i \in S_q \setminus Z^{\star}$ and $P_j \in S_q$, then the simulator provides output on the behalf of $\FAcast$ as follows.
 	\begin{myitemize}
 	\item[--] If $P_j \in S_q \setminus Z^{\star}$, then send the output $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$.
 	\item[--] Else, if $(\test,\sid,q,s^{(q)}_j)$ sent by $\Adv$ on the behalf of party $P_j \in S_q \cap Z^{\star}$ to $P_i$ has been recorded, if $s^{(q)}_j = [s]_q$, send the output $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$.
 	\end{myitemize} 
\item[--] If, for some $S_q \in \SharingSpec$, $\Adv$ sends $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ on the behalf of $P_i \in S_q \cap Z^{\star}$ for some $P_j \in S_q$ to $\FAcast$ with $\sid^{(q)}_{ij} = \sid || q || i || j$, then the simulator records it. 
\end{myitemize}
%-----
\noindent {\bf Construction of $\C_q$ for each $S_q \in \SharingSpec$ and Public Announcement}: 
\begin{myitemize}
\item[--] For each $S_q \in \ShareSpec$, the simulator plays the role of $P_{\D}$ and adds edge $(P_i,P_j)$ to $G^{\D}_q$ if the following hold.
	\begin{myitemize}
	\item[--] $P_i,P_j \in S_q$.
	\item[--] One of the following is true.
		\begin{myitemize}
		\item $P_i,P_j \in S_q \setminus Z^{\star}$.
		\item If $P_i \in S_q \cap Z^{\star}$ and $P_j \in S_q \setminus Z^{\star}$, then the simulator has recorded $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ sent by $\Adv$ to $\FAcast$, and recorded $(\test,\sid,q,s^{(q)}_i)$ such that $s^{(q)}_i = [s]_q$.
		\item If $P_i, P_j \in S_q \cap Z^{\star}$, then the simulator has recorded $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ and $(P_j,\Acast,\sid^{(q)}_{ji},\OK_q(j,i))$ sent by $\Adv$ on behalf of $\FAcast$.
		\end{myitemize}
	\end{myitemize}
\item[--] For each $S_q \in \ShareSpec$, the simulator finds valid $\C_q$ which forms a clique in $G^{\D}_q$, such that $\C_q = S_q \setminus Z$ for some $Z \in \AdvStructure$. When $\Adv$ requests output from $\FAcast$ with $\sid_{\D} = \sid || \D$, the simulator sends the output $(\Sender,\Acast,\sid_{\D},\{\C_q\}_{S_q \in \ShareSpec})$ on the behalf of $\FAcast$.
\end{myitemize}
%---
% \noindent {\bf Verification of $\C_q$ for each $S_q \in \SharingSpec$}: \\[.2cm]
%--- 
% \noindent {\bf Share Computation}:  \\~\\
%---   
 \centerline{\underline{\bf Simulation when $\D$ is Corrupt}} 
 %---
  In this case, the simulator $\SimPVSS$ interacts with $\Adv$ during the various steps of $\PiPerVSS$ as follows. \\[.2cm]
%---
%----
\noindent {\bf Distribution of shares by the dealer}: If $\Adv$ sends $(\dist,\sid,q,v)$ on the behalf of $\D$ to party $P_i \in S_q \setminus Z^{\star}$, then the simulator records it and sets $s^{(q)}_i$ to be $v$. \\[.2cm]
%----     
 \noindent {\bf Pair-wise Consistency Tests}: For each $S_q \in \SharingSpec$ such that $S_q \cap Z^{\star} \neq \phi$, for each party $P_i \in S_q \cap Z^{\star}$, the simulator does the following for every honest party $P_j \in S_q \setminus Z^{\star}$.
 	\begin{myitemize}
 	\item[--] If $s^{(q)}_j$ has been set to some value, then send $(\test,\sid,q,s^{(q)}_j)$ to $\Adv$ on the behalf of $P_j$.
 	\item[--] If $\Adv$ sends $(\test,\sid,q,s^{(q)}_i)$ on the behalf of $P_i$ to $P_j$, then record it. 
 	\end{myitemize}
%-----
 \noindent {\bf Results of Consistency Tests and Public Announcement}: 
\begin{myitemize}
\item[--] If, for some $S_q \in \SharingSpec$, $\Adv$ queries $\FAcast$ with $\sid^{(q)}_{ij} = \sid || q || i || j$ for parties $P_i \in S_q \setminus Z^{\star}$ and $P_j \in S_q$, then the simulator provides output on the behalf of $\FAcast$, if $s^{(q)}_i$ has been set to some value, as follows.
 	\begin{myitemize}
 	\item[--] If $P_j \in S_q \setminus Z^{\star}$, then if  $s^{(q)}_j$ has been set to some value such that $s^{(q)}_i = s^{(q)}_j$, send the output $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$.
 	\item[--] Else, if $(\test,\sid,q,s^{(q)}_j)$ sent by $\Adv$ on the behalf of party $P_j \in S_q \cap Z^{\star}$ to $P_i$ has been recorded, if $s^{(q)}_j = s^{(q)}_i$, send the output $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$.
 	\end{myitemize} 
\item[--] If, for some $S_q \in \SharingSpec$, $\Adv$ sends $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ on the behalf of $P_i \in S_q \cap Z^{\star}$ for some $P_j \in S_q$ to $\FAcast$ with $\sid^{(q)}_{ij} = \sid || q || i || j$, then the simulator records it. 
\end{myitemize}
%-----
\noindent {\bf Construction of $\C_q$ for each $S_q \in \SharingSpec$}: For each $S_q \in \ShareSpec$, the simulator plays the role of each honest party $P_i \in S_q \setminus Z^{\star}$ and adds edge $(P_j,P_k)$ to $G^{i}_q$ if the following hold.
\begin{myitemize}
	\item[--] $P_j,P_k \in S_q$.
	\item[--] One of the following is true.
		\begin{myitemize}
		\item If $P_i,P_j \in S_q \setminus Z^{\star}$, then the simulator set $s^{(q)}_i$ and $s^{(q)}_j$ such that $s^{(q)}_i = s^{(q)}_j$.
		\item If $P_i \in S_q \cap Z^{\star}$ and $P_j \in S_q \setminus Z^{\star}$, then the simulator has recorded $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ sent by $\Adv$ to $\FAcast$, recorded $(\test,\sid,q,s^{(q)}_i)$ and set $s^{(q)}_j$ to a value such that $s^{(q)}_j = s^{(q)}_i$.
		\item If $P_i, P_j \in S_q \cap Z^{\star}$, then the simulator has recorded $(P_i,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ and $(P_j,\Acast,\sid^{(q)}_{ji},\OK_q(j,i))$ sent by $\Adv$ on behalf of $\FAcast$.
		\end{myitemize}
\end{myitemize}
%---
\noindent {\bf Verification of $\C_q$ for each $S_q \in \SharingSpec$}: If $\Adv$ sends $(\Sender,\Acast,\sid_{\D},\{\C_q\}_{S_q \in \ShareSpec})$ to $\FAcast$, then the simulator plays the role of the honest parties and verifies if $\C_q$ is valid for each $S_q \in \ShareSpec$. If each $\C_q$ is valid, then the simulator sends $(\Share,\sid,P_{\D},\{[s]_q\}_{S_q \in \ShareSpec})$ to $\FVSS$, where $[s]_q$ is set to $s^{(q)}_i$ for some $P_i \in \C_q \setminus Z^{\star}$. \\[.2cm]
\commentAA{Simulator written ommiting share computation, since no extra messages are sent by honest parties for this. Not sure if this is right, please check once.}
%--- 
% \noindent {\bf Share Computation}:  \\~\\ 
%--- 
\end{simulatorsplitbox}   
%----


%----
\end{comment}


==> AppStatAMPC.tex <==
\section{Statistically-Secure AMPC}
\label{app:Statistical}


%----
\subsection{Asynchronous Information Checking Protocol}
%---

In this section, we formally prove the properties of our instantiation of AICP. While proving these properties, we assume that $\AdvStruct$ satisfies the $\Q^{(3)}(\PartySet,\AdvStruct)$ condition. We first show that when $P_S$, $P_I$ and $P_R$ are honest, then all honest parties set the local bit indicating that the authentication has completed to $1$. Furthermore, $P_R$ will {\it accept} the signature {\it revealed} by $P_I$.

\begin{lemma}
%----
\label{lemma:AICPCorrectness}
%----
If $P_S, P_I$ and $P_R$ are {\it honest}, then all (honest) parties $P_i$ set $\authCompleted^{(\sid,i)}_{P_S,P_I,P_R}$ to $1$ during $\Auth$. Moreover, $P_R$ outputs $\vec{S}$ at the end of $\Reveal$.  
%----
\end{lemma}
%----
\begin{proof}
%----
Let $P_S,P_I$ and $P_R$ be honest. Let $\Hon$ be the set of honest parties in $\PartySet$. We first show that each honest party $P_i$ sets $\authCompleted^{(\sid,i)}_{P_S,P_I,P_R}$ to $1$ during $\Auth$. During $\Auth$, $P_S$ will select and send signing polynomials to $P_I$, and corresponding verification points to each verifier. Each honest verifier will eventually receive its verification point, and send a message indicating this to $P_I$. Hence, $P_I$ will eventually find a set $\R = \PartySet \setminus Z$, for some $Z \in \AdvStructure$, where each verifier in $\R$ has indicated that it has received its verification point. This is because $\Hon = \PartySet \setminus Z^{\star}$. $P_I$ will then randomly choose $d \in \F \setminus \{0\}$, compute $B(x) = dF(x) + M(x)$, and send $(d,B(x),\R)$ to $\FAcast$. Upon request with $\sid_I$, each party including $P_S$ will receive this as output from $\FAcast$. $P_S$ will then verify that $B(\alpha_j) = dv_j + m_j$ for all verifiers $P_j \in \R$, which will hold true since $P_I$ is honest and will correctly compute $B(x)$, and send message $\OK$ to $\FAcast$. Upon request with $\sid_S$, each honest verifier $P_i$ will receive this message from $\FAcast$, and set $\authCompleted^{(\sid,i)}_{P_S,P_I,P_R}$ to $1$. Furthermore, no honest verifier $P_i$ will add $P_S$ to $\LocalDiscarded^{(i)}$, since $B(\alpha_i) = dv_i + m_i$ will hold true.

In $\Reveal$, $P_I$ will send $F(\cdot)$ to $P_R$, and each honest verifier $P_i \in \Hon \cap \R$ will send its verification points $(\alpha_i,v_i,m_i)$ to $P_R$. For each such point, $v_i = F(\alpha_i)$ holds true, and the point will be {\it accepted}. Since $\Hon \cap \R = \R \setminus Z^{\star}$, $P_R$ will eventually receive points from a set of parties $\R' = \R \setminus Z$, which are {\it accepted}, for some $Z \in \AdvStructure$. Hence, $P_R$ will output $\vec{S}$.  
%----
\end{proof}

We next show that when $P_S,P_I$ and $P_R$ are {\it honest}, then the adversary does not learn anything about the vector of secrets $\vec{S}$ during either $\Auth$ or $\Reveal$.

\begin{lemma}
%----
\label{lemma:AICPPrivacy}
%----
If $P_S, P_I$ and $P_R$ are {\it honest}, then the view of adversary throughout is independent of $\vec{S}$. 
%----
\end{lemma}
%----
\begin{proof}
%----
We note that $t$ can be the maximum number of parties which can be corrupted. Without loss of generality, assume that the parties $P_1,\ldots,P_{t'} \in \PartySet$ are under the control of $\Adv$, where $t' \leq t$, and $t' = |Z^{\star}|$. During $\Auth$, $\Adv$ learns the values $((\alpha_1,v_1,m_1),\ldots,(\alpha_{t'},v_{t'},m_{t'}))$. However, since $F(\cdot)$ is of degree $t+L$, for every candidate $\vec{S} = (s^{(1)},\ldots,s^{(L)}) \in \F^{(L)}$, $|\F|^{t-t'}$ possible candidate polynomials for $F(\cdot)$ which are consistent with $v_1 ,\ldots,v_{t'}$ can be defined. $\Adv$ also learns the value of $d$, $B(x) = dF(x) + M(x)$ and the set $\R$ of supporting verifiers. However, since $M(\cdot)$ is chosen uniformly at random, for every possible polynomial $M(x)$ which is consistent with $m_1,\ldots,m_{t'}$, there is a unique $F(x) = d^{-1}\cdot(B(x) - M(x))$ of degree $L+t$, which is consistent with $v_1,\ldots,v_{t'}$. Furthermore, from the proof of Lemma \ref{lemma:AICPCorrectness}, $P_S$ sends an $\OK$ message to $\FAcast$, since $B(\alpha_j) = dv_j + m_j$ for all verifiers $P_j \in \PartySet$. During $\Reveal$, $\Adv$ does not learn anything new, since the verification points and signing polynomials are sent privately to $P_R$.
%----
\end{proof}

We next show that with high probability, a corrupt intermediary $P_I$ cannot reveal a vector of secrets during $\Reveal$, which is {\it different} from that obtained from an honest $P_S$ during the corresponding instance of $\Auth$.

\begin{lemma}
%----
\label{lemma:AICPUnforgeability}
%----
Let $P_S$ and $P_R$ be {\it honest}, and suppose corrupt $P_I$ reveals 
     $\ICSig^{(\ell)}(P_S \rightarrow P_I \rightarrow P_R, \vec{S'^{(\ell)}})$ during $\ell = 1,\ldots,M$ instances of $(\Auth^{(\ell)},\Reveal^{(\ell)})$.
     If $P_R$ outputs $\vec{S'^{(\ell)}}$ during $\Reveal^{(\ell)}$, then {\it irrespective of the value of} $M$, except with probability at most $\frac{L+t}{|\F| - L}$, the condition
     $\vec{S'^{(\ell)}} = \vec{S^{(\ell)}}$ holds.
%----
\end{lemma}
%----
\begin{proof}
%----
Let $\Hon$ be the set of honest parties in $\PartySet$. We fix a value of $\ell \in \{1,\ldots,M\}$ for which $P_R$ has obtained output in $\Reveal^{(\ell)}$. Since $P_R$ has obtained an output as part of the protocol $\Reveal^{(\ell)}$, $P_R$ has received some polynomial $F'(x)$ of degree $t+L$ from $P_I$, and has set $\authCompleted^{(\sid_\ell,R)}_{P_S,P_I,P_R}$ to $1$ during $\Auth^{(\ell)}$. Furthermore, $P_I \notin \LocalDiscarded^{(\ell,R)}$. There are now two cases.

\begin{myitemize}
\item[--] {\it $P_R$ received $\NOK$ along with $\vec{S'^{(\ell)}}$ as output from $\FAcast$} : In this case, since $P_S$ is honest, $\vec{S'^{(\ell)}} = \vec{S^{(\ell)}}$.
%----
\item[--] {\it $P_R$ received $\OK$ along with $(d,B(x),\R)$ as output from $\FAcast$} : This means that $B(\alpha_i) = dv_i + m_i$ for all honest verifiers $P_i \in \R$. Suppose that during $\Reveal^{(\ell)}$, $P_I$ sent $F'(x) \neq F(x)$ to $P_R$. We show that in this case, except with probability $\frac{L+t}{|\F| - L}$, $P_R$ will add $P_I$ to $\LocalDiscarded^{(\ell,R)}$. To prove this, we show that except with probability $\frac{L+t}{|\F| - L}$, the verification point of each honest verifier is {\it rejected}. Suppose that $P_R$ receives a point $(\alpha_i,v_i,m_i)$ from an honest verifier $P_i \in \Hon \cap \R$. This point can be {\it accepted} in the following two cases.
	\begin{myitemize}
	\item $v_i = F'(\alpha_i)$ : This is possible with probability at most $\frac{L+t}{|\F| - L}$. This is because $F'(x)$ and $F(x)$, being distinct polynomials of degree $L+t$, can have  at most $L+t$ points in common.
	\item $dv_i + m_i \neq B(\alpha_i)$ : This is impossible, since $P_S$ has verified that $B(\alpha_i) = dv_i + m_i$ for all verifiers $P_i \in \R$.
	\end{myitemize}
Since $\Hon \cap \R = \R \setminus Z^{\star}$, $P_R$ will eventually receive points from a set of parties $R' \subset \R$, such that $\R' = \R \setminus Z$ for some $Z \in \AdvStructure$, such that each point received is {\it rejected}. Also, the set of {\it corrupt} parties in $\R$ {\it cannot} form a candidate set for $\R'$. This is because since $\AdvStructure$ satisfies the $\Q^{(3)}(\PartySet,\AdvStructure)$ condition,  it satisfies the $\Q^{(2)}(\R,\AdvStructure)$ condition, and thereby, the $\Q^{(1)}(\R',\AdvStructure)$ condition. Hence, any candidate set of parties for $\R'$ must contain at least one honest party.
\end{myitemize}
We further note that once $P_I$ is added to $\LocalDiscarded^{(\ell,R)}$, $P_R$ will not obtain any output from $P_I$ as part of any later instance of $\Reveal$. Hence, irrespective of the value of $M$, except with probability $\frac{L+t}{|\F| - L}$, $\vec{S'^{(\ell)}} = \vec{S^{(\ell)}}$ for all instances of $\Reveal^{(\ell)}$ where $P_R$ obtains an output. 
%----
\end{proof}

We next show that if an honest $P_I$ completes the authentication phase and tries to reveal a vector of secrets to an honest $P_R$, then with high probability, $P_R$ will accept this vector of secrets.

\begin{lemma}
%----
\label{lemma:AICPNonRepudiation}
%----
Let $P_S$ be {\it corrupt} and $P_I, P_R$ be {\it honest}. Suppose that during $\ell = 1,\ldots,M$ instances of $(\Auth^{(\ell)},\Reveal^{(\ell)})$, $P_S$ gives $\ICSig(\sid_\ell,P_S \rightarrow P_I \rightarrow P_R, \vec{S'^{(\ell)}})$ to $P_I$. Suppose that $P_I$ sets $\authCompleted^{(\sid_\ell,I)}_{P_S,P_I,P_R}$ to $1$ during $\Auth^{(\ell)}$, for some $\ell \in \{1,\ldots,M\}$, and  $P_I$ reveals
    $\ICSig^{(\ell)}(P_S \rightarrow P_I \rightarrow P_R, \vec{S'^{(\ell)}})$ to $P_R$. Then, {\it irrespective of the value of} $M$, except with probability at most $\frac{n}{|\F|-1}$, $P_R$ outputs $\vec{S'^{(\ell)}}$ during $\Reveal^{(\ell)}$. 
%----
\end{lemma}
%----
\begin{proof}
%----
Let $\Hon$ be the set of honest parties in $\PartySet$. We fix a value of $\ell \in \{1,\ldots,M\}$ for which $P_I$ has set $\authCompleted^{(\sid_\ell,I)}_{P_S,P_I,P_R}$ to $1$ during $\Auth^{(\ell)}$. Suppose that $P_I$ reveals
    $\ICSig^{(\ell)}(P_S \rightarrow P_I \rightarrow P_R, \vec{S'^{(\ell)}})$ to $P_R$. Then, we show that except with probability at most $\frac{n}{|\F|-1}$, $P_R$ outputs $\vec{S'^{(\ell)}}$ during $\Reveal^{(\ell)}$. Since $P_I$ has set $\authCompleted^{(\sid_\ell,I)}_{P_S,P_I,P_R}$ to $1$, $P_I$ has received $(d,B(x),\R)$ from $\FAcast$, which means that $P_R$ will also eventually receive this from $\FAcast$. There are now two cases.
\begin{myitemize}
%----
\item[--] {\it $P_I$ received $\NOK$ along with $\vec{S''^{(\ell)}}$ as output from $\FAcast$} : In this case, $P_R$ will also eventually receive $\NOK$ along with $\vec{S''^{(\ell)}}$ as output from $\FAcast$. Hence, $P_R$ will set $\authCompleted^{(\sid_\ell,R)}_{P_S,P_I,P_R}$ to $1$ and output $\vec{S'^{(\ell)}}$ during $\Reveal^{(\ell)}$.
%----
\item[--] {\it $P_I$ received $\OK$ along with $(d,B(x),\R)$ as output from $\FAcast$} : Eventually, $P_R$ will also receive the message $\OK$ from $\FAcast$, and set $\authCompleted^{(\sid_\ell,R)}_{P_S,P_I,P_R}$ to $1$. Suppose that $P_R$ receives signing polynomial $F'(x)$ from $P_S$ during $\Auth^{(\ell)}$. We show that except with probability at most $\frac{n}{|\F|-1}$, the verification point $(\alpha_i,v_i,m_i)$ of {\it each} party $P_i$ in $\Hon \cap \R$ is {\it accepted} by $P_R$. To show this, we consider two cases. 
	\begin{myitemize}
	\item $v_i = F'(\alpha_i)$ : In this case, according to the protocol steps, $(\alpha_i,v_i,m_i)$ is {\it accepted}.
	\item $v_i \neq F'(\alpha_i)$ : In this case, we claim that $dv_i + m_i = B(\alpha_i)$ with a probability of at most $\frac{1}{|\F|-1}$. This is because this will be possible only when $P_I$ chooses $d$ such that $d = (M'(\alpha_i) - m_i)\cdot(v_i - F'(\alpha_i))^{-1}$, where $M'(\alpha_i)$ is the masking polynomial $P_I$ received from $P_S$ during $\Auth^{(\ell)}$. Since $d$ is chosen uniformly at random from $F \setminus \{0\}$, this happens with a probability of at most $\frac{1}{|\F|-1}$. Hence, except with a probability of at most $\frac{1}{|\F|-1}$, $(\alpha_i,v_i,m_i)$ will be {\it accepted}. Furthermore, in this case, from the protocol steps, $P_i$ adds $P_S$ to $\LocalDiscarded^{(i)}$ during $\Auth^{(\ell)}$.  
	\end{myitemize}
	It now follows from the union bound that the verification point of {\it every} honest party in $\R$ is {\it accepted}, except with a probability of at most $\frac{n}{|\F|-1}$. Since $\Hon \cap \R = \R \setminus Z^{\star}$, $P_R$ will eventually receive points from a set of parties $\R' = \R \setminus Z$, which are {\it accepted} except with a probability of $\frac{n}{|\F|-1}$, for some $Z \in \AdvStructure$. Hence, $P_R$ will output $\vec{S'^{(\ell)}}$.
\end{myitemize}
We further note that once $P_S$ is added to $\LocalDiscarded^{(i)}$ for some verifier $P_i \in \PartySet$ in an instance $\Auth^{(\ell)}$, then $P_i$ will  not be a part of the set of supporting verifiers for any later instance $\Auth^{(\ell')}$. Hence, $P_S$ can give each verifier an ``inconsistent" point only {\it once}, except with a probability of at most $\frac{1}{|\F|-1}$. By the union bound, it will follows that except with a probability of at most $\frac{n}{|\F|-1}$, $P_S$ will be added to $\LocalDiscarded^{(i)}$ for every honest verifier $P_i$ which has received an inconsistent verification point during any of the $M$ instances of $\Auth$. We now claim that irrespective of the value of $M$, except with a probability of at most $\frac{n}{|\F|-1}$, $P_S$ can ``cheat" a maximum of $n$ times, once with respect to each verifier. To prove this, for any instance of $\Auth$, we consider the set $\R$ of supporting verifiers. Since $\AdvStructure$ satisfies the $\Q^{(3)}(\PartySet,\AdvStructure)$ condition, and since $\R = \PartySet \setminus Z$ for some $Z \in \AdvStructure$, $\AdvStructure$ must satisfy the $\Q^{(2)}(\R,\AdvStructure)$ condition. This implies that $\R$ has to include at least one honest party. However, once a verifier $P_i$ adds $P_S$ to $\LocalDiscarded^{(i)}$, according to the protocol steps, it does not send the message $(\Received,i)$ to $P_I$, and cannot be included into the set $\R$. Thus, $\Auth$ will not complete for an honest $P_I$ after every honest verifier has discarded $P_S$. Hence, irrespective of the value of $M$, $P_R$ outputs  $\vec{S'^{(\ell)}}$ revealed by honest $P_I$ during $\Reveal^{(\ell)}$, except with a probability of at most $\frac{n}{|\F|-1}$.
%----
\end{proof}
%----

We next prove a Lemma regarding the communication complexity of $\Auth$ and $\Reveal$.

\begin{lemma}
\label{lemma:AICPCommunication}
%----
$\Auth$ requires a communication of $\Order((n+L) \cdot \log{|\F|})$ bits, $n$ calls to $\FAcast$ with $\Order(\log(n))$ bit messages and 1 call to $\FAcast$ with $\Order(L \cdot \log{|\F|})$ bit messages, while $\Reveal$ requires a communication of $\Order((n+L)\cdot \log{|\F|})$ bits.
%----
\end{lemma}
%----
\begin{proof}
%----
During $\Auth$, $P_S$ sends $F(x)$ and $M(x)$ of degree at most $t+L$ to $P_I$, and verification points to each verifier. This requires a communication of $\Order((n+L) \cdot \log{|\F|})$ bits. In addition, each verifier $P_i \in \PartySet$ broadcasts a message $(\Received,\sid,i)$. This requires $n$ calls to $\FAcast$ with $\Order(\log(n))$ bit messages. To announce an $\OK$ or $\NOK$ message, $P_S$ makes 1 call to $\FAcast$. To send $\vec{S} = (s^{(1)},\dots,s^{(L)})$ for an $\NOK$ message, this requires sending a message with $\Order(L \cdot \log{|\F|})$ bits. During $\Reveal$, $P_I$ sends $F(x)$ to $P_R$, and each verifier sends its verification point. This requires a communication of $\Order((n+L)\cdot \log{|\F|})$ bits.
%----
\end{proof}
%----

%----
\subsection{Statistical VSS Protocol}
%---

In this section, we prove the properties of $\PiStatVSS$ stated in Theorem \ref{thm:StatVSS}. Throughout the section, we assume that $\AdvStruct$ satisfies the $\Q^{(3)}(\PartySet,\AdvStruct)$ condition, and thus, $\ShareSpec$ satisfies the $\Q^{(2)}(\ShareSpec,\AdvStruct)$ condition. \\ \\
%---
{\bf Theorem \ref{thm:StatVSS}}
%---
 {\it Consider a static malicious adversary $\Adv$ characterized by an adversary-structure $\AdvStructure$, satisfying the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition
  and let  $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$ be the sharing specification.\footnote{Hence $\ShareSpec$
   satisfies the $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition.} 
  Then protocol $\PiStatVSS$ UC-securely realizes the functionality $\FVSS$
   with statistical security in the $\FAcast$-hybrid model, in the 
   presence of $\Adv$.
   To share $L$ values, the protocol makes $\Order(|\AdvStructure| \cdot n^4)$ calls to $\FAcast$ with $\Order(\log{n})$ bit messages, $\Order(|\AdvStructure| \cdot n^3)$ calls to $\FAcast$ with $\Order(L \cdot \log{|\F|})$ bit messages
    and additionally incurs a communication of 
   $\Order(|\AdvStructure| \cdot ( n^4+n^3 \cdot L) \log{|\F|})$ bits. By replacing the calls to $\FAcast$ with protocol $\PiAcast$, the protocol incurs a total communication of $\Order(|\AdvStructure| \cdot (n^4 + n^3 \cdot L )\log{|\F|} + n^4 \log{n}))$
   bits.}
%-----
\begin{proof}
%----
In the protocol, $|\ShareSpec| = |\AdvStructure|$. The dealer needs to send the share $s^{(q)}$ to all the parties in $S_q$, and this requires a communication of $\Order(|\AdvStruct| \cdot n \cdot L \log{|\F|})$ bits. As part of pairwise consistency checks, for every $S_q \in \ShareSpec$, each party as $P_S$ sends a signature on $s^{(q)}$ to every other party in $S_q$ as intermediary, for every party in $\PartySet$ as receiver. This incurs a communication of $\Order(|\AdvStructure| \cdot n^3)$ times that of $\Auth$, which amounts to $\Order(|\AdvStructure| \cdot n^4)$ calls to $\FAcast$ with $\Order(\log{n})$ bit messages, $\Order(|\AdvStructure| \cdot n^3)$ calls to $\FAcast$ with $\Order(L \cdot \log{|\F|})$ bit messages
    and a communication of 
   $\Order(|\AdvStructure| \cdot ( n^4+n^3 \cdot L) \log{|\F|})$ bits. While announcing the results of pairwise consistency checks and broadcasting core sets, for each $S_q \in \ShareSpec$, $\Order(n^2)$ calls to $\FAcast$ are made with $\Order(\log{n})$ bit messages. Additionally, revealing $s^{(q)}$ to each party in $S_q \setminus \C_q$ for every pair of parties in $\C_q$ as possible senders and itermediaries, for every $S_q \in \ShareSpec$, requires a communication of $\Order(|\AdvStructure| \cdot n^3)$ times that of $\Reveal$. This amounts to the communication of $\Order(|\AdvStructure| \cdot ( n^4+n^3 \cdot L) \log{|\F|})$ bits.

We next prove the security of the protocol for $L=1$; the proof for be generalized for any value of $L$. Let $\Adv$ be an arbitrary adversary, attacking the protocol $\PiPerVSS$ by corrupting a set of parties
  $Z^{\star} \in \AdvStructure$ and let $\Env$ be an arbitrary environment. We show the existence of a simulator $\SimSVSS$, such that for any
 $Z^{\star} \in \AdvStructure$,
  the outputs of the honest parties and the view of the adversary in the 
   protocol $\PiStatVSS$ is indistinguishable from the outputs of the honest parties and the view of the adversary in an execution in the ideal world involving 
  $\SimSVSS$ and $\FVSS$, except with a probability of $n^2 \cdot \errorAICP$. The simulator is similar to that of $\SimSVSS$, except that the simulator has to simulate giving and accepting signatures on the behalf of honest parties, as part of pairwise consistency checks. In addition, for each $S_q \in \ShareSpec$, the simulator has to simulate revealing signatures to corrupt parties outside the core set $\C_q$ on the behalf of honest parties in $\C_q$. The simulator is presented in Figure \ref{fig:SimSVSS}.

%----
\begin{simulatorsplitbox}{$\SimSVSS$}{Simulator for the protocol $\PiStatVSS$ where $\Adv$ corrupts the parties in set $Z^{\star}$, where $Z^{\star} \in \AdvStructure$}{fig:SimSVSS}
	\justify
%----
$\SimPVSS$ constructs virtual real-world honest parties and invokes the real-world adversary $\Adv$. The simulator simulates the view of
 $\Adv$, namely its communication with $\Env$, the messages sent by the honest parties and the interaction with $\FAcast$. 
  In order to simulate $\Env$, the simulator $\SimPVSS$ forwards every message it receives from 
   $\Env$ to $\Adv$ and vice-versa.  The simulator then simulates the various phases of the protocol as follows, depending upon whether the dealer is honest or corrupt. \\~\\
%---
 \centerline{\underline{\bf Simulation When $P_{\D}$ is Honest}} 
%----
\noindent {\bf Interaction with $\FVSS$}: the simulator interacts with the functionality $\FVSS$ and receives a request based delayed output
  $(\Share,\sid,P_{\D},\{[s]_q\}_{S_q \cap Z^{\star} \neq \emptyset})$, on the behalf of the parties in $Z^{\star}$.\\[.2cm]
%----
\noindent {\bf Distribution of Shares by $P_{\D}$}: On the behalf of the dealer, the simulator sends $(\dist, \sid, P_{\D}, q, [s]_q)$ to $\Adv$, corresponding to 
 every $P_i \in Z^{\star} \cap S_q$. \\[.2cm]
%----     
 \noindent {\bf Pairwise Consistency Tests}: 
 \begin{myitemize}
 \item[--]  For each $S_q \in \SharingSpec$ such that $S_q \cap Z^{\star} \neq \emptyset$,
  corresponding to each $P_i \in S_q \cap Z^{\star}$, the simulator does the following.
 	\begin{myitemize}
 	\item  On the behalf of every party $P_j \in S_q \setminus Z^{\star}$ as signer, for every $P_k \in \PartySet$ as a receiver, give $\ICSig(\sid^{(P_\D,q)}_{j,i,k},P_j \rightarrow P_i \rightarrow P_k, s_{qj})$ to $\Adv$, where $s_{qj} = [s]_q$.
 	\item Upon receiving $\ICSig(\sid^{(P_\D,q)}_{i,j,k}, P_i \rightarrow P_j \rightarrow, P_k, s_{qi})$ from $\Adv$, sent on the behalf of $P_i$ as signer to $P_j \in S_q$ as an intermediary for $P_k \in \PartySet$ as a receiver, record it.
 	\end{myitemize}
 \item[--] For each $S_q \in \SharingSpec$, for every $P_i,P_j \in S_q \setminus Z^{\star}$ the simululator simulates giving $\ICSig(\sid^{(P_\D,q)}_{i,j,k},P_i \rightarrow P_j \rightarrow P_k,v)$ to $P_j$, for all parties $P_k \in \PartySet$, and interacts with $\Adv$ as part of this instance. Based on the appropriate condition, the simulator chooses $v$ as follows.
 	\begin{myitemize}
 	\item {$S_q \cap Z^{\star} \neq \phi$ : }Choose $v$ to be $[s]_q$. 
 	\item {$S_q \cap Z^{\star} = \phi$ : } Pick a random value $v$ from $\F$. 
 	\end{myitemize}
 
 \end{myitemize}
%-----
 \noindent {\bf Announcing Results of Consistency Tests}: 
\begin{myitemize}
\item[--] If for any $S_q \in \SharingSpec$, $\Adv$ requests an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$ corresponding to parties
 $P_i \in S_q \setminus Z^{\star}$ and $P_j \in S_q$, then the simulator provides output on the behalf of $\FAcast$ as follows.
 	\begin{myitemize}
 	\item If $P_j \in S_q \setminus Z^{\star}$, then send the output $(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$.
 	\item If $P_j \in (S_q \cap Z^{\star})$, then send the output $(P_i, \Acast ,\sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$, if the message $\ICSig(\sid^{(P_\D,q)}_{j,i,k},P_j \rightarrow P_i \rightarrow P_k, s_{qj})$ has been recorded 
	         on the behalf of $P_j$ as a signer, sent to party $P_i$ as an intermediary, for every party $P_k \in \PartySet$ as a receiver, such that $s_{qj} = [s]_q$ holds.	         	       
	\end{myitemize} 
\item[--] If for any $S_q \in \SharingSpec$ and any $P_i \in S_q \cap Z^{\star}$, 
 $\Adv$ sends $(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ to $\FAcast$
 with $\sid^{(P_{\D}, q)}_{ij}$ on the behalf of 
  $P_i$ for any $P_j \in S_q$, then the simulator records it. 
  Moreover, if $\Adv$ requests an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$, then 
  the simulator sends the output $(P_i, \Acast ,\sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ on the behalf of $\FAcast$.
  %---
\end{myitemize}
%-----
\noindent {\bf Construction of Core Sets and Public Announcement}: 
\begin{myitemize}
\item[--] For each $S_q \in \ShareSpec$, the simulator plays the role of $P_{\D}$ and adds edge $(P_i,P_j)$ to the graph $G^{(\D)}_q$ over the vertex set $S_q$, if the following hold.
	\begin{myitemize}
	\item $P_i,P_j \in S_q$.
	\item One of the following is true.
		\begin{myenumerate}
		\item $P_i,P_j \in S_q \setminus Z^{\star}$.
		\item If $P_i \in S_q \cap Z^{\star}$ and $P_j \in S_q \setminus Z^{\star}$, then the simulator has recorded 
		$(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ sent by $\Adv$ on the behalf of $P_i$ to $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$, and has recorded the message $\ICSig(\sid^{(P_\D,q)}_{i,j,k},P_i \rightarrow P_j \rightarrow P_k, s_{qi})$ on the behalf of $P_i$ as a signer, sent to party $P_j$ as an intermediary for every party $P_k \in \PartySet$ as a receiver, such that $s_{qi} = [s]_q$ holds.
		\item If $P_i, P_j \in S_q \cap Z^{\star}$, then the simulator has recorded $(P_i, \Acast, \sid^{(q)}_{ij}, \OK_q(i,j))$
		 and $(P_j, \Acast, \allowbreak \sid^{(q)}_{ji}, \OK_q(j,i))$ sent by $\Adv$ on behalf $P_i$ and $P_j$ respectively, to 
		 $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$ and $\FAcast$ with $\sid^{(P_{\D}, q)}_{ji}$.
		 %---		 
		\end{myenumerate}
	\end{myitemize}
\item[--] For each $S_q \in \ShareSpec$, the simulator finds the set $\C_q$ which forms a clique in $G^{\D}_q$, such that $S_q \setminus \C_q \in \AdvStructure$.
  When $\Adv$ requests output from $\FAcast$ with $\sid_{P_{\D}}$, 
  the simulator sends the output $(\Sender, \Acast, \sid_{P_{\D}}, \{\C_q\}_{S_q \in \ShareSpec})$ on the behalf of $\FAcast$.
\end{myitemize}
%-----
\noindent {\bf Output Computation}: For each $S_q \in \ShareSpec$, upon finding valid $\C_q \in G^\D_q$, simulator does the following for every $P_i \in (S_q \setminus \C_q) \cap Z^{\star}$, $P_j \in \C_q \setminus Z^{\star}$.
	\begin{myitemize}
	\item[--] Reveal $\ICSig(\sid^{(P_\D,q)}_{k,j,i},P_k \rightarrow P_j \rightarrow P_i, s_{qk})$ on the behalf of $P_j$ to $\Adv$ for every party $P_k \in \C_q \setminus \{P_j\}$, where $s_{qk} = [s]_q$.
	\end{myitemize}
%---
% \noindent {\bf Verification of $\C_q$ for each $S_q \in \SharingSpec$}: \\[.2cm]
%--- 
% \noindent {\bf Share Computation}:  \\~\\
%---   
 \centerline{\underline{\bf Simulation When $P_{\D}$ is Corrupt}} 
 %---
  In this case, the simulator $\SimPVSS$ interacts with $\Adv$ during the various phases of $\PiStatVSS$ as follows. \\[.2cm]
%---
%----
\noindent {\bf Distribution of shares by $P_{\D}$}: If $\Adv$ sends $(\dist, \sid, P_{\D}, q, v)$ 
 on the behalf of $P_{\D}$ to any party $P_i \in S_q \setminus Z^{\star}$, then the simulator records it and sets $s_{qi}$ to be $v$. \\[.2cm]
%----     
 \noindent {\bf Pairwise Consistency Tests}: 
 \begin{myitemize}
 \item[--] For each $S_q \in \SharingSpec$ such that 
  $S_q \cap Z^{\star} \neq \emptyset$, corresponding to each party $P_i \in S_q \cap Z^{\star}$ and each 
  $P_j \in S_q \setminus Z^{\star}$, the simulator does the following.
 	\begin{myitemize}
 	\item If $s_{qj}$ has been set to some value, then give $\ICSig(\sid^{(P_\D,q)}_{j,i,k},P_j \rightarrow P_i \rightarrow P_k, s_{qj})$ to $\Adv$ on the behalf of $P_j$ as signer, for every $P_k \in \PartySet$ as receiver.
 	\item Upon receiving $\ICSig(\sid^{(P_\D,q)}_{i,j,k}, P_i \rightarrow P_j \rightarrow, P_k, s_{qi})$ from $\Adv$, sent on the behalf of $P_i$ as signer to $P_j \in S_q$ as an intermediary for $P_k \in \PartySet$ as a receiver, record it.
 	\end{myitemize}
 \item[--] For each $S_q \in \SharingSpec$ such that 
  $S_q \cap Z^{\star} \neq \emptyset$, corresponding to each party $P_i, P_j \in S_q$, the simulator does the following.
  	\begin{myitemize}
  	\item Upon setting $s_{qi}$ to some value, simultate giving $\ICSig(\sid^{(P_\D,q)}_{i,j,k},P_i \rightarrow P_j \rightarrow P_k,s_{qi})$ to $P_j$, for all parties $P_k \in \PartySet$, and interact with $\Adv$ as part of this instance.
  	\end{myitemize}
 \end{myitemize}
 
%-----
 \noindent {\bf Announcing Results of Consistency Tests}: 
\begin{myitemize}
\item[--] If for any $S_q \in \SharingSpec$, $\Adv$ requests an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$ corresponding to
 parties $P_i \in S_q \setminus Z^{\star}$ and $P_j \in S_q$, then the simulator provides the 
  output on the behalf of $\FAcast$ as follows, if $s_{qi}$ has been set to some value.
 	\begin{myitemize}
 	\item If $P_j \in S_q \setminus Z^{\star}$, then send the output $(P_i,\Acast,\sid^{(P_{\D}, q)}_{ij},\OK_q(i,j))$, if
	$s_{qj}$ has been set to some value and $s_{qi} = s_{qj}$ holds.
 	\item If $P_j \in (S_q \cap Z^{\star})$, then send the output $(P_i, \Acast ,\sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$, if the message $\ICSig(\sid^{(P_\D,q)}_{j,i,k},P_j \rightarrow P_i \rightarrow P_k, s_{qj})$ has been recorded 
	         on the behalf of $P_j$ as a signer, sent to party $P_i$ as an intermediary, for every party $P_k \in \PartySet$ as a receiver, such that $s_{qj} = s_{qi}$ holds.
 	\end{myitemize} 
\item[--]  If for any $S_q \in \SharingSpec$ and any $P_i \in S_q \cap Z^{\star}$, 
 $\Adv$ sends $(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ to $\FAcast$
 with $\sid^{(P_{\D}, q)}_{ij}$ on the behalf of 
  $P_i$ for any $P_j \in S_q$, then the simulator records it. 
  Moreover, if $\Adv$ requests an output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$, then 
  the simulator sends the output $(P_i, \Acast ,\sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ on the behalf of $\FAcast$.
  \end{myitemize}
%-----
\noindent {\bf Construction of Core Sets}: For each $S_q \in \ShareSpec$, the simulator plays the role of 
 the honest parties $P_i \in S_q \setminus Z^{\star}$ and adds the edge $(P_j,P_k)$ to the graph $G^{(i)}_q$ over vertex set $S_q$, if the following hold.
\begin{myitemize}
	\item[--] $P_j, P_k \in S_q$.
	\item[--] One of the following is true.
		\begin{myitemize}
		\item If $P_j, P_k \in S_q \setminus Z^{\star}$, then the simulator has set $s_{qj}$ and $s_{qk}$ to some values, such that $s_{qj} = s_{qk}$.
		\item If $P_j \in S_q \cap Z^{\star}$ and $P_k \in S_q \setminus Z^{\star}$, then the simulator has recorded 
		$(P_j, \Acast, \sid^{(P_{\D}, q)}_{jk}, \OK_q(j,k))$ sent by $\Adv$ on the behalf of $P_j$ to $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$, and has recorded the message $\ICSig(\sid^{(P_\D,q)}_{j,k,m},P_j \rightarrow P_k \rightarrow P_m, s_{qj})$ on the behalf of $P_j$ as a signer, sent to party $P_k$ as an intermediary for every party $P_m \in \PartySet$ as a receiver, and has set $s_{qk}$ to a value such that $s_{qj} = s_{qk}$ holds.
		\item If $P_j, P_k \in S_q \cap Z^{\star}$, then the simulator has recorded 
		$(P_j, \Acast, \sid^{(P_{\D}, q)}_{jk}, \OK_q(j, k))$ and $(P_k, \Acast, \allowbreak \sid^{(P_{\D}, q)}_{kj}, \OK_q(k, j))$ sent by $\Adv$ on behalf of
		$P_j$ and $P_k$ respectively, to $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$ and $\FAcast$ with $\sid^{(P_{\D}, q)}_{kj}$. 		
		\end{myitemize}
\end{myitemize}
%---
\noindent {\bf Verification of Core Sets and Interaction with $\FVSS$}:
   %----
      \begin{myitemize}
      %----
        \item If  $\Adv$ sends $(\Sender, \Acast, \sid_{P_{\D}}, \{\C_q\}_{S_q \in \ShareSpec})$ to $\FAcast$ with $ \sid_{P_{\D}}$ on the behalf of
  $P_{\D}$, then the simulator records it. Moreover, if $\Adv$ requests an output from $\FAcast$ with $ \sid_{P_{\D}}$, then on the behalf
  of $\FAcast$, the simulator sends the output $(P_{\D}, \Acast , \sid_{P_{\D}}, \{\C_q\}_{S_q \in \ShareSpec})$.
       %---
       \item If simulator has recorded the sets  $ \{\C_q\}_{S_q \in \ShareSpec}$, then it plays 
     the role of the honest parties and verifies if $\C_q$ is valid for each $S_q \in \ShareSpec$, by checking
     if $S_q \setminus \C_q \in \AdvStructure$ and if $\C_q$ constitutes a clique in the graph $G^{(i)}_q$ of every party $P_i \in \PartySet \setminus Z^{\star}$.
    If each $\C_q$ is valid, then the simulator sends $(\Share, \sid, P_{\D}, \{s_q\}_{S_q \in \ShareSpec})$ to $\FVSS$, where $s_q$ is set to 
     $s_{qi}$ for any $P_i \in \C_q \setminus Z^{\star}$. 
     \end{myitemize}
     
%--- 
\end{simulatorsplitbox}   
%----

We now prove a series of claims, which helps us to prove the theorem. We start with an {\it honest}
 $P_{\D}$.
%-----
\begin{claim}
\label{claim:SVSSHonestDPrivacy}
%---
If $P_{\D}$ is honest, then the view of $\Adv$ in the simulated execution of $\PiStatVSS$ with $\SimPVSS$ is identically distributed to the view of $\Adv$ in the real execution of $\PiStatVSS$ involving honest parties.
%---
\end{claim}
%----
\begin{proof}
%----
Let $\ShareSpec^{\star} \defined
  \{S_q \in \ShareSpec \mid S_q \cap Z^{\star} \neq \emptyset \}$. Then the 
   view of $\Adv$ during the various executions consists of the following.
\begin{myenumerate}
\item[--] The shares $\{[s]_q\}_{S_q \in \ShareSpec^{\star}}$ distributed by $P_{\D}$: In the real execution, $\Adv$ receives $[s]_q$ from $P_{\D}$ for each $S_q \in \ShareSpec^{\star}$. In the simulated execution, the simulator provides this to $\Adv$ on behalf of $P_{\D}$. Clearly, the distribution of the shares is identical in both the
 executions.
%----
\item[--] Corresponding to every $S_q \in \ShareSpec^{\star}$, the signature
  $\ICSig(\sid^{(P_\D,q)}_{j,i,k},P_j \rightarrow P_i \rightarrow P_k, s_{qj})$ received from party $P_j \in S_q \setminus Z^{\star}$ for every party $P_k \in \PartySet$, sent to every party $P_i \in S_q \cap Z^{\star}$
    as part of pairwise consistency tests: While each $P_j$ sends this to $\Adv$ in the real execution, the simulator sends this on the behalf of $P_j$ in the simulated execution.
    Clearly, the distribution of the messages is identical in both the executions.    
%----
\item[--] Corresponding to every $S_q \in \ShareSpec$, the view generated when $P_i$ gives $\ICSig(\sid^{(P_\D,q)}_{i,j,k},P_i \rightarrow P_j \rightarrow P_k, v))$ to $P_j$ for all $P_k \in \PartySet$, where $P_i , P_j \in S_q \setminus Z^{\star}$ : We consider the following two cases.
	\begin{myitemize}
	\item $S_q \in \ShareSpec^{\star}$ : In both the real and ideal execution, the value of $v$ is $[s]_q$. Since the simulator simulates the interaction of honest parties with $\Adv$ during the ideal execution, the distribution of messages is identical in both the executions.
	\item $S_q \notin \ShareSpec^{\star}$ : In the ideal execution, the simulator chooses $v$ to be a random value from $\F$, while in the real execution, $v$ is $[s]_q$. However, due to the privacy property of AICP (Lemma \ref{lemma:AICPPrivacy}), the view of $\Adv$ is independent of the value of $v$ in either of the executions. Hence, the distribution of the messages is identical in both the executions. 
	\end{myitemize}
%----
\item[--] For every $S_q \in \ShareSpec$ and every $P_i,P_j \in S_q$, the outputs $\OK_q(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$
 of the pairwise consistency tests, received as output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$: 
 To compare the distribution of these messages in the two executions,
  we consider the following cases, considering an arbitrary $S_q \in \ShareSpec$ and arbitrary $P_i, P_j \in S_q$.
	\begin{myitemize}
	%----
	\item[--] $P_i,P_j \in S_q \setminus Z^{\star}$: In both the executions, 
	 $\Adv$ receives $\OK_q(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ as the output from $\FAcast$ with $\sid^{(P_{\D}, q)}_{ij}$.
	%----
	\item[--] $P_i \in S_q \setminus Z^{\star}, P_j \in (S_q \cap Z^{\star}) $:  In both the 
	 executions, $\Adv$ receives $\OK_q(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \allowbreak \OK_q(i,j))$ as the output from $\FAcast$ with 
	 $\sid^{(P_{\D}, q)}_{ij}$ if and only if $\Adv$ gave $\ICSig(\sid^{P_\D,q}_{j,i,k},P_j \rightarrow P_i \rightarrow P_k,s_{qj})$ on the behalf of $P_j$ to $P_i$ for all parties $P_k \in \PartySet$ such that $s_{qj} = [s]_q$ holds.
	%----
	\item[--] $P_i \in (S_q \cap Z^{\star}) $:  In both the executions, 
	$\Adv$ receives $\OK_q(P_i, \Acast, \sid^{(q)}_{ij}, \OK_q(i,j))$ if and only if 
	$\Adv$ on the behalf of $P_i$ has sent $(P_i, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(i,j))$ to $\FAcast$
	with $\sid^{(P_{\D}, q)}_{ij}$ for $P_j$.
	%----
	\end{myitemize}
%----
   Clearly, irrespective of the case, the distribution of the $\OK_q$ messages is identical in both the executions.
%---
\item[--] The core sets $\{\C_q\}_{S_q \in \ShareSpec}$: In both the 
 executions, the sets $\C_q$ are determined, based on the $\OK_q$ messages delivered to $P_{\D}$. So the distribution of these sets is also identical. 
\end{myenumerate}
%----
\item[--] Corresponding to every $S_q \in \ShareSpec^{\star}$, the signatures $\ICSig(\sid^{P_\D,q}_{k,i,j},P_k \rightarrow P_i \rightarrow P_j,s_{qk})$ revealed by party $P_i \in \C_q \setminus Z^{\star}$ to $P_j \in (S_q \setminus \C_q) \cap Z^{\star}$, signed by every party $P_k \in \C_q \setminus \{P_i\}$ : We note that the distributon of core sets $\C_q$ for each $S_q \in \ShareSpec$ is the same in both the executions. In the real execution, $P_i$, upon receiving $\ICSig(\sid^{P_\D,q}_{k,i,j},P_k \rightarrow P_i \rightarrow P_j,s_{qk})$, checks if $s_{qk} = s_{qi}$ holds, before adding the edge $(P_i,P_k)$ in $G^i_q$. Since $P_\D$ is honest, $s_{qi} = [s]_q$. In the ideal execution as well, the simulator reveals $\ICSig(\sid^{P_\D,q}_{k,i,j},P_k \rightarrow P_i \rightarrow P_j,s_{qk})$ to $\Adv$, where $s_{qk} = [s]_q$. Hence, the distribution of messages is identical in both executions.
\end{proof}
%----

We next claim that if the dealer is {\it honest}, then conditioned on the view of the adversary $\Adv$ (which is identically distributed in both the executions, as per the previous claim),
  the outputs of the honest parties are identically distributed in both the executions.
%----
\begin{claim}
\label{claim:SVSSHonestDCorrectness}
%----
If $P_{\D}$ is honest, then conditioned on the view of $\Adv$, the output of the honest parties during the execution of $\PiStatVSS$ involving $\Adv$ has the
   same distribution as the output of the honest parties in the ideal-world involving $\SimPVSS$ and $\FVSS$, except with a probability of $n^2 \cdot \errorAICP$.
%----
\end{claim}
%-----
%----
\begin{proof}
%----
Let $P_{\D}$ be honest and let $\View$ be an arbitrary view of $\Adv$. Moreover, let $\{s_q \}_{S_q \cap Z^{\star} \neq \emptyset}$ be the shares
 of the corrupt parties, as per $\View$. Furthermore, let $\{s_q \}_{S_q \cap Z^{\star} = \emptyset}$ be the shares, used by $P_{\D}$
  in the simulated execution, corresponding to the set $S_q \in \ShareSpec$, such that $S_q \cap Z^{\star} = \emptyset$. \commentAA{In the current simulator, we haven't shown simulator choosing shares for $S_q \in \ShareSpec$ such that $S_q \cap Z^{\star} = \phi$. Should we do this?}
   Let $s \defined \displaystyle \sum_{S_q \cap Z^{\star} \neq \emptyset} s_q + \sum_{S_q \cap Z^{\star} = \emptyset} s_q$.
   Then in the simulated execution, each {\it honest} party $P_i$ obtains the output $\{[s]_q\}_{P_i \in S_q}$ from $\FVSS$, where
   $[s]_q = s_q$. We now show that except with a probability of $n^2 \cdot \errorAICP$, $P_i$ eventually obtains the
    output $\{[s]_q\}_{P_i \in S_q}$ in the real execution as well, if $P_{\D}$'s inputs in the protocol $\PiStatVSS$ are 
    $\{s_q \}_{S_q \in \ShareSpec}$.
    
    Since $P_{\D}$ is {\it honest}, it sends the share $s_q$ to {\it all} the parties in the set $S_q$, which is eventually delivered. Now consider {\it any} $S_q \in \ShareSpec$.
     During the pairwise consistency tests, each {\it honest} $P_k \in S_q$ will eventually send $\ICSig(\sid^{(P_\D,q)}_{k,j,m}, P_k \to P_j \to P_m, s_{qk})$ to 
      {\it all} the parties $P_j$ in $S_q$, for all parties $P_m \in \PartySet$, where $s_{qk} = s_q$. Consequently, every {\it honest} $P_j \in S_q$ will eventually send the message $\OK_q(j, k)$ for broadcast to
      $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$, corresponding to every {\it honest} $P_k \in S_q$. This is because, by the correctness of AICP (Lemma \ref{lemma:AICPCorrectness}), $P_j$ will receive $s_{qk}$, and $s_{qj} = s_{qk} = s_q$ will hold.
      So, every {\it honest} party (including $P_{\D}$) eventually receives the output
      $\OK_q(P_j, \Acast, \sid^{(P_{\D}, q)}_{ij}, \OK_q(j, k))$ from $\FAcast$ with $\sid^{(P_{\D}, q)}_{jk}$.
      This implies that the parties in $S_q \setminus Z^{\star}$ will eventually form a clique in the graph $G^{(i)}_q$
      of every {\it honest} $P_i$. This further implies that $P_{\D}$ will eventually find a set $\C_q$ where $S_q \setminus \C_q \in \AdvStructure$
      and where $\C_q$ constitutes a clique in the consistency graph of every honest party. 
      This is because the set $S_q \setminus Z^{\star}$ is guaranteed to eventually constitute a clique.
            Hence $P_{\D}$ eventually sends the sets $\{ \C_q\}_{S_q \in \ShareSpec}$ to $\FAcast$ with $\sid_{P_{\D}}$, which are eventually delivered to every honest
      party. Moreover, the verification of these sets will be eventually successful for every honest party.
      
      Next consider an arbitrary {\it honest} $P_i \in S_q$. If $P_i \in \C_q$, then it has already received the share $s_q$ from $P_{\D}$
      and $s_{qi} = s_q$ holds. Hence $P_i$ sets $[s]_q$ to $s_q$. So consider the case when $P_i \not \in \C_q$. In this case, 
      $P_i$ sets $[s]_q$, based on whether it is accepts a common value $s_{qk}$ from an intermediary $P_j$ in $\C_q$, such that $P_j$ is able to reveal $s_{qk}$ for all parties $P_k \in \C_q \setminus \{P_j\}$. 
      If $P_i$ accepts signatures on such a value, then it sets $[s]_q$ to the common $s_{qk}$.
      To complete the proof, we need to show that except with a probability of $n \cdot \errorAICP$, $P_i$ will eventually accept signatures on a common value which is the same as $s_q$. From the union bound, it follows that the probability with which each honest party outputs $s_q$ will be $n^2 \cdot \errorAICP$.
      
      The proof follows from the fact that since $\ShareSpec$ satisfies the $\Q^{(2)}(\ShareSpec,\AdvStructure)$ condition, and since $\C_q = S_q \setminus Z$ for some $Z \in \AdvStructure$, $\AdvStructure$ satisfies the $\Q^{(1)}(\C_q,\AdvStructure)$ condition. Hence, for every $S_q \in \ShareSpec$, $\C_q$ contains at least one honest party. Let this honest party be $P_{h}$. From the non-repudiation of AICP (Lemma \ref{lemma:AICPNonRepudiation}), for a given party $P_k \in \C_q$, except with probability $\errorAICP$, $P_{h}$ will be able to reveal $\ICSig(\sid^{(P_\D,q)}_{k,h,i},P_k \to P_h \to P_i,s_{qk})$ to $P_i$. From the protocol steps, it follows that $s_{qk} = s_q$, since $P_h$ and $P_k$ are a part of $\C_q$, which is a clique. From the union bound, it follows that $P_h$ will be able to reveal the signature on $s_q$ for {\it all} $P_k \in \C_q \setminus \{P_h\}$ to $P_i$, except with a probability of $n \cdot \errorAICP$. Furthermore, consider a corrupt $P_j \in \C_q$. From the unforgeability of AICP (Lemma \ref{lemma:AICPUnforgeability}), except with a probability of $\errorAICP$, it is not possible for a corrupt party $P_j$ to reveal $\ICSig(\sid^{(P_\D,q)}_{h,j,i},P_h \to P_j \to P_i,s_{qh})$ to $P_i$, such that $s_{qh} \neq s_q$. From the union bound, it follows that no corrupt party $P_j \in \C_q$ can reveal a signature on $s_{qh} \neq s_q$ signed by $P_h$ to $P_i$, except with a probability of $n \cdot \errorAICP$. 
      %----
   %----
\end{proof}
%----

We next prove certain claims with respect to a {\it corrupt} dealer. The first obvious claim is that the view of $\Adv$ in this
case is also identically distributed in both the real as well as simulated execution. This is simply
because in this case, the {\it honest} parties have {\it no} inputs
  and the simulator simply plays the role of the honest parties, {\it exactly}
 as per the steps of the protocol $\PiStatVSS$ in the simulated execution.

%------
\begin{claim}
\label{claim:SVSSCorruptDPrivacy}
%---
If $P_{\D}$ is corrupt, then 
the view of $\Adv$ in the simulated execution of $\PiStatVSS$ with $\SimPVSS$ is identically distributed to the view of $\Adv$ in the real execution of
$\PiStatVSS$ involving honest parties.
%---
\end{claim}
%-----
%----
\begin{proof}
%---
The proof follows from the fact that if $P_{\D}$ is {\it corrupt}, then $\SimPVSS$ participates in a full execution of the protocol
 $\PiStatVSS$, by playing the role of the honest parties as per the steps of $\PiStatVSS$.
 Hence, there is a one-to-one correspondence between simulated
  executions and real executions.
%---
\end{proof}
%----

We finally claim that if the dealer is {\it corrupt}, then conditioned on the view of the adversary (which is identical in both
the executions as per the last claim), the outputs of the honest parties are identically distributed in 
 both the executions.
 %----
\begin{claim}
\label{claim:SVSSCorruptDCorrectness}
%----
If $\D$ is corrupt, then conditioned on the view of $\Adv$, the output of the honest parties during the execution of $\PiStatVSS$ involving $\Adv$ has the  same distribution as the output of the honest parties in the ideal-world involving $\SimPVSS$ and $\FVSS$.
%----
\end{claim}
%-----
%----
\begin{proof}
%----
Let $P_{\D}$ be {\it corrupt} and let 
 $\View$ be an arbitrary view of $\Adv$. We note that it can be found out from $\View$ whether valid
   core sets $\{\C_q\}_{S_q \in \ShareSpec}$ have been generated during the corresponding execution of $\PiStatVSS$ or not. We now consider the following cases.
 %---
\begin{myitemize}
%----
\item[--] {\it No core sets $\{\C_q\}_{S_q \in \ShareSpec}$ are generated as per $\View$}: In this case, the honest parties do not obtain any output in either execution.
 This is because in the real execution of $\PiStatVSS$, the honest parties compute their output only when they get valid core sets $\{\C_q\}_{S_q \in \ShareSpec}$
 from $P_{\D}$'s broadcast. And if this is not the case, then in the simulated execution, 
  the simulator $\SimPVSS$ does not provide any input to $\FVSS$ on behalf of $P_\D$; hence, $\FVSS$ does not produce any output for the honest parties.
%----
\item[--] {\it Core sets $\{\C_q\}_{S_q \in \ShareSpec}$ generated as per $\View$ are invalid}:
 Again, in this case, the honest parties do not obtain any output in either execution.
  This is because in the real execution of $\PiStatVSS$, even if the sets 
   $\{\C_q\}_{S_q \in \ShareSpec}$ are received from $P_{\D}$'s broadcast,
    the honest parties compute their output only when each $\C_q$ set is found to be {\it valid}, with respect to the verifications
    performed by the honest parties in their own consistency graphs.
    And if these verifications fail (implying that the core sets are invalid), then in the simulated execution, 
    the simulator $\SimPVSS$ does not provide any input to $\FVSS$ on behalf of $P_\D$, implying that
     $\FVSS$ does not produce any output for the honest parties.
%----
\item[--] {\it Valid core sets $\{\C_q\}_{S_q \in \ShareSpec}$ are generated as per $\View$}:
  We first note that in this case, $P_{\D}$ has distributed some common share, say $s_q$, as determined by $\View$, 
  to all the parties in $\C_q \setminus Z^{\star}$, during the real execution of $\PiStatVSS$. 
  This is because all the parties in $\C_q \setminus Z^{\star}$ are {\it honest}, and form a clique
  in the consistency graph of the honest parties. Hence, 
  every $P_j, P_k \in \C_q \setminus Z^{\star}$ have broadcasted the messages $\OK_q(j, k)$ and $\OK_q(k, j)$
  after checking that $s_{qj} = s_{qk}$ holds, where $s_{qj}$ and $s_{qk}$ are the values 
  received from $P_{\D}$ by $P_j$ and $P_k$ respectively. This is due to the correctness of AICP (Lemma \ref{lemma:AICPCorrectness}).
  
  We next show that in the real execution of $\PiStatVSS$, except with a probability of $n^2 \cdot \errorAICP$, every party in $S_q \setminus Z^{\star}$ eventually sets
  $[s]_q = s_q$. While this is obviously true for the parties in $\C_q \setminus Z^{\star}$, we consider an arbitrary party
  $P_i \in S_q \setminus (Z^{\star} \cup \C_q)$. From the protocol steps,
      $P_i$ sets $[s]_q$ to some value, based on whether it is accepts a common value $s_{qk}$ from an intermediary $P_j$ in $\C_q$, such that $P_j$ is able to reveal $s_{qk}$ for all parties $P_k \in \C_q \setminus \{P_j\}$. 
      If $P_i$ accepts signatures on such a value, then it sets $[s]_q$ to the common $s_{qk}$.
      We next argue that except with a probability of $n \cdot \errorAICP$, $P_i$ will eventually accept signatures on a common value which is the same as $s_q$. From the union bound, it follows that the probability with which each honest party outputs $s_q$ will be $n^2 \cdot \errorAICP$. The proof for this is exactly the {\it same}, as Claim \ref{claim:SVSSHonestDCorrectness}. 
      
      Thus, in the real execution, except with a probability of $n^2 \cdot \errorAICP$, every honest party $P_i$ eventually outputs $\{[s]_q = s_q \}_{P_i \in S_q}$.
      From the steps of $\SimPVSS$, the simulator sends the shares $\{s_q \}_{S_q \in \ShareSpec}$ to $\FVSS$ on the behalf of
      $P_{\D}$ in the simulated execution. Consequently, in the ideal world, $\FVSS$ will eventually deliver
      the shares $\{[s]_q = s_q \}_{P_i \in S_q}$ to every honest $P_i$.
      Hence, except with a probability of $n^2 \cdot \errorAICP$, the outputs of the honest parties are identical in both the worlds.
     %----
\end{myitemize}
%----
\end{proof}
%----
The proof of the theorem now follows
  from Claims \ref{claim:SVSSHonestDPrivacy}-\ref{claim:SVSSCorruptDCorrectness}.
%---
\end{proof}

%----
\subsection{Properties of the Protocol $\BasicMult$}
%---
In this section, we formally prove the properties of the protocol $\BasicMult$ (see Fig \ref{fig:BasicMult} for the formal description of the protocol). 
 While proving these properties, we will assume that  $\AdvStructure$ satisfies the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition.
  This further implies that the sharing specification $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$
  satisfies the $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition. 
  Moreover, while proving these properties, we assume that no honest party is ever included in the set $\Discarded$. Note that this is ensured in the protocol $\RandMultLCE$, where $\BasicMult$ is used as a subprotocol. We first show that the intersection of any two sets in $\ShareSpec$ contains at least one honest party {\it outside} $\Discarded$.
  %----
  \begin{claim}
  \label{claim:BasicMultAdvCondition}
  %----
 For every $Z \in \AdvStructure$ and every ordered pair $(p, q) \in \{1, \ldots, h \} \times \{1, \ldots, h \}$,
  the set $(S_p \cap S_q) \setminus \Discarded$ contains at least one honest party.
  %----
  \end{claim}
  %-----
  \begin{proof}
  %----
  From the definition of the sharing specification $\ShareSpec$, we have
   $S_p = \PartySet \setminus Z_p$ and $S_q = \PartySet \setminus Z_q$, where $Z_p, Z_q \in \AdvStructure$. Let $Z^{\star} \in \AdvStructure$ be the set of corrupt parties during the protocol $\BasicMult$. Now, $S_p \cap S_q = (\PartySet \setminus Z_p) \cap (\PartySet \setminus Z_q) = \PartySet \setminus (Z_p \cup Z_q)$. This means that $(S_p \cap S_q) \cup Z_p \cup Z_q = \PartySet$. If $(S_p \cap S_q) \subseteq Z^{\star}$, then $Z^{\star} \cup Z_p \cup Z_q = \PartySet$. This is a violation of the $\Q^{(3)}(\PartySet,\AdvStructure)$ condition, and hence, $S_p \cap S_q$ contains at least one honest party. Since $\Discarded$ contains only corrupt parties, $(S_p \cap S_q) \setminus \Discarded$ contains at least one honest party.
  %---
  \end{proof}
  
We next show that during each hop, a distinct summand-sharing party $P_j$ is selected, such that all parties hold shares corresponding to the sum of summands $P_j$ is supposed to share.

%---
\begin{claim}
  \label{claim:BasicMultACS}
  %----
 For every $Z \in \AdvStructure$, if all honest parties participate during the hop number $\hop$ in the protocol $\BasicMult$, then
 all honest parties eventually obtain a common summand-sharing party, say $P_j$, for this hop, such that the honest parties
  will eventually hold $[c^{(j)}_\iter]$. Moreover, party $P_j$ will be distinct from the summand-sharing party
   selected for any hop number $\hop' < \hop$.
  %----
  \end{claim}
  %-----
  \begin{proof}
  %---
  Since all honest parties participate in hop number $\hop$, it follows that 
  $\Products_\iter \neq \emptyset$ at the beginning of hop number $\hop$. This implies that there exists at least one ordered pair $(p, q) \in \Products_\iter$.
   From Claim \ref{claim:BasicMultAdvCondition}, 
    there exists at least one {\it honest} party in $(S_p \cap S_q) \setminus Z$, say $P_k$, who will have both the shares 
  $[a]_p$ as well as $[b_q]$ (and hence the summand $[a]_p [b]_q$). We also note that $P_k$ {\it would not} have been selected as the common summand-sharing 
  party in any previous $\hop' < \hop$, as otherwise $P_k$ would have already included the summand $[a]_p[b]_q$ in the sum $c^{(k)}_\iter$ shared
  by $P_k$ during hop $\hop'$, implying that $(p, q) \not \in \Products_\iter$. Now during the hop number $\hop$, party $P_k$
  will randomly secret-share the sum $c^{(k)}_\iter$ by making a
  call to $\FVSS$  and every honest $P_i$ will eventually receive an output
   $(\Share, \sid_{\hop, k}, P_k, \{ [c^{(k)}_\iter]_q \}_{P_i \in S_q})$  from $\FVSS$
    with $\sid_{\hop, k, \iter, Z}$. 
 Moreover, $P_k$ {\it will not} be present in the set $\Discarded$.
  
  We next claim that during the hop number $\hop$, there will be at least one instance of $\FABA$, corresponding to which {\it all} honest parties
  eventually receive the output $1$. For this, we consider two possible cases:
  %----
  \begin{myitemize}
  %---
  \item[--] {\it At least one honest party participates with input $0$ in the $\FABA$ instance corresponding to $P_k$}: Let 
  $P_i$ be an {\it honest} party, who sends $(\vote, \sid_{\hop, k}, 0)$ to $\FABA$ with 
  $\sid_{\hop, k}$. Then from the steps of $\BasicMult$, it follows that there exists some $P_j \in \PartySet$, such that
  $P_i$ has received
    $(\decide, \sid_{\hop, j}, 1)$ as the output from $\FABA$ with  $\sid_{\hop, j}$. Hence, {\it every} honest party
    will eventually receive the output $(\decide, \sid_{\hop, j}, 1)$ as the output from $\FABA$ with  $\sid_{\hop, j}$.
  %----
  \item[--] {\it No honest party participates with input $0$ in the $\FABA$ instance corresponding to $P_k$}:
  In this case, {\it every} honest party will eventually send $(\vote, \sid_{\hop, k}, 1)$ to $\FABA$ with 
  $\sid_{\hop, k}$ and eventually receives the output $(\decide, \sid_{\hop, k}, 1)$ from $\FABA$. 
  %---
  \end{myitemize}
  %----
  Now based on the above claim, we can further claim that 
   all honest parties will eventually participate with some input in all the
  $n$ instances of $\FABA$ invoked during the hop number $\hop$
  and hence all the $n$ instances of $\FABA$ during the hop number $\hop$ will eventually produce an output.
  Since the summand-sharing party for hop number $\hop$   
  corresponds to the least indexed $\FABA$ instance in which all the honest parties obtain $1$ as the output,
   it thus follows that eventually the honest parties will select a summand-sharing party. Moreover, this summand-sharing party will be common,
  as it is based on the outcome of $\FABA$ instances.
  
  Let $P_j$ be the summand-sharing party for the hop number $\hop$.
   We next show that the honest parties will eventually hold $[c^{(j)}_\iter]$.
   For this, we note that since $P_j$ has been selected as the summand-sharing party, {\it at least} one {\it honest} party, say
   $P_i$, must have sent $(\vote, \sid_{\hop, j}, 1)$ to $\FABA$ with 
  $\sid_{\hop, j}$. If not, then $\FABA$ with $\sid_{\hop, j}$ will never produce the output
  $(\decide, \sid_{\hop, j}, 1)$ and hence $P_j$ will not be the summand-sharing party for the hop number $\hop$.
  Now since $P_i$ sent $(\vote, \sid_{\hop, j}, 1)$ to $\FABA$, it follows that
  $P_i$ has received an output $(\Share, \sid_{\hop, j}, P_j, \{ [c^{(j)}_\iter]_q \}_{P_i \in S_q})$  from $\FVSS$
    with $\sid_{\hop, j}$. This implies that $P_j$ must have sent the message 
    $(\Dealer, \sid_{\hop, j}, (c^{(j)}_{\iter,1}, \ldots, c^{(j)}_{\iter,h}))$ to
    $\FVSS$ with $\sid_{\hop, j}$. 
    Consequently, every honest party will eventually receive their respective outputs from 
     $\FVSS$ with $\sid_{\hop, j}$ and hence the honest parties will eventually hold
     $[c^{(j)}_\iter]$.
     
     Finally, to complete the proof of the claim, we need to show that party $P_j$ is different from the summand-sharing parties selected
     during the hops $1, \ldots, \hop - 1$. If $P_j$ has been selected as a summand-sharing party for any hop number $\hop' < \hop$, then
     no honest party ever sends $(\vote, \sid_{\hop, j}, 1)$ to $\FABA$ with 
  $\sid_{\hop, j}$. Consequently, $\FABA$ with $\sid_{\hop, j}$ will never send the output 
  $(\decide, \sid_{\hop, j}, 1)$ to any honest party and hence $P_j$ will not be selected as the summand-sharing party
  for hop number $\hop$, which is a contradiction.
  %--
  \end{proof}
  
We next prove a claim regarding the communication complexity of protocol $\BasicMult$. 
%----
\begin{claim}
  \label{claim:BasicMultComplexity}
  %----
  In protocol $\BasicMult$, all honest parties eventually obtain an output.
   The protocol makes $\Order(n^2)$ calls to $\FVSS$ and $\FABA$.
  %----
  \end{claim}
  %-----
  \begin{proof}
  %---
  From Claim \ref{claim:BasicMultAdvCondition} and \ref{claim:BasicMultACS}, it follows that the number of hops in the protocol 
   is $\Order(n)$, as in each hop a new summand-sharing party is selected and if all honest parties are included
   in the set of summand-sharing parties $\Selected_\iter$, then $\Products_\iter$ becomes $\emptyset$.
   The proof now follows from the fact that in each hop, there are $\Order(n)$ calls to $\FVSS$ and $\FABA$. 
  %---
  \end{proof}

We next make a claim regarding the privacy of $\BasicMult$  
  
%----
\begin{claim}
  \label{claim:BasicMultPrivacy}
  %----
  During protocol $\BasicMult$, $\Adv$ learns nothing about $a$ and $b$.
  %----
  \end{claim}
  %-----
  \begin{proof}
  %---
  Since the proof is similar to that of Claim $\ref{claim:OptMultPrivacy}$, we skip the formal proof.
  %---
  \end{proof}

We next show that if no party in $\PartySet \setminus \Discarded$ behaves maliciously, then all honest parties hold shares of a value $c_\iter$, such that $c_\iter$ is $ab$.  

  %---
  \begin{claim}
  \label{claim:BasicMultCorrectness}
  %---
  In protocol $\BasicMult$, if no party in $\PartySet \setminus \Discarded$ behaves maliciously, then for each $P_i \in \Selected_\iter$, the condition
   $c^{(i)}= \sum_{(p, q) \in \Products^{(i)}_\iter} [a]_p[b]_q$ holds and
   $c_\iter = ab$. 
  %--
  \end{claim}
%----
  \begin{proof}
  %---
  From the protocol steps, it follows that $\Selected_\iter \cap \Discarded = \emptyset$, as no honest party ever votes for any party from $\Discarded$ as a candidate
  summand-sharing party during any hop in the protocol.  
  Now since $\Selected_\iter \subseteq (\PartySet \setminus \Discarded)$, 
  if no party in $\PartySet \setminus \Discarded$ behaves maliciously, then it implies that every party 
  $P_i \in \Selected_\iter$ has behaved honestly and secret-shares $c^{(i)}_\iter$ by calling $\FVSS$, where
  $c^{(i)} = \sum_{(p, q) \in \Products^{(i)}_\iter} [a]_p[b]_q$.
  Moreover, from the protocol steps, it follows that for every $P_j, P_k \in \Selected_\iter$:
  %---
  \[ \displaystyle \Products^{(j)}_\iter \cap \Products^{(k)}_\iter = \emptyset.  \]
  %---
  To prove this, suppose $P_j$ and $P_k$ are included in $\Selected_\iter$ during hop number $\hop_j$ and $\hop_k$ respectively, where
  without loss of generality, $\hop_j < \hop_k$. 
  Then from the protocol steps, during $\hop_j$, the parties would set
  $\Products^{(k)}_\iter = \Products^{(k)}_\iter \setminus \Products^{(j)}_\iter$. This ensures that
  during $\hop_k$, there exists no ordered pair $(p, q) \in \{1, \ldots, |\ShareSpec| \} \times \{1, \ldots, |\ShareSpec| \}$, such that
  $(p, q) \in \Products^{(j)}_\iter \cap \Products^{(k)}_\iter$.
  
  Since all the parties $P_i \in \Selected_\iter$ have behaved honestly, 
   from the protocol steps, it also follows that :
  %---
  \[ \displaystyle \bigcup_{P_i \in \Selected_\iter} \Products^{(i)}_\iter = \{ (p, q) \}_{p, q = 1, \ldots, |\ShareSpec|}. \]
  %---
  Finally, from the protocol steps, it follows that 
   $\forall P_j \in \PartySet \setminus \Discarded$, the condition
  $c^{(j)} _\iter= 0$ holds. Now since $c_\iter =  c^{(1)}_\iter + \ldots + c^{(n)}_\iter$, it follows that
  if no party in $\PartySet \setminus \Discarded$ behaves maliciously, then $c_\iter = ab$. 
  %---
  \end{proof}
 
%-----
\noindent {\bf Lemma \ref{lemma:BasicMult}.}
%----
{\it Let  $\AdvStructure$ satisfy the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition. Then
 the parties eventually compute  $[c_\iter]$ and $([c^{(1)}_\iter], \ldots, [c^{(n)}_\iter])$ in $\BasicMult$ 
 where $c_\iter = c^{(1)}_\iter + \ldots + c^{(n)}_\iter$, provided no honest party is ever included in $\Discarded$.
 If no party in $\PartySet \setminus \Discarded$ behaves maliciously, then for all $P_i \in \Selected_\iter$, the condition
   $c^{(i)}_\iter = \sum_{(p, q) \in \Products^{(i)}} [a]_p[b]_q$ holds and
   $c_\iter = ab$. Furthermore, $\Adv$ does not learn any additional information about $a$ and $b$. The protocol makes $\Order(n^2)$ calls to $\FVSS$ and $\FABA$.}
%----
\begin{proof}
%----
The proof follows from Claims \ref{claim:BasicMultAdvCondition}-\ref{claim:BasicMultCorrectness}.
%---
\end{proof}
%----

%----
\subsection{Properties of the Protocol $\RandMultLCE$}
%---
In this section, we formally prove the properties of the protocol $\RandMultLCE$ (see Fig \ref{fig:StatMultCI} for the formal description of the protocol). 
 While proving these properties, we will assume that  $\AdvStructure$ satisfies the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition.
  This further implies that the sharing specification $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$
  satisfies the $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition. We first claim that the parties eventually obtain shares corresponding to random values $a_\iter,b_\iter, b'_\iter$ and $c_\iter$.
  
\begin{claim}
\label{claim:RandMultLCERandomACS}
%------
Consider an instance $\RandMultLCE$ invoked during iteration $\iter$. Every honest party $P_i$ eventually obtains the shares $\{[a_\iter]_q\}_{P_i \in S_q}$, $\{[b_\iter]_q\}_{P_i \in S_q}$, $\{[b'_\iter]_q\}_{P_i \in S_q}$ and $\{[r_\iter]_q\}_{P_i \in S_q}$ corresponding to the values $a_\iter,b_\iter,b'_\iter$ and $r_\iter$ respectively. Furthermore, $a_\iter,b_\iter,b'_\iter$ and $r_\iter$ are uniformly random values uknown to $\Adv$ before their shares are reconstructed.
%------
\end{claim}
%------
\begin{proof}
%------
We show that all honest parties $P_i$ obtain $\{[a_\iter]_q\}_{P_i \in S_q}$ such that $a_\iter$ is a uniformly random value unknown to the adversary, before its shares are reconstructed. A similar argument can be used to show that this holds for $\{[b_\iter]_q\}_{P_i \in S_q}$, $\{[b'_\iter]_q\}_{P_i \in S_q}$ and $\{[r_\iter]_q\}_{P_i \in S_q}$ corresponding to $b_\iter,b'_\iter$ and $r_\iter$ as well.

Let $\Hon$ be the set of honest parties in $\PartySet$. Each honest party $P_j$ will pick a uniformly random value $a^{(j)}_\iter$, and choose $a^{(j)}_{\iter,1}, \ldots, a^{(j)}_{\iter,h}$ such that $a^{(j)}_{\iter,1} + \ldots + a^{(j)}_{\iter,h} = a^{(j)}_\iter$. $P_j$ will then send $(\Dealer,\sid_{j,1},(a^{(j)}_{\iter,1}, \ldots, a^{(j)}_{\iter,h}))$ to $\FVSS$. Hence, each honest party $P_k$ will obtain $(\Share,\sid_{j,1},P_j,\{a^{(j)}_{\iter}\})$ from $\FVSS$, upon request with session id $\sid_{j,1}$, and send $(\vote,\sid_j,1)$ to $\FABA$. Thus, $P_i$ will eventually obtain $(\decide,\sid_j,1)$ for $\FABA$ corresponding to each honest party $P_j$. Since $\PartySet \setminus \Hon = Z^{\star}$, a subset of parties $\GlobalProv_{(\iter,i)}$ will eventually be found. Thus, all honest parties will eventually participate in $\FABA$ corresponding to every party $P_j \in \PartySet$, and $\CoreSet_{\iter}$ will eventually be found. 

Now, we will show that $\GlobalProv_{(\iter,i)}$ contains at least one honest party. This would mean that $\CoreSet_\iter$ also contains at least one honest party, since $\GlobalProv_{(\iter,i)} \subseteq \CoreSet_\iter$. Since $\AdvStructure$ satisfies the $\Q^{(3)}(\PartySet,\AdvStructure)$ condition, and since $\PartySet \setminus \GlobalProv_{(\iter,i)} \in \AdvStructure$, $\PartySet$ satisfies the $\Q^{(2)}(\GlobalProv_{(\iter,i)},\AdvStructure)$ condition. This means that $\GlobalProv_{(\iter,i)}$, and subsequently $\CoreSet_\iter$, contain at least one honest party. Let this honest party be $P_h$. Since $a_\iter \defined \displaystyle \sum_{P_j \in \CoreSet} a^{(j)}_\iter$, $a_\iter \defined a^{(h)}_\iter + \displaystyle \sum_{P_j \in \CoreSet \setminus \{P_h\}} a^{(j)}_\iter$. Since $a^{(h)}_\iter$ is chosen uniformly at random from $\F$, $a_\iter$ is also a uniformly random value.

%------
\end{proof}
%------

We next claim that each honest party will reconstruct the same value of $d_\iter$, and agree on whether the protocol has succeeded or failed.

\begin{claim}
\label{claim:RandMultLCETermination}
%------
Consider an instance of $\RandMultLCE$ invoked during iteration $\iter$. Eventually, each honest party $P_i$ reconstructs a (common) value $d_\iter$.
%------
\end{claim}
%------
\begin{proof}
%------
From Claim \ref{claim:RandMultLCERandomACS}, $P_i$ eventually obtains the shares $\{[a_\iter]_q\}_{P_i \in S_q}$, $\{[b_\iter]_q\}_{P_i \in S_q}$, $\{[b'_\iter]_q\}_{P_i \in S_q}$ and $\{[r_\iter]_q\}_{P_i \in S_q}$ corresponding to the values $a_\iter,b_\iter,b'_\iter$ and $r_\iter$ respectively. From Lemma \ref{lemma:BasicMult}, each honest party $P_i$ eventually obtains outputs $\{[c^{(1)}_\iter]_q , \ldots, [c^{(n)}_\iter]_q, [c_\iter]_q \}_{P_i \in S_q}$ and $\{[c'^{(1)}_\iter]_q , \ldots, [c'^{(n)}_\iter]_q, [c'_\iter]_q \}_{P_i \in S_q}$ from the corresponding instances of $\BasicMult$. From Lemma \ref{lemma:PerRec}, each party $P_i$ will participate in $\PiPerRec$ with $\{[r_\iter]_q\}_{P_i \in S_q}$ and be able to reconstruct $r_\iter$. By a similar argument, they will also be able to reconstruct $e_\iter$, followed by $d_\iter$. 
%------
\end{proof}
%------

We next claim that if no party in $\PartySet \setminus \Discarded$ behaves maliciously, then the parties eventually obtain shares corresponding to a random multiplication triple.

\begin{claim}
\label{claim:RandMultLCENoMaliciousBehaviour}
%------
Consider an instance of $\RandMultLCE$ invoked during iteration $\iter$. If no party in $\PartySet \setminus \Discarded$ behaves maliciously, then each honest party $P_i$ sets $\flag^{(i)}_\iter=0$ and outputs shares $\{([a_\iter]_q,[b_\iter]_q,[c_\iter]_q)\}_{P_i \in S_q}$, such that $c_\iter = a_\iter b_\iter$ holds.
%------
\end{claim}
%------
\begin{proof}
%------
 From Lemma \ref{lemma:BasicMult}, if no party behaves maliciously, then for all parties $P_j \in \Selected_\iter$, it holds that $c^{(j)}_\iter = \sum_{(p,q) \in \Products^{(j)}_{(\iter,c)}}$, and that $c'^{(j)}_\iter = \sum_{(p,q) \in \Products^{(j)}_{(\iter,c')}}a_pb'_q$. For every $P_j \in \Selected_\iter$, it then holds that $r_\iter c^{(j)}_\iter + c'^{(j)}_\iter \neq r_\iter \sum_{(p,q) \in \Products^{(j)}_{(\iter,c)}} a_pb_q + \sum_{(p,q) \in \Products^{(j)}_{(\iter,c')}}a_pb'_q$. Then, we can infer the following.

$$\displaystyle \sum_{P_j \in \Selected_\iter} r^{(j)_\iter}_\iter c^{(j)}_\iter + c'^{(j)}_\iter = \sum_{P_j \in \Selected_\iter} r^{(j)} \sum_{(p,q) \in \Products^{(j)}_{(\iter,c)}} a_pb_q + \sum_{(p,q) \in \Products^{(j)}_{(\iter,c')}}a_pb'_q$$

By summing over the parties $P_j \in \Selected$, the following holds, based on how $r^{(\iter)}, a^{(\iter)}, b^{(\iter)}$ and $b'^{(\iter)}$ are defined.

$$r_\iter c_\iter + c'_\iter = r_\iter a_\iter b_\iter + a_\iter b'_\iter$$

But since $e_\iter = r_\iter b_\iter + b'_\iter$, 

$$r_\iter c_\iter + c'_\iter = e_\iter a_\iter \implies e_\iter a_\iter - c_\iter - c'_\iter = 0 \implies d_\iter = 0$$

Hence, the reconstructed value of $d_\iter$ is $0$, and each party $P_i$ outputs $\{([a_\iter]_q,[b_\iter]_q,[c_\iter]_q)\}_{P_i \in S_q}$ along with $\Success$. From Lemma \ref{lemma:BasicMult}, it holds that $c_\iter = a_\iter b_\iter$.
%------
\end{proof}
%------

We next show that if the protocol $\RandMultLCE$ succeeds, then with high probability, each honest party obtains shares corresponding to a random multiplication triple as output.

\begin{claim}
\label{claim:RandMultLCECorrectness}
%------
Consider an instance of $\RandMultLCE$ invoked during iteration $\iter$. If during the protocol, party $P_i$ sets $\flag^{(i)}_\iter=0$ and outputs $\{([a_\iter]_q,[b_\iter]_q,[c_\iter]_q)\}_{P_i \in S_q}$, then the values $a_\iter$ and $b_\iter$ are uniformly random values unknown to $\Adv$, such that except with a probability of $\frac{1}{|\F|}$, $c_\iter = a_\iter \cdot b_\iter$ holds. 
%------
\end{claim}
%------
\begin{proof}
%------
From Claim \ref{claim:RandMultLCETermination}, the parties will be able to reconstruct a value $d_\iter$. Suppose that $P_i$ has set $\flag^{(i)}_\iter=0$ and obtained output $\{([a_\iter]_q,[b_\iter]_q,[c_\iter]_q)\}_{P_i \in S_q}$. This means that the reconstructed value of $d_\iter$ is $0$. We first show that except with a probability of $\frac{1}{|\F|}$, $c_\iter = a_\iter \cdot b_\iter$ holds. Assume that it does not. Then, since $d_\iter = 0$, $r_\iter = (c'_\iter - a_\iter b'_\iter) \cdot (a_\iter b_\iter - c_\iter)^{-1}$ must hold. But from Claim \ref{claim:RandMultLCERandomACS}, $r_\iter$ is a uniformly random value in $\F$, and this is possible only with probability at most $\frac{1}{|\F|}$. Hence, except with a probability of $\frac{1}{|\F|}$, $c_\iter = a_\iter \cdot b_\iter$ holds.

We next show that the values $a_\iter$ and $b_\iter$ remain uniformly random values unknown to $\Adv$. From Claim \ref{claim:RandMultLCERandomACS}, the value of $a_\iter$ and $b_\iter$ is uniformly random to $\Adv$. From Lemma \ref{lemma:BasicMult}, $\Adv$ learns nothing about $a_\iter$, $b_\iter$ and $b'_\iter$ during the two instances of $\BasicMult$. While $\Adv$ learns the value of $e_\iter$, since $b'_\iter$ is a uniformly random value in $\F$, for every possible value of $b'_\iter$, there is a unique value of $b_\iter = (e_\iter - b'_\iter) \cdot r^{-1}_\iter$. Hence, $b_\iter$ also remains unknown to $\Adv$. Since $d_\iter$ is $0$ when all parties follow the protocol correctly, the value of $d_\iter$ also does not reveal anything about $a_\iter$ and $b_\iter$ to $\Adv$. 
%------
\end{proof}
%------

We next claim that if the protocol $\RandMultLCE$ fails, then each honest party discards at least one corrupt party which was not discarded in an earlier iteration.

\begin{claim}
\label{claim:RandMultLCECheaterIdentification}
%------
Consider an instance of $\RandMultLCE$ invoked during iteration $\iter$. Consider an honest party $P_i$. If $P_i$ sets $\flag^{(i)}_\iter=1$, then at least one corrupt party $P_j$ is added by every honest party $P_i$ to $\Discarded$. Furhtermore, $P_j$ will be different from any party added to $\Discarded$ during any previous iteration $\iter' < \iter$.
%------
\end{claim}
%------
\begin{proof}
%------
From Claim \ref{claim:RandMultLCETermination}, the parties will be able to reconstruct a value $d_\iter$. From Lemma \ref{lemma:PerRec}, the parties will be able to reconstruct  $a_\iter,b_\iter,b'_\iter,c^{(1)}_\iter,\ldots,c^{(n)}_\iter,c'^{(1)}_\iter,\ldots,c'^{(n)}_\iter$. We claim that for at least one player $P_j \in \Selected_\iter$, it must hold that $r_\iter c^{(j)}_\iter + c'^{(j)}_\iter \neq r\sum_{(p,q) \in \Products^{(j)}_{(\iter,c)}} a_pb_q + \sum_{(p,q) \in \Products^{(j)}_{(\iter,c')}}a_pb'_q$. Otherwise, from Claim \ref{claim:RandMultLCENoMaliciousBehaviour}, the reconstructed value of $d_\iter$ is $0$. Now, since $P_j \in \Selected_\iter$, from the protocol steps of $\BasicMult$, $P_j \notin \Discarded$. This is because if $P_j$ was added to $\Discarded$ in a previous iteration, then no honest party will send $(\vote,\sid_{\hop,j},1)$ to $\FABA$ in $\BasicMult$ during iteration $\iter$, and hence, no honest party will obtain $(\decide,\sid_{\hop,j},1)$ from $\FABA$. Hence, at least one corrupt party $P_j$ different from any party added to $\Discarded$ in previous iterations will be added by {\it all} honest parties $P_i$ to $\Discarded$ during iteration $\iter$.
%------
\end{proof}
%------

We next prove a claim regarding the communication complexity of protocol $\RandMultLCE$.

\begin{claim}
\label{claim:RandMultLCECommunication}
%------
In protocol $\RandMultLCE$, all honest parties eventually obtain an output. The protocol makes $\Order(n^2)$ calls to $\FVSS$ and $\FABA$, and incurs a communication of $\Order(|\AdvStruct| \cdot n^3 \log{|\F|})$ bits.
%------
\end{claim}
%------
\begin{proof}
%------
From Claim \ref{claim:RandMultLCETermination}, all honest parties eventually obtain an output. Since each party calls $\FVSS$ four times, the protocol makes $\Order(n)$ calls to $\FVSS$. Since the protocol uses one instance of $\FABA$ corresponding to each party, $\Order(n)$ calls to $\FABA$ are made. $2$ calls to $\BasicMult$ are made to obtain a sharing of $c_\iter$ and $c'_\iter$. Since $\BasicMult$ makes $\Order(n^2)$ calls to $\FVSS$ and $\FABA$, $\RandMultLCE$ also makes $\Order(n^2)$ calls to $\FVSS$ and $\FABA$. For cheater identification, $\Order(n)$ values must be reconstructed. This requires a communication of $\Order(|\AdvStruct| \cdot n^3 \log{|\F|})$ bits.
%------
\end{proof}
%------

%-----
\noindent {\bf Lemma \ref{lemma:RandMultLCE}.}
%----
{\it Let  $\AdvStructure$ satisfy the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition. Then
 all honest parties $P_i$ eventually either obtain shares $\{([a_\iter]_q,[b_\iter]_q,[c_\iter]_q)\}_{P_i \in S_q}$ such that with a probability of $1-\frac{1}{|\F|}$, $c_\iter = a_\iter b_\iter$, or add a corrupt party $P_j$ to $\Discarded$ which was not added to $\Discarded$ in any previous iteration. In the former case, the view of $\Adv$ is independent of $a_\iter$ and $b_\iter$. The protocol makes $\Order(n^2)$ calls to $\FVSS$ and $\FABA$, and incurs a communication of $\Order(|\AdvStruct| \cdot n^3 \log{|\F|})$ bits.}
%----
\begin{proof}
%----
The proof follows from Claims \ref{claim:RandMultLCERandomACS}-\ref{claim:RandMultLCECommunication}.
%---
\end{proof}
%----

%---
\subsection{Properties of the Protocol $\PiStatTriples$}%----

 In this section, we prove the security of the protocol $\PiStatTriples$ (see Fig \ref{fig:StatTriples} for the formal details of the protocol) in the $(\FVSS, \FABA)$-hybrid model.
  While proving these properties, we will assume that  $\AdvStructure$ satisfies the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition.
  This further implies that the sharing specification $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$
  satisfies the $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition. 
  \\~\\
 %----
   \noindent {\bf Theorem \ref{thm:PiStatTriples}.}
  %---
  {\it If $\AdvStructure$ satisfies the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition,
  then  $\PiStatTriples$ is a statistically-secure protocol for securely realizing $\FTriples$ with UC-security in the $(\FVSS, \FABA)$-hybrid model. 
   The protocol makes $\Order(M \cdot n^3)$ calls to $\FVSS$ and $\FABA$,
   and additionally incurs a communication of $\Order(M \cdot |\AdvStruct| \cdot n^4 \log{|\F|})$ bits. 
  %--
  }
  \begin{proof}
  %---
  The communication complexity and the number of calls to $\FVSS$ and $\FABA$ simply follows from the fact that since $\RandMultLCE$ may be called up to $\Order(n)$ times, and from the communication complexity of $\RandMultLCE$. This is because from Lemma \ref{lemma:RandMultLCE}, if an iteration fails, then a distinct corrupt party is discarded. We next prove the security. For the ease of explanation, we consider the case where
  only one multiplication-triple is generated in $\PiStatTriples$; i.e.~
   $M = 1$. The proof can be easily modified for any general $M$.
   
   Let $\Adv$ be an arbitrary adversary, attacking the protocol $\PiPerTriples$ by corrupting a set of parties
  $Z^{\star} \in \AdvStructure$ and let $\Env$ be an arbitrary environment. We show the existence of a simulator $\SimStatTriples$ (Fig \ref{fig:SimStatTriples}),
   such that for any
 $Z^{\star} \in \AdvStructure$,
  the outputs of the honest parties and the view of the adversary in the 
   protocol $\PiStatTriples$ is indistinguishable from the outputs of the honest parties and the view of the adversary in an execution in the ideal world involving 
  $\SimStatTriples$ and $\FTriples$. 
  
  The high level idea of the simulator is that the simulator simulates the actions of honest parties during an instance $\widetilde{\Pi}_{\mathsf{RandMultCI}}$ for each iteration by simulating the actions of the honest parties during the underlying $\FVSS$ and $\FABA$ instances. Upon obtaining a positive output from $\widetilde{\Pi}_{\mathsf{RandMultCI}}$ during a certain iteration $\iter'$, the simulator records this output and sends the shares of the output triple corresponding to the corrupt parties to $\FTriples$, on the behalf of $\Adv$. $\SimStatTriples$ is presented in Figure \ref{fig:SimStatTriples}.

%----
\begin{simulatorsplitbox}{$\SimStatTriples$}{Simulator for the protocol $\PiStatTriples$
  where $\Adv$ corrupts the parties in set $Z^{\star} \in \AdvStructure$}{fig:SimStatTriples}
	\justify
%----
$\SimStatTriples$ constructs virtual real-world honest parties and invokes the real-world adversary $\Adv$. The simulator simulates the view of
 $\Adv$, namely its communication with $\Env$, the messages sent by the honest parties and the interaction with $\FVSS$ and $\FABA$. 
  In order to simulate $\Env$, the simulator $\SimStatTriples$ forwards every message it receives from 
   $\Env$ to $\Adv$ and vice-versa.  The simulator then simulates the various stages of the protocol as follows. 
%---
\begin{myitemize}
%----
\item[--] \textbf{Initialization : } On behalf of the honest parties, the simulator initializes $\Discarded$ to $\emptyset$ and $\iter$ to $1$.
%----
\item[--] \textbf{Generating Random Multiplication Triple with Cheater Identification : } The simulator plays the role of the honest parties as per the protocol and interacts with $\Adv$ for an instance $\widetilde{\Pi}_{\mathsf{RandMultCI}}(\PartySet,\AdvStruct,\ShareSpec,\iter)$. During this instance, the simulator simulates the interface for $\FABA$ and $\FVSS$ for $\Adv$ during the underlying instances of $\widetilde{\Pi}_{\mathsf{BasicMult}}$, by itself performing the role of $\FABA$ and $\FVSS$. Based on the appropriate condition, simulator does the following.
	\begin{myitemize}
	%----
	\item {\bf Simulator has set $\flag^{(i)}_\iter=0$ corresponding to some honest $P_i$: } Then set $\{[\widetilde{a}]_q,[\widetilde{b}]_q,[\widetilde{c}]_q\}_{P_j \in S_q}$ to be the output $\{[\widetilde{a}_\iter]_q,[\widetilde{b}_\iter]_q,[\widetilde{c}_\iter]_q\}_{P_j \in S_q}$, obtained on the behalf of each $P_j \in Z^{\star}$.
	%----
	\item {\bf Simulator has set $\flag^{(i)}_\iter=1$ corresponding to some honest $P_i$:} Set $\iter = \iter+1$ and go to step {\bf Generating Random Multiplication Triple with Cheater Identification}.
	%----
	\end{myitemize}
	%----
%----
\item[--] {\bf Interaction with $\FTriples$ : } Let $\{[\widetilde{a}]_q,[\widetilde{b}]_q,[\widetilde{c}]_q\}_{S_q \cap Z^{\star} \neq \emptyset}$ be the output shares correposnding to parties in $Z^{\star}$. The simulator sends $\{\shares,\sid,\{[\widetilde{a}]_q,[\widetilde{b}]_q,[\widetilde{c}]_q\}$ to $\FTriples$,  on the behalf of $\Adv$.
%----
\end{myitemize}    
%---
\end{simulatorsplitbox}

We now prove a series of claims which will help us finally prove the theorem. We first show that the view generated by $\SimStatTriples$ for $\Adv$ is identically distributed to $\Adv$'s view during the real execution of $\PiStatTriples$.

%----
\begin{claim}
\label{claim:StatTriplesPrivacy}
%---
The view of $\Adv$ in the simulated execution with $\SimPerTriples$ is identically distributed as the view of $\Adv$ in the real execution of
 $\PiPerTriples$.
%---
\end{claim}
%---------
\begin{proof}
%----
In both the real world and ideal world executions, the parties run an instance of $\RandMultLCE$ for each iteration $\iter$ to obtain an output. During each of these instances, from Lemma \ref{lemma:RandMultLCE}, in case the simulator has set $\flag^{(i)}_\iter=0$ corresponding to some honest $P_i$, the view of $\Adv$ is identical in both the executions. Else, in both executions, the parties discard at least one corrupt party and proceed to the next iteration. Hence, the view of $\Adv$ in both executions is identically distributed.
%----
\end{proof}

We now show that conditioned on the view of $\Adv$, the output of honest parties is identically distributed in the real execution of $\PiStatTriples$ involving $\Adv$, as well as in the ideal execution involving $\SimStatTriples$ and $\FTriples$.

%----
\begin{claim}
\label{claim:PerTriplesOutputDistribution}
%---
Conditioned on the view of $\Adv$, the output of the honest parties is identically distributed in the real execution of $\PiPerTriples$ involving $\Adv$ and in the ideal execution involving $\SimPerTriples$ and $\FTriples$, except with a probability of $\frac{n}{|\F|}$.
%---
\end{claim}
%---------
\begin{proof}
%----
In the real execution of $\PiPerTriples$, from Lemma \ref{lemma:RandMultLCE}, during each iteration $\iter$, each honest party $P_i$ either obtains shares of a random multiplication triple $\{([a_\iter]_q,[b_\iter]_q,[c_\iter]_q)\}_{P_i \in S_q}$ with a probability of $\frac{1}{|\F|}$, or identifies and discards a corrupt party. From Lemma \ref{lemma:RandMultLCE}, a {\it distinct} party is discarded during each iteration. Since the number of corrupt parties is lesser than $n$, the number of iterations cannot exceed $n$. Furthermore, once all parties in $Z^{\star}$ are discarded, from Claim \ref{claim:RandMultLCENoMaliciousBehaviour}, the instance of $\RandMultLCE$ will succeed during some iteration $\iter'$. From Lemma \ref{lemma:RandMultLCE}, the outputs shares $\{([a_{\iter'}]_q,[b_{\iter'}]_q,[c_{\iter'}]_q)\}_{P_i \in S_q}$ correspond to a random multiplication triple such that $c_{\iter'} = a_{\iter'} b_{\iter'}$, and that the view of $\Adv$ is independent of $a_{\iter'}$ and $b_{\iter'}$. Hence, from the union bound, it follows that except with a probability of $\frac{n}{|\F|}$, the honest parties eventually output a random multiplication triple. 

To complete the proof, we now show that conditioned on the shares $\{([a_{\iter'}]_q, [b_{\iter'}]_q, [c_{\iter'}]_q) \}_{S_q \cap Z^{\star} \neq \emptyset}$ (which are determined by
    $\View$), the honest
    parties output secret-sharing
     of some random multiplication-triple in the ideal-world, which are consistent with
   the shares  $\{([a_{\iter'}]_q, [b_{\iter'}]_q, [c_{\iter'}]_q) \}_{S_q \cap Z^{\star} \neq \emptyset}$.
    However, this simply follows from the fact that in the ideal-world, the simulator
    $\SimPerTriples$ sends the shares $\{([a_{\iter'}]_q, [b_{\iter'}]_q, [c_{\iter'}]_q) \}_{S_q \cap Z^{\star} \neq \emptyset}$
     to $\FTriples$ on the behalf of the parties in $Z^{\star}$.
    And as an output, $\FTriples$ generates a random secret-sharing of some random multiplication-triple, consistent with the shares
    provided by $\SimPerTriples$. 
%----
\end{proof}

\end{proof}









==> perfectModified.tex <==
\section{Perfectly-secure AMPC Protocol}
%----
In this section, we present our perfectly-secure AMPC protocol. Throughout this section, we assume that the adversary-structure $\AdvStructure$ satisfies the
  $\Q^{(4)}(\PartySet, \AdvStructure)$ condition, which is a necessary condition for perfectly-secure AMPC.
   We first start with the definition of secret-sharing used in our perfectly-secure protocol. The secret-sharing is 
  based on the one from \cite{Mau02} and is
  defined with respect to
  a {\it sharing specification} $\ShareSpec = (S_1, \ldots, S_h)$, which is a tuple of subsets of $\PartySet$. 
  %---
  \begin{definition}[\cite{Mau02,HT13}]
  %-
  A value $s \in \F$ is said to be secret-shared with respect to a sharing specification $\ShareSpec = (S_1, \ldots, S_h)$, if the following holds:
  %---
   \begin{myitemize}
    %----
     \item[--] There exist shares $s_1, \ldots, s_h$, such that $s = s_1 + \ldots + s_h$. 
     %---
     \item[--] For $q = 1, \ldots, h$, the share $s_q$ is know to every (honest) party in $S_q$.  
     %-----
   \end{myitemize}
  %--
  \end{definition}
  %---
  A sharing of a value $s$ is denoted by $[s]$, where the notation $[s]_q$ is used to denote the $q^{th}$ share. Note that
  $P_i$ will hold the shares $\{[s]_q\}_{P_i \in S_q}$.
  It is easy to see that the above secret-sharing is {\it linear}, as given $[s_1]$ and $[s_2]$, then
  $[c_1s_1 + c_2 s_2] = c_1[s_1] + c_2[s_2]$ for any publicly-known $c_1, c_2 \in \F$.
  In general, the parties can locally
   compute a sharing of any linear combination of shared values (with respect to a sharing specification $\ShareSpec$)
    by locally computing the linear combination of their shares.
  
  
  
  A sharing specification $\ShareSpec = (S_1, \ldots, S_h)$ is called {\it $\AdvStructure$-private},
   if for every $Z \in \AdvStructure$, there is an $S \in \ShareSpec$, such that $Z \cap S = \emptyset$.
   A sharing specification $\ShareSpec = (S_1, \ldots, S_h)$ and an adversary-structure $\AdvStructure$ 
   satisfy $\Q^{(k)}(\ShareSpec, \AdvStructure)$ condition if the union of no $k$ subsets from $\AdvStructure$
   spans {\it any} subset from $\ShareSpec$. That is, for every $Z_{i_1}, \ldots, Z_{i_k} \in \AdvStructure$ and every
   $S \in \ShareSpec$:
%----
 \[  S \not \subseteq Z_{i_1} \cup \ldots \cup Z_{i_k}. \]
 %---
  We will be using the sharing specification $\ShareSpec = (S_1, \ldots, S_h)
 \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$, where $\AdvStructure$ is the adversary structure. Thus $\ShareSpec$ is
  {\it $\AdvStructure$-private}. If $\AdvStructure$ satisfies the
  $\Q^{(4)}(\PartySet, \AdvStructure)$ condition, then it also implies that $\AdvStructure$ and the above $\ShareSpec$
   satisfy the $\Q^{(3)}(\ShareSpec, \AdvStructure)$ condition.
   %----
 \subsection{Secret-sharing and Reconstruction Protocols}
 %----
 
 
 
 \paragraph{\bf Verifiable Secret-Sharing (VSS):}
 %----
 We use the perfectly-secure VSS protocol of \cite{CP20}, which
  allows a designated {\it dealer} to verifiably secret-share its input $s \in \F$.
   Apart from the input of the dealer, each (honest) party will have an ``external" participation-input, based on which the party decides how to participate in the protocol.
   Looking ahead, this external input will be decided based on the parent protocols, where the VSS protocol will be used as a sub-protocol, depending upon
   whether a party has locally identified the dealer to be corrupt in the parent protocol. For an
   {\it honest} dealer, it will be guaranteed that the parent protocol eventually sets the participation-input positively for every honest party.
    We stress that this external input was not used in \cite{CP20} and we slightly modify the protocol in our context to decide the actions of the parties
    based on their participation-inputs.
   
   If the dealer is {\it honest}, then the honest parties eventually complete the protocol with a secret-sharing of $s$, such that
   the view of the adversary remains independent of $s$. 
      If the dealer is {\it corrupt} and {\it no} honest party participates with a positive participation-input, then the protocol never gets completed for any honest party.
      However, if the dealer is {\it corrupt} and some honest party completes the protocol\footnote{This implies that at least one honest party
      participated with a positive participation-input. However, it {\it need not} be the case that {\it all} honest parties
      participated with a positive participation-input}, 
       then all honest parties eventually complete the protocol with a secret-sharing
    of some value (this is the verifiability guarantee provided by the protocol). 
    
    The high level idea of the protocol is as follows: dealer on having the input $s$, generates random shares $s_1, \ldots, s_h$ of $s$, where the share
    $s_q$ is given to all the parties in the set $S_q \in \ShareSpec$. To verify whether dealer has distributed the {\it same} share to all the parties in $S_q$, the 
    parties in $S_q$ perform pair-wise consistency test of the supposedly common share and {\it publicly} announce the result. 
    Next the parties check if there exists a subset of ``core" parties $\C_q$, where $S_q \setminus \C_q \in \AdvStructure$, who have positively confirmed the pair-wise
    consistency of their supposedly common share. Such a subset $\C_q$ is guaranteed for an {\it honest} dealer, as the set of honest parties in $S_q$ always 
    constitute a candidate $\C_q$. To ensure that all honest parties have the same version of the core sets $\C_1, \ldots, \C_h$, \
    dealer is assigned the task of identifying these sets based on the results of the pair-wise consistency tests and making them public. 
    Once the core sets are identified and verified, it guarantees that within each core set $\C_q$,    
    dealer has distributed some common share  to all {\it honest} parties within $\C_q$.
    The next goal is to ensure that even the honest parties in $S_q \setminus \C_q$ get this common share.
    For this, the (honest) parties in $S_q \setminus \C_q$ ``filter" out the supposedly common shares received during the pair-wise consistency test
    and ensure that they obtain the common share held by the honest parties in $\C_q$. 
    
    The protocol described till now is {\it without} considering the participation-inputs.\footnote{In fact, this is the way protocol was designed in \cite{CP20}}
    To take into account the participation-inputs, the protocol is modified as follows: a party participates in the pair-wise consistency tests if and only if
    its participation-input is {\it positive}. For the rest of the protocol steps, the party participates as above, {\it irrespective} of its participation-input.
    This is signified in the formal description of the protocol by presenting the protocol steps for the pair-wise consistency test in red color. 
    Notice that if the participation-input of {\it all} honest parties is {\it negative}, then the protocol
    never gets completed, as no core sets will be found, as otherwise the $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition (and hence the 
    $\Q^{(3)}(\ShareSpec, \AdvStructure)$ condition)  is violated. The VSS protocol is presented in Figure \ref{fig:PerAVSS}.

%----
\begin{protocolsplitbox}{$\PiPerVSS$}{The perfectly-secure VSS protocol in the $\FAcast$-hybrid model. 
 The public inputs are $\PartySet$, $\AdvStructure$, sharing specification $\ShareSpec = (S_1, \ldots, S_h)$ 
 and the dealer $P_{\D}$. The above steps are executed by every $P_i \in \PartySet$}{fig:PerAVSS}
\justify
%----

\begin{myitemize}
%----
\item {\bf Distribution of shares by $P_{\D}$} : If $P_i$ is $P_{\D}$, then execute the following steps.
	\begin{myenumerate}
	%----
	\item On having input $s^{(1)}, \ldots, s^{(h)} \in \F$, for each $S_q \in \ShareSpec$, send $(\dist,\sid,q,s^{(q)})$ to all parties $P_i \in S_q$.
	%----
	\end{myenumerate} 
%----
\item {\bf Pairwise consistency tests} : For each $S_q \in \ShareSpec$, if $P_i \in S_q$, then execute the following steps on having input $\participate$.
	\begin{myenumerate}
	%----
	\item Upon receiving $(\dist,\sid,q,s^{(q)}_i)$ from $\D$, send $(\test,\sid,q,s^{(q)}_i)$ to every party $P_j \in S_q$.
	%----
	\item Upon receiving $(\test,\sid,q,s^{(q)}_j)$ from $P_j \in S_q$, if $s^{(q)}_i = s^{(q)}_j$, send $(\Sender,\Acast,\sid^{(q)}_{ij},\OK_q(i,j))$ to $\FAcast$, where $\sid^{(q)}_{ij} = \sid || q || i || j$.
	%----
	\end{myenumerate}
%----
\item {\bf Constructing consistency graph} : For each $S_q \in \ShareSpec$, execute the following steps.
	\begin{myenumerate}
	%----
	\item For every $P_j \in S_q$, request output for every $P_k \in S_q \setminus \{P_j\}$ with $\sid^{(q)}_{jk}$ from $\FAcast$ until $(P_j,\Acast,\sid^{(q)}_{jk},\OK_q(j,k))$ is received.
	%----
	\item Initialize a set $\C_q$ to $\phi$. Construct a consistency graph $G^i_q$ with $S_q$ as the vertex set.
	%----
	\item Add the edge $(P_j,P_k)$ to $G^i_q$ if $(P_j,\Acast,\sid^{(q)}_{jk},\OK_q(j,k))$ and $(P_k,\Acast,\sid^{(q)}_{kj},\OK_q(k,j))$  is received from $\FAcast$. 
	%----
	\end{myenumerate}
%----
\item {\bf Identification of core sets} :  If $P_i$ is $P_{\D}$, then execute the following steps.
	%----
	\begin{myenumerate}
	%----
	\item For each $S_q \in \ShareSpec$, once a set $\W_q$ of parties which form a clique in $G^{\D}_q$ is identified, such that $\W_q = \ S_q \setminus Z$ for some $Z \in \AdvStructure$, then assign $\C_q \coloneqq \W_q$.
	%----
	\item Upon computing non empty $\C_q$ for each $S_q \in \ShareSpec$, send $(\Sender,\Acast,\sid_{\D},\{ \C_q \}_{S_q \in \ShareSpec})$, where $\sid_{\D} = \sid || \D$.
	%----
	\end{myenumerate}
%----
\item {\bf Share computation} : Execute the following steps.
	%----
	\begin{myenumerate}
	%----
	\item For each $S_q \in \ShareSpec$ such that $P_i \in S_q$, set $[s]_q$ to $\bot$.
	%----
	\item Request output with $\sid_{\D}$ from $\FAcast$ until $(\Sender,\Acast,\sid_{\D},\{ \C_q \}_{S_q \in \ShareSpec})$ is received.
	%----
	\item Wait until the parties in $\C_q$ form a clique in $G^i_q$, such that $\C_q = S_q \setminus Z$ for some $Z \in \AdvStructure$, for all $S_q \in \ShareSpec$. Upon receiving $(\dist,\sid,q,s^{(q)})$ from a set of parties $\C'_q = \C_q \setminus Z$ for some $Z \in \AdvStructure$, set $[s]_q = s^{(q)}$.
	%----
	\item Upon setting $[s]_q$ to some non $\bot$ value for each $S_q \in \ShareSpec$ such that $P_i \in S_q$, output $(\Share,\sid,P_{\D},\{[s]_q\}_{P_i \in S_q})$.
	%----
	\end{myenumerate}
%----
\end{myitemize}
%----
\end{protocolsplitbox}
%----


    
    
    
    
  %----
\paragraph{Default Secret-Sharing:}
%---   
 We will use the perfectly-secure protocol $\PiPerDefaultShare$ which takes a {\it public} input $s \in \F$ along with a sharing specification $\ShareSpec = (S_1, \ldots, S_h)$ 
 and {\it non-interactively} generates a secret-sharing of $s$. For this, the parties collectively set $[s]_1 = s$ and $[s]_2 = \ldots = [s]_h = 0$.
  As the protocol is non-interactive, the adversary learns no additional information during the protocol.
 %-----
 \paragraph{Reconstruction Protocol:} 
  %---
  Let $s$ be a value which is secret-shared with respect to a sharing specification $\ShareSpec = (S_1, \ldots, S_h)$, such that 
  $\ShareSpec$ and the underlying adversary-structure $\AdvStructure$ 
   satisfy $\Q^{(2)}(\ShareSpec, \AdvStructure)$ condition. Moreover, let $q \in \{1, \ldots, h \}$ and the the goal is to {\it publicly} reconstruct
   the share $[s]_q$. This can be done easily using a perfectly-secure protocol $\PiPerRecShare$ presented in \cite{CP20}.
   In the protocol, each party in $S_q$ sends the share $[s]_q$ to every other party {\it outside} $S_q$.
   While the parties in $S_q$ can readily output $[s]_q$, the parties outside $S_q$ can eventually output $[s]_q$ by considering the 
   copy of $[s]_q$ received identically from a subset of parties in $S_q$ excluding some potentially corrupt subset from $\AdvStructure$.
   The protocol incurs a communication of $\Order(n^2 \log{|\F|})$ bits. 

   Given protocol $\PiPerRecShare$, one can publicly reconstruct $s$ by using a protocol $\PiPerRec$ by invoking an instance of $\PiPerRecShare$
   for each share of $s$. This will incur a communication of $\Order(|\ShareSpec| \cdot n^2 \log{|\F|})$ bits. For the sake of completeness, protocols 
   $\PiPerRecShare$ and $\PiPerRec$ are presented in Appendix \ref{app:Perfect}.
  %----
  \subsection{The AMPC Protocol in the Pre-Processing Model} 
  %---
  In this section, we present our perfectly-secure AMPC protocol assuming an ideal functionality $\FTriples$ (see Fig \ref{fig:FTriples}), which generates $M$ number of secret-shared
  random multiplication-triples, which are random from the point of view of the adversary (recall that $M$ is the number of multiplication gates in the circuit $\ckt$).
   The secret-shared triples are used for evaluating the multiplication gates in $\ckt$, using the Beaver's method \cite{Bea91}.
    Functionality $\FTriples$ allows the ideal-world adversary to specify the shares
    for each of the triples on the behalf of corrupt parties. 
    The functionality then ``completes" the sharings of all the triples randomly, while keeping them ``consistent" with the shares specified by the 
     adversary.\footnote{Looking ahead, in our realization of
    $\FTriples$, the real-world adversary will have full control over the shares of the corrupt parties, corresponding to the
    resultant random multiplication-triples generated in the protocol. To capture it, we make the provision for the adversary to specify the shares of the
    corrupt parties in $\FTriples$.}
    
   \begin{systembox}{$\FTriples$}{The ideal functionality for asynchronous pre-processing phase.}{fig:FTriples}
	\justify
%----
$\FTriples$ proceeds as follows, running with parties $\PartySet = \{P_1, \ldots, P_n \}$ and an adversary $\Sim$
 and is parametrized by a sharing specification $\ShareSpec = (S_1, \ldots, S_h)$ and an adversary-structure $\AdvStructure$, such that $\ShareSpec$ is {\it $\AdvStructure$-private}.
  Let $Z^{\star}$ denote the set of corrupt parties. 
  %---
    \begin{myitemize}
     %----
       \item If there exists a set of parties ${\cal A}$ such that $\PartySet \setminus {\cal A} \in \AdvStructure$ and every 
       $P_i \in {\cal A}$ have sent the message $(\triples, \sid, P_i)$, then send $(\triples, \sid, {\cal A})$ to $\Sim$
       and prepare the output as follows.
  %----
         \begin{myitemize}
       %----
         \item Generate a secret-sharing of $M$ number of random multiplication-triples. To generate
          one such sharing, randomly select $u, v \in \F$ and compute $w = u \cdot v$ and execute the steps for
           ``Single Sharing Generation" (see below)
           for $u, v$ and $w$.
           %---
             \item Let $\{([u^{(\ell)}], [v^{(\ell)}], [w^{(\ell)}] )\}_{\ell \in \{1, \ldots, M\}}$ be the resultant secret-sharing of the 
           multiplication-triples.
           Send a request-based delayed output
        $(\tripleshares, \sid, \{[u^{(\ell)}]_q, [v^{(\ell)}]_q, [w^{(\ell)}]_q) \}_{\ell \in \{1, \ldots, M\}, P_i \in S_q})$  to each $P_i \in \PartySet \setminus Z^{\star}$
        (no need to send the respective shares to the parties in $Z^{\star}$, as $\Sim$ already has the shares of all the corrupt parties).           
          %----    
    \end{myitemize}
    %-----
{\bf Single Sharing Generation}: The functionality does the following to generate a secret-sharing  of a given value $s$.
   %-------
       \begin{myitemize}
       %----
         \item Upon receiving $(\shares, \sid, \{s_q \}_{S_q \cap Z^{\star} \neq \emptyset})$ from $\Sim$, 
         randomly select $s_r \in \F$ corresponding to each $S_r \in \ShareSpec$ for which $S_r \cap Z^{\star} = \emptyset$, such that\footnote{Note that $\Sim$ {\it cannot}
         delay sending the shares on the behalf of the corrupt parties indefinitely. This is because in the corresponding real-world protocol,
         the adversary {\it cannot} delay indefinitely the generation of secret-sharing of the multiplication-triples.}
          %---
         \[ \displaystyle \sum_{S_q \cap Z^{\star} \neq \emptyset} s_q + \sum_{S_r \cap Z^{\star} \neq \emptyset} s_r = s. \]
         %----     
         \item For $q = 1, \ldots, h$, set the share $[s]_q = s_q$.
         %----    
       \end{myitemize}    
  %----
    \end{myitemize}
  %-----
  \end{systembox}
  %---
  
  The AMPC protocol $\PiPerAMPC$ (see Fig \ref{fig:PerAMPC}) is presented in the $(\FTriples, \FVSS, \FABA)$-hybrid model. 
  The parties start with a {\it pre-processing phase} by generating secret-sharing of $M$ number of random multiplication-triples through
 $\FTriples$.  Next in the {\it input phase}, each party acts as a dealer and generates a random secret-sharing of its input (for the circuit $\ckt$) by calling $\FVSS$. 
  To avoid an indefinite wait, 
  the parties next agree on a common subset $\CoreSet$ of input-providers, whose corresponding 
  function-inputs are eventually secret-shared. This is done by generalizing the {\it agreement on a common-subset} (ACS) protocol of \cite{BKR94}.
  The idea used here is to invoke $n$ instances of $\FABA$, where the $j^{th}$ instance is used to decide whether
  $P_j$ should be included in $\CoreSet$.
  
   
   Once $\CoreSet$ is decided, for the remaining parties the parties take a default-sharing of $0$ as the corresponding input. 
   The parties then jointly start evaluating each gate in $\ckt$ in a secret-shared fashion, where for each gate the parties generate a secret-sharing of 
   the gate-output from a secret-sharing of the gate-input(s). The linear gates are evaluated non-interactively due to the linearity of secret-sharing, 
   while for the multiplication gates the parties deploy the Beaver's method, using the secret-shared
   multiplication-triples generated in the pre-processing phase. 
   Finally once the function-output is secret-shared, the parties publicly reconstruct the same.
   
   In the protocol, all honest parties may not be reconstructing the function-output at the same ``time" and
   different parties may be at different phases of the protocol, as the protocol is executed asynchronously. Consequently, a party upon reconstructing the function-output
   cannot afford to terminate immediately, as its presence and participation might be needed for the completion of various phases of the protocol by other honest parties.
   Consequently, there is a {\it termination phase}, whose code is executed concurrently throughout the protocol to check if a party can ``safely" terminate the protocol with 
   the function output.

 %----
\begin{protocolsplitbox}{$\PiPerAMPC$}{The perfectly-secure AMPC protocol in the $(\FTriples, \FVSS, \FABA)$-hybrid model. The public inputs of
 the protocol are $\PartySet, \ckt$ and $\AdvStructure$. The above steps are executed by every 
 $P_i \in \PartySet$}{fig:PerAMPC}
	\justify
%----
Set the sharing specification as $\ShareSpec = (S_1, \ldots, S_h)
 \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$, where $\AdvStructure$ is the adversary structure.\footnote{Thus $\ShareSpec$ is
  {\it $\AdvStructure$-private}.}
%----
\begin{center}\underline{\bf Pre-Processing Phase}\end{center}
%----
Upon receiving the input $(\prep, \sid, P_i)$ from the environment, proceed as follows:
   %-----
     \begin{mydescription}
     %---
     \item [1.] Send $(\triples, \sid, P_i)$ to the functionality $\FTriples$.
     %---
     \item [2.] Request output from $\FTriples$ until receiving 
       $(\tripleshares, \sid, \{[u^{(\ell)}]_q, [v^{(\ell)}]_q, [w^{(\ell)}]_q) \}_{\ell \in \{1, \ldots, M\}, P_i \in S_q})$ from $\FTriples$. 
     %----
     \end{mydescription}  
%----
\begin{center}\underline{\bf Input Phase}\end{center}
 Once the output from $\FTriples$ is received then upon receiving the input $(\inp, \sid, x^{(i)})$ from the environment, proceed as follows:
%---
    \begin{myitemize}
    %----
    \item {\bf Secret-sharing of the Inputs and Collecting Shares of Other Inputs}:
    %---
      \begin{mydescription}
       %----
         \item Randomly select the shares $x^{(i)}_1, \ldots, x^{(i)}_h \in \F$, subject to the condition that
         $x^{(i)} = x^{(i)}_1 + \ldots + x^{(i)}_h$.
         Send $(\Dealer, \sid_i, (x^{(i)}_1, \ldots, x^{(i)}_h))$ to $\FVSS$, where 
         $\sid_i \defined \sid || i$.\footnote{The notation $\sid_i$ is used here to distinguish among the $n$ different calls to
         $\FVSS$.}
         %---
         \item For $j = 1, \ldots, n$, send $(\participate, \sid_j)$ to $\FVSS$ with $\sid_j$ and 
          request output,  until receiving
          $(\Share, \sid_j, P_j, \{[x^{(j)}]_q \}_{P_i \in S_q})$,  where $P_j$ acts as the dealer.          
       %---
      \end{mydescription}
     %-------------- 
    \item {\bf Selecting Common Input-Providers}: Initialize a set of {\it local input-providers} $\LocalProv_i$ to $\emptyset$
    and a set of {\it global input-providers} $\GlobalProv_i$ to $\emptyset$.
    %----
       \begin{mydescription}
         %------
             \item[1.]  If $(\Share, \sid_j, P_j, \{[x^{(j)}]_q \}_{P_i \in S_q})$ is received from $\FVSS$, then include $P_j$ to $\LocalProv_i$ and send              
              $(\vote, \sid_j, 1)$ to $\FABA$, 
              where $\sid_j \defined \sid || j$.\footnote{The notation $\sid_j$ is used here to distinguish among the $n$ different calls to
         $\FABA$.}
             %----
             \item [2.] For $j = 1, \ldots, n$, request outputs from $\FABA$ until receiving $(\decide, \sid_j, v_j)$.
             %---
             \item [3.] Include $P_j$ to $\GlobalProv_i$ if $(\decide, \sid_j, v_j)$ is received from $\FABA$, such that $v_j = 1$.
         %---
              \item [4.] If $\PartySet \setminus \GlobalProv_i \in \AdvStructure$,
               then stop executing step 1 under ``{\bf Selecting Common Input-Providers}" and send
              $(\vote, \sid_j, 0)$ to $\FABA$, for every $j \in \{1, \ldots, n \}$ such that $P_j \not \in \GlobalProv_i$.
          %----
             \item [5.] Once $(\decide, \sid_j, v_j)$ is received from $\FABA$ for every $j \in \{1, \ldots, n \}$, set
                  $\CoreSet = \{P_j: v_j = 1\}$.
            %---
            \item [6.] Wait until receiving $(\Share, \sid_j, P_j, \{[x^{(j)}]_q \}_{P_i \in S_q})$ from $\FVSS$ for every $P_j \in \CoreSet$.              
               For every $P_j \not \in \CoreSet$, participate in an instance of of the protocol $\PiPerDefaultShare$ with public input $0$, to generate a default secret-sharing of $0$.               
            %----
       \end{mydescription}
    \end{myitemize}
%----
\begin{center}\underline{\bf Circuit-Evaluation Phase}\end{center}
Wait until the Input Phase is completed, resulting in a set $\CoreSet$ of input providers and the shares
 for each input of the input-providers in $\CoreSet$ and the shares of the random multiplication triples are received. Then evaluate each gate $g$ in the circuit
 according to the topological ordering as follows, depending upon the type of $g$.
     %----
        \begin{myitemize}
         %-----
           \item {\bf Addition Gate}: If $g$ is an addition gate with inputs $x, y$ and output $z$, then corresponding to every $S_q$ such that
           $P_i \in S_q$, set $[z]_q = [x]_q + [y]_q$ as the share
           corresponding to $z$. Here $\{[x]_q\}_{P_i \in S_q}$ and $\{[y]_q\}_{P_i \in S_q}$ are $P_i$'s shares 
           corresponding to gate-inputs $x$ and $y$ respectively.
           %---
             \item {\bf Multiplication Gate}: If $g$ is the $\ell^{th}$ multiplication gate with inputs $x, y$ and output $z$, where $\ell \in \{1, \ldots, M \}$, then do the following:
        %----
               \begin{mydescription}
               %----
               \item [1.] Corresponding to every $S_q$ such that $P_i \in S_q$, set 
                  $[d^{(\ell)}]_q \defined [x]_q - [u^{(\ell)}]_q$ and $[e^{(\ell)}]_q \defined [y]_q - [v^{(\ell)}]_q$, where $\{[x]_q\}_{P_i \in S_q}$ and $\{[y]_q\}_{P_i \in S_q}$ are 
                  $P_i$'s shares corresponding to gate-inputs $x$ and $y$ respectively and $\{([u^{(\ell)}]_q, [v^{(\ell)}]_q, [w^{(\ell)}]_q)\}_{P_i \in S_q}$
                  are $P_i$'s shares corresponding to the $\ell^{th}$ multiplication-triple.
               %-----
               \item [2.] Participate in instances of $\PiPerRec$ with shares $\{[d^{(\ell)}]_q \}_{P_i \in S_q}$ and $\{[e^{(\ell)}]_q \}_{P_i \in S_q}$ to publicly reconstruct 
                 $d^{(\ell)}$ and $e^{(\ell)}$, where $d^{(\ell)} \defined x - u^{(\ell)}$ and $e^{(\ell)} \defined y - v^{(\ell)}$.
               %----  
               \item [4.] Upon reconstructing $d^{(\ell)}$ and $e^{(\ell)}$, corresponding to every $S_q$ such that $P_i \in S_q$, set
                 $[z]_q \defined d^{(\ell)} \cdot e^{(\ell)} + d^{(\ell)} \cdot [v^{(\ell)}]_q + e^{(\ell)} \cdot [u^{(\ell)}]_q + [w^{(\ell)}]_q$.
                 Set $\{[z]_q \}_{P_i \in S_q}$ as the shares corresponding to $z$.
               %---
               \end{mydescription}
        %----
          \item {\bf Output Gate}: If $g$ is the output gate with output $y$, then participate in an instance of $\PiPerRec$ with shares $\{[y]_q \}_{P_i \in S_q}$ to publicly
          reconstruct $y$.
        %----
       \end{myitemize}
%---
\begin{center}\underline{\bf Termination Phase}\end{center}
%---
Concurrently execute the following steps during the protocol:
   %----
   \begin{mydescription}
   %---
   \item[1.] If the circuit-output $y$ is computed, then send $(\Ready, \sid, P_i, y)$ to every party in $\PartySet$.
     %---
      \item[--] If the message $(\Ready, \sid, P_j, y)$ is received from a set of parties ${\cal A}$ such that $\AdvStructure$ satisfies  $\Q^{(1)}({\cal A}, \AdvStructure)$ condition, then 
       send $(\Ready, \sid, P_i, y)$  to every party in $\PartySet$.
       %---
       \item[--] If the message $(\Ready, \sid, P_j, y)$ is received from a set of parties $\W$ such that $(\PartySet \setminus \W) \in \AdvStructure$, 
       then output $y$ and terminate.
   %---
   \end{mydescription}
%---
\end{protocolsplitbox}
%----

The properties of the protocol $\PiPerAMPC$ are stated in Theorem \ref{thm:PerAMPC}, which is proved in Appendix \ref{app:Perfect}. Intuitively, 
 the protocol eventually terminates, as the set $\CoreSet$ is eventually decided. This is because even if the corrupt parties do not secret-share their inputs,
 the inputs of all honest parties are eventually secret-shared. Once $\CoreSet$ is decided, the evaluation of each gate will be eventually completed:
  while the addition gates are evaluated non-interactively, the evaluation of multiplication gates require reconstructing the corresponding masked gate-inputs
  which is eventually completed due to the reconstruction protocols.
  The privacy of the inputs of the honest parties in $\CoreSet$ will be maintained as the sharing specification $\ShareSpec$ is $\AdvStructure$-private.
  Moreover, the inputs of the corrupt parties in $\CoreSet$ will be independent of the inputs of the honest parties in $\CoreSet$, as inputs are secret-shared
  via calls to $\FVSS$. Finally, correctness holds since each gate is evaluated correctly. 
 %----
 \begin{theorem}
\label{thm:PerAMPC}
%---
Protocol $\PiPerAMPC$ UC-securely realizes the functionality $\Functionality$ (see Fig \ref{fig:FAMPC} in Appendix \ref{app:UC}) 
 with perfect security in the $(\FTriples, \FVSS, \FABA)$-hybrid model, in the 
 presence of a static malicious adversary characterized by an adversary-structure $\AdvStructure$, satisfying the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition.
  The protocol needs a communication of $\Order(|\AdvStructure| \cdot n^2 \log{|\F|})$ bits.\footnote{We stress that in the $(\FTriples, \FVSS, \FABA)$-hybrid, the protocol
  requires {\it only} $\Q^{(3)}(\PartySet, \AdvStructure)$ condition. To realize $\FTriples$, the condition $\Q^{(4)}(\PartySet, \AdvStructure)$ is needed, due to which
  the overall protocol will require $\Q^{(4)}(\PartySet, \AdvStructure)$ condition.}
%---
\end{theorem}
%----
\subsection{Protocol for Realizing $\FTriples$}
%----
In this section, we present a perfectly-secure protocol for securely realizing the functionality $\FTriples$.

%%%%%%%%OLD STUFF%%%%%%%%
\begin{comment}
%------
A perfectly-secure VSS protocol allows a designated {\it dealer} $P_D \in \PartySet$ to verifiably secret-share its input $s \in \F$.
  If the dealer is {\it honest} and all honest parties participate in the protocol, then the honest parties eventually complete the protocol with a secret-sharing of $s$.
  The verifiability guarantees that if the dealer is {\it corrupt} and some honest party completes the protocol, then all honest parties eventually complete the protocol with a secret-sharing
  of some value, provided all honest parties participate in the protocol.
   Note that for a {\it corrupt} dealer, it is {\it not} necessary that the honest parties complete the protocol, as dealer may not invoke the protocol at the first place
   or if ``sufficiently many"
    {\it honest} parties do not participate in the protocol.\footnote{Looking ahead, in our AMPC protocol, if a party $P_i$ is identified to be corrupted, then honest parties will stop
   participating in any subsequent VSS instance invoked by $P_i$ as a dealer. Consequently, in these instances, no output might be generated.} 
    The above requirements are formalized through the ideal functionality $\FVSS$, presented in Fig \ref{fig:FVSS}. Looking ahead, the way 
  $\FVSS$ will be used in our AMPC protocol is as follows: $P_D$ on having the input $s$, {\it randomly} picks the shares $s_1, \ldots, s_h \in \F$, subject to the condition that
  $s_1 + \ldots + s_h = s$ and sends the vector $(s_1, \ldots, s_h)$ to $\FVSS$, who then distributes the shares to the corresponding parties. 
  If $P_D$ is {\it honest} and $\ShareSpec$ is {\it $\AdvStructure$-private}, then this will ensure that the view of the adversary will be independent of $s$.
  %-----
  \begin{systembox}{$\FVSS$}{The ideal functionality for VSS for session id $\sid$.}{fig:FVSS}
	\justify
%----
$\FVSS$ proceeds as follows, running with parties $\PartySet = \{P_1, \ldots, P_n \}$ and an adversary $\Sim$ and is parametrized 
 by a sharing specification $\ShareSpec = (S_1, \ldots, S_h)$, adversary-structure $\AdvStructure$  and a dealer $P_D$. 
   %----
    \begin{myenumerate}
     %----
         \item Upon receiving $(\Dealer, \sid, (s_1, \ldots, s_h))$ from $P_D$ (or from $\Sim$ if $P_D$ is corrupt) and
         $(\participate, \sid)$ from a set of parties in $\PartySet \setminus Z$ for some $Z \in \AdvStructure$,
           do the following:\footnote{Note that if $P_D$ is {\it corrupt}, then
         $\Sim$ may not send any tuple $(s_1, \ldots, s_h)$ to $\FVSS$ or sufficiently many honest parties
         may not indicate their participation, in which case the functionality will not generate any output.}
         %-----
             \begin{myitemize}
             %----
             \item For $q = 1, \ldots, h$, set $[s]_q = s_q$.
             %---
           %  \item If $P_D$ is {\it not} corrupt, then send $(\Dealer, \sid, P_D)$ to $\Sim$.
             %--- 
             \item Generate a request-based delayed output $(\Share, \sid, P_D, \{[s]_q \}_{P_i \in S_q})$ for every {\it honest} party $P_i$.
             %---
             \end{myitemize}
         %----
       \end{myenumerate}  
  %---
  \end{systembox}
  %----
 
 In \cite{CP20}, a {\it perfectly-secure} VSS protocol $\PiPerVSS$ is presented, provided 
 the underlying $\ShareSpec$ and the adversary-structure $\AdvStructure$ 
   satisfy $\Q^{(3)}(\ShareSpec, \AdvStructure)$ condition. The protocol incurs a communication of $\Order(|\ShareSpec| \cdot \poly(n, \log{|\F|}))$ bits.
   In \cite{CP20}, the UC-security of $\PiPerVSS$
   was {\it not} shown and so for the sake of completeness, we present the
   protocol $\PiPerVSS$ and show that it securely realizes $\FVSS$ with 
    UC-security in Appendix \ref{app:Perfect}.
   %----
   \end{comment} 


   

==> statVSS.tex <==
\subsection{Statistically-Secure VSS Protocol}
%--
In this section, we present our statistically secure protocol $\PiStatVSS$, which realizes the functionality $\FVSS$ (Fig \ref{fig:FVSS}) with UC-security. The protocol allows a designated dealer $P_\D$ to secret-share a vector of shares $(s_1,\ldots,s_h)$, while ensuring that the parties output a secret sharing of $s \defined s_1 + \ldots + s_h$, such that $[s]_q = s_q$, for each $S_q \in \ShareSpec$. The protocol ensures that even if $P_\D$ is {\it corrupt}, if some honest party completes the protocol, then every honest party completes the protocol, such that there is some value which has been secret shared by $P_\D$.

The overall idea of the protocol is to make the parties agree on a ``core" set $\C_q$ of parties for each $S_q \in \ShareSpec$, such that $\C_q$ contains at least one {\it honest} party, say $P_h$. The set $\C_q$ is defined such that all parties in the set agree on the share $s_q$. Furthermore, each party in $\C_q$ must have received a {\it signature} on the value $s_q$ signed by every other party in $\C_q$, for every party in $\PartySet$ as a receiver. The {\it non-repudiation} of AICP enables $P_h$ to reveal the value of $s_q$, signed by every other party in $\C_q$, to all the parties {\it outside} $\C_q$ in $S_q$. Furthermore, the {\it unforgeability} of AICP ensures that with high probability, no corrupt party in $\C_q$ can reveal a value other than $s_q$, signed by $P_h$, to any party outside $\C_q$ in $S_q$. This enables {\it all} parties in $S_q$ to ``filter" out the value of $s_q$ from the core set of parties $\C_q$. 

The protocol proceeds as follows. $P_\D$ gives the share $s_q$ to all the parties in the set $S_q \in \ShareSpec$. To verify whether dealer has distributed the {\it same} share to all the parties in $S_q$, the parties in $S_q$ perform pairwise consistency tests of the supposedly common share, by giving a signature on the received share to every other party in $S_q$, for every party in $\PartySet$ as a receiver. Based on whether the signatures have been {\it accepted}, the parties publicly announce the results. Each party then constructs a {\it consistency graph}, where an edge between two parties indicates that both the parties have accepted shares on a common value, which can be revealed to all parties in $\PartySet$. $P_\D$ is then assigned the task of finding the ``core" sets $\C_q$ for each $S_q \in \ShareSpec$. To do this, $P_\D$ searches for a set of parties $\C_q$ in $S_q$ such that $S_q \setminus \C_q \in \AdvStructure$, and that the parties in $\C_q$ form a clique in its consistency graph. This can be found when $P_\D$ is {\it honest}, since the set of honest parties in $S_q$ forms a candidate set for $\C_q$. Since $\ShareSpec$ satisfies the $\Q^{(2)}(\ShareSpec,\AdvStructure)$ condition, $\AdvStructure$ satisfies the $\Q^{(1)}(\C_q,\AdvStructure)$ condition, and contains at least one {\it honest} party. Upon finding a valid core set for each $S_q \in \ShareSpec$, $P_\D$ makes them public. Once the parties receive and verify these, they can then ``filter" out the value of $s_q$ from the parties in $\C_q$. Protocol $\PiStatVSS$ is present in Figure \ref{fig:VSS_stat}. 

\begin{protocolsplitbox}{$\PiStatVSS(\PartySet,\AdvStruct,\D,\SharingSpec,(s^{(1)},\ldots,s^{(h)}))$}{Protocol for $\D$ to verifiably share value $s$}{fig:VSS_stat}
%----
\justify
%----   
\begin{myitemize}
%----
\item[--] {\bf Distribution of Shares by $P_{\D}$ : } If $P_i$ is $P_{\D}$, then execute the following steps.
	\begin{myitemize}
	%----
	\item On having input $s^{(1)}, \ldots, s^{(h)} \in \F$, for each $S_q \in \ShareSpec$, send $(\dist,\sid,q,s^{(q)})$ to all parties $P_i \in S_q$.
	%----
	\end{myitemize}  
%----
\item[--] {\bf Pairwise Consistency Tests and Public Announcement of Results : } For each $S_q \in \ShareSpec$, if $P_i \in S_q$, do the following.
%----
	\begin{myitemize}
	%----
	\item Upon receiving $(\dist,\sid,q,s_{qi})$ from $\D$, for all parties $P_j \in S_q \setminus \{P_i\}$ and $P_k \in \PartySet$, give $\ICSig(\sid^{(P_\D,q)}_{i,j,k}, P_i \rightarrow P_j \rightarrow P_k, s_{qi})$ to $P_j$, where $\sid^{(P_\D,q)}_{i,j,k} = \sid || P_\D || q || i || j || k$.
	%----
	\item Upon receiving $\ICSig(\sid^{(P_\D,q)}_{j,i,k}, P_j \rightarrow P_i \rightarrow P_k, s_{qj})$ from $P_j \in S_q$ for every party $P_k \in \PartySet$, if $s_{qi} = s_{qj}$, send $(\Sender,\Acast,\sid^{(P_\D,q)}_{i,j},\OK_q(i,j))$ to $\FAcast$, where $\sid^{(P_\D,q)}_{i,j} = \sid || P_\D || q || i || j$.
	%----
	\end{myitemize}
    %----
%----
\item[--] {\bf Constructing Consistency Graph} : For each $S_q \in \ShareSpec$, execute the following steps.
	\begin{myitemize}
	%----
	\item Initialize a set $\C_q$ to $\phi$. Construct an undirected consistency graph $G^{(i)}_q$ with $S_q$ as the vertex set.
	%----
	\item For every $P_j \in S_q$, and every $P_k \in S_q \setminus \{P_j\}$ request output with $\sid^{(P_\D,q)}_{j,k}$ from $\FAcast$ until $(P_j,\Acast,\sid^{(P_\D,q)}_{j,k},\OK_q(j,k))$ is received.
	%----
	\item Add the edge $(P_j,P_k)$ to $G^{(i)}_q$ if $(P_j,\Acast,\sid^{(P_\D,q)}_{j,k},\OK_q(j,k))$ and $(P_k,\Acast,\sid^{(P_\D,q)}_{k,j},\OK_q(k,j))$  is received from $\FAcast$. 
	%----
	\end{myitemize}
%----
\item[--] {\bf Identification of Core Sets and Public Announcements} :  If $P_i$ is $P_{\D}$, then execute the following steps.
	%----
	\begin{myitemize}
	%----
	\item For each $S_q \in \ShareSpec$, check if there exists a subset of parties $\W_q \subseteq S_q$, such that $S_q \setminus \W_q \in \AdvStructure$
	and the parties in $\W_q$ form a clique in the consistency graph $G^{\D}_q$. If such a $\W_q$ exists, then assign $\C_q \coloneqq \W_q$.
	%----
	\item Upon computing a set $\C_q$ satisfying the above conditions 
	for each $S_q \in \ShareSpec$, send $(\Sender, \Acast, \sid_{P_{\D}}, \allowbreak \{ \C_q \}_{S_q \in \ShareSpec})$, where $\sid_{P_{\D}} = \sid || P_{\D}$.
	%----
	\end{myitemize}
%----
\item[--] {\bf Share computation} : Execute the following steps.
	%----
	\begin{myitemize}
	%----
	%----
	\item For each $S_q \in \ShareSpec$ such that $P_i \in S_q$, initialize $[s]_q $ to $\bot$.
	%----
	\item Keep requesting an output from $\FAcast$ with $\sid_{\D}$ until an output is received.
	%----
	\item Upon receiving an output $(\Sender, \Acast, \sid_{P_{\D}}, \{ \C_q \}_{S_q \in \ShareSpec})$ from $\FAcast$ with $\sid_{P_{\D}}$, 
	wait until the parties in $\C_q$ form a clique in $G^{(i)}_q$, corresponding to each $S_q \in \ShareSpec$. Then verify if
	$S_q \setminus \C_q \in \AdvStructure$, for each $S_q \in \ShareSpec$. If the verification is successful, then proceed to compute the output for each $S_q$ such that $P_i \in S_q$
	as follows.
	%----
	    \begin{myenumerate}
	    %----
	    \item Corresponding to each $\C_q$ such that $P_i \in \C_q$, set $[s]_q = s_{qi}$. Reveal $\ICSig(\sid^{(P_\D,q)}_{j,i,k}, P_j \rightarrow P_i \rightarrow P_k, s_{qi})$ signed by party $P_j \in \C_q \setminus \{P_i\}$ to every party $P_k \in S_q \setminus \C_q$.  
	    %----
		\item Corresponding to each $\C_q$ such that $P_i \notin \C_q$, set $[s]_q = s_q$, where $\ICSig(\sid^{(P_\D,q)}_{k,j,i},P_k \rightarrow P_j \rightarrow P_i, s_q)$ has been received from $P_j \in \C_q$, for all signers $P_k \in \C_q \setminus \{P_j\}$
		
		%----
	    \end{myenumerate}
	    %----
	\item Once $[s]_q \neq \bot$ for each $S_q \in \ShareSpec$ such that $P_i \in S_q$, output $(\Share, \sid,P_{\D}, \{[s]_q\}_{P_i \in S_q})$.
	%----
	\end{myitemize}
%----
\end{myitemize}
\end{protocolsplitbox}

 \paragraph{Protocol $\PiStatVSS$ for secret-sharing $L$ vectors $\{(s^{(1,1)},\dots,s^{(1,h)}),\ldots,(s^{(L,1)},\dots,s^{(L,h)})\}$:} Protocol $\PiStatVSS$ can be easily extended to secret-share $L$ vectors by invoking AICP for a vector of values. Namely, for each $S_q \in \ShareSpec$, if party $P_i$ belongs to $S_q$, it invokes $\Auth$ and $\Reveal$ for the vector $\vec{S} = (s^{(1,q)},\ldots,s^{(L,q)})$ during pairwise-consistency tests, and share computation respectively. The rest of the protocol remains the same. Theorem \ref{thm:StatVSS} is proven in Appendix \ref{app:Statistical}.
 
\begin{theorem}
\label{thm:StatVSS}
%---
 Consider a static malicious adversary $\Adv$ characterized by an adversary-structure $\AdvStructure$, satisfying the $\Q^{(3)}(\PartySet, \AdvStructure)$ condition
  and let  $\ShareSpec = (S_1, \ldots, S_h) \defined \{ \PartySet \setminus Z | Z \in \AdvStructure\}$ be the sharing specification. Then protocol $\PiStatVSS$ UC-securely realizes the functionality $\FVSS$
   with statistical security in the $\FAcast$-hybrid model, in the 
   presence of $\Adv$.
   To share $L$ values, the protocol makes $\Order(|\AdvStructure| \cdot n^4)$ calls to $\FAcast$ with $\Order(\log{n})$ bit messages, $\Order(|\AdvStructure| \cdot n^3)$ calls to $\FAcast$ with $\Order(L \cdot \log{|\F|})$ bit messages
    and additionally incurs a communication of 
   $\Order(|\AdvStructure| \cdot ( n^4+n^3 \cdot L) \log{|\F|})$ bits. By replacing the calls to $\FAcast$ with protocol $\PiAcast$, the protocol incurs a total communication of $\Order(|\AdvStructure| \cdot (n^4 + n^3 \cdot L )\log{|\F|} + n^4 \log{n}))$
   bits.
%---
\end{theorem}
%-----
 
 We use the default sharing protocol $\PiPerDefaultShare$ and the reconstruction protocol $\PiPerRec$ to obtain a secret-sharing of a default value, and reconstruct a secret-shared value repsectively. 


==> symbols_env.tex <==
%--------------------------------------------------------------
%New Style boxes
%--------------------------------------------------------------



%----- Box Environment ---------------------------------------------------------
\RequirePackage{mdframed}

%Basic box structure with title box
\newenvironment{titlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		%skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		%skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=15pt}\setlist[enumerate]{leftmargin=15pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-0.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

%title box style
\tikzstyle{normal} = [thick, fill=white, text=black, draw, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]
\tikzstyle{gray} = [thick, fill=gray!90, text=white, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]

%box style
\mdfdefinestyle{commonbox}{%
	%align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	%innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	%splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}


\mdfdefinestyle{roundbox}{style=commonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{systembox}[3]
{\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gsystembox}[3]
{\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}}
	
	

\newenvironment{protocolbox}[3]
{\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}


\newenvironment{algobox}[3]
{\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{reductionbox}[3]
{\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gamebox}[3]
{\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{simulatorbox}[3]
{\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}
%-------------------------------------------------------------------------------



%-------------------------------------------------------------------------------
%Split Box for IEETran Version
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{splittitlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\mdfdefinestyle{commonsplitbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}

\newenvironment{protocolsplitbox}[3]
{\begin{splittitlebox}{Protocol \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}
	
\newenvironment{schemesplitbox}[3]
{\begin{splittitlebox}{Functionality \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}
	
	
\newenvironment{simulatorsplitbox}[3]
{\begin{splittitlebox}{Simulator \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}	
	
\newenvironment{experimentsplitbox}[3]
{\begin{splittitlebox}{Experiment \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}	


%------------------------------------------------------------------------------
% Full Width Environments
%------------------------------------------------------------------------------

\newenvironment{systembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gsystembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{protocolbox*}[3]
{\begin{strip}
\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{algobox*}[3]
{\begin{strip}
\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{reductionbox*}[3]
{\begin{strip}
\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gamebox*}[3]
{\begin{strip}
\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{simulatorbox*}[3]
{\begin{strip}
\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}




%------------------------------------------------------------------------------
%Basic box structure with mytitle box without embossed title
%------------------------------------------------------------------------------

%box style
\mdfdefinestyle{mycommonbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=3pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
}
\mdfdefinestyle{myroundbox}{style=mycommonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{titlebox*}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=0.3\baselineskip,
		skipabove={0.4em},
		skipbelow={1em},needspace=3\baselineskip,
		frametitleaboveskip=5em,
		innerrightmargin=5pt
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\normalfont \TitleCaption}\label{\TitleLabel}}
	\medskip
}

%------------------------------------------------------------------------------
% Box Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox}[3]
{\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygsystembox}[3]
{\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myprotocolbox}[3]
{\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myalgobox}[3]
{\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myreductionbox}[3]
{\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygamebox}[3]
{\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mysimulatorbox}[3]
{\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}
%-------------------------------------------------------------------------------


%------------------------------------------------------------------------------
% Full Width Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygsystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myprotocolbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myalgobox*}[3]
{\begin{strip}
		\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myreductionbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygamebox*}[3]
{\begin{strip}
		\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mysimulatorbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}






%-------------------------------------------------------------------------------
% Basic protocol box without Algohead NDSS
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{mytbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\newenvironment{mytsplitbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-0.8em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\newenvironment{mypbox}[3]
{\begin{mytbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytbox}}

\newenvironment{mypsplitbox}[3]
{\begin{mytsplitbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytsplitbox}}












